Can Selfish Groups be Self-Enforcing?

Algorithmic graph theory has thoroughly analyzed how, given a network describing constraints between various nodes, groups can be formed among these so that the resulting configuration optimizes a \emph{global} metric. In contrast, for various social and economic networks, groups are formed \emph{de facto} by the choices of selfish players. A fundamental problem in this setting is the existence and convergence to a \emph{self-enforcing} configuration: assignment of players into groups such that no player has an incentive to move into another group than hers. Motivated by information sharing on social networks -- and the difficult tradeoff between its benefits and the associated privacy risk -- we study the possible emergence of such stable configurations in a general selfish group formation game. Our paper considers this general game for the first time, and it completes its analysis. We show that convergence critically depends on the level of \emph{collusions} among the players -- which allow multiple players to move simultaneously as long as \emph{all of them} benefit. Solving a previously open problem we exactly show when, depending on collusions, convergence occurs within polynomial time, non-polynomial time, and when it never occurs. We also prove that previously known bounds on convergence time are all loose: by a novel combinatorial analysis of the evolution of this game we are able to provide the first \emph{asymptotically exact} formula on its convergence. Moreover, we extend these results by providing a complete analysis when groups may \emph{overlap}, and for general utility functions representing \emph{multi-modal} interactions. Finally, we prove that collusions have a significant and \emph{positive} effect on the \emph{efficiency} of the equilibrium that is attained.

==> Long/SAUVEGARDE/efficiency-long-SAUVEGARDE_copie.tex <==
\section{Efficiency Stability Trade-off}
\label{sec:efficiency}

\def\MIS{{\sc Maximum Independent Set problem}\xspace}

%However, choosing among multiple channels might add an extra computational complexity, that we characterize in this section.
%Also, the influence of transitivity remains open.

%It is interesting to denote that all our proofs for the existence of stable configurations rely on showing that some deviations increase the global utility. These arguments also imply that any configuration that has maximum utility is stable under these transformations.

%We then wish to study, more generally, the computational property and efficiency of all stable configurations.\\

Efficiency of configuration can be estimated through the sum of utility received by all the players. It has been proved in~\cite{Kleinberg:2010ul}, that computing a maximum partition is NP-complete even with uniform games. Hence, it does not only require coordination, but also has a prohibitive computational cost. We first strengthen this result by showing that this optimum cannot even be \emph{approximated} within a sublinear multiplicative factor.

\begin{lemma}
\label{lem:mcp-not-multiplicative}
For every $1 > \epsilon > 0$, the problem of finding a maximum partition cannot be approximated within any $n^{\epsilon - 1}$-ratio in polynomial time, unless P=NP.
\end{lemma}



However, we have a construction to show that using $q>1$ channels adds in general no particular difficulty to that computation.
It could be useful for classes of graphs for which we have a good 
approximation to find a maximum partition (see Figure~\ref{fig:transformation} for an intuition about the related transformation).

% we prove that as long as $\setW\subseteq\{-M\}\cup \NatInt^*$ the problem of computing a maximum configuration with $q$ channels is not more difficult than the problem of computing such a configuration for a graph with single channel obtained using a linear transformation. 
%described in Definition~\ref{def:transformation}.

\iffalse
\begin{definition}
\label{def:transformation}
For any graph $G=(V,w)$ with $\setW \subseteq \{-\infty\} \cup \NatInt$, 
let $G'=(V',w')$ be as follows. \\
\textbf{a)} For any $u \in V$, we have $q$ nodes $u_{1},u_{2}, \ldots, u_{q} \in V'$ and we set $w'_{u_{i},u_{j}} = -\infty$ for any $i,j$, $1 \leq i < j \leq q$; \\
\textbf{b)} For any $u,v \in V$ such that $w_{u,v} \in \{-\infty,0\}$, we set $w'_{u_{i},v_{j}} = w_{u,v}$ for any $i,j$, $1 \leq i, j \leq q$; \\
\textbf{c)} For any $u,v \in V$ such that $w_{u,v} > 0$, for any $g$, $1 \leq g \leq q$, we have two nodes $uv_{g,1}, uv_{g,2} \in V'$, as shown in Figure~\ref{fig:transformation}, such that for any $i, j$, $1 \leq i, j \leq q$: 
\\
$\bullet$ $w'_{u_{i},uv_{g,1}} = w'_{v_{i},uv_{g,1}} = (h(g,w_{u,v}) - h(g-1,w_{u,v}))/2$; \\
$\bullet$ $w'_{u_{i},v_{j}} = 0$; \\
$\bullet$ $w'_{uv_{g,1},uv_{g,2}} = 3 (h(g,w_{u,v}) - h(g-1,w_{u,v}))/4$; \\
$\bullet$ $w'_{y,uv_{g,2}} = -\infty$, $\forall y \notin \{ uv_{g,1},uv_{g,2} \}$; \\
$\bullet$ $w'_{uv_{g,1},uv_{g',1}} = -\infty$, $\forall g' \neq g$, $1 \leq g' \leq q$; \\
$\bullet$ $w'_{y,uv_{g,1}} = 0,\forall y\! \notin\!\{u_{i}, v_{i}, uv_{g',1}, uv_{g,2}, 1\!\!\leq i, g'\!\!\!\leq q\}$.
\end{definition}
\fi

\begin{figure}[t]
\centerline{\includegraphics[width=0.5\linewidth]{Figures/Transformation.pdf}}
%\vspace{-0.4cm}
\caption{Representation in the graph G' of an edge uv with positive weight in the transformation.}
\label{fig:transformation}
%\vspace{-0.2cm}
\end{figure}


\iffalse
Let $P'$ be a maximum partition of the nodes for $G'$. 
Note that $X(u_{i}) \neq X(u_{j})$ for any $i\neq j$, and $X(u_{i}) = X(v_{j})$ if, and only if, a unique $uv_{g,1}$ exists such that $X(u_{i}) = X(uv_{g,1}) = X(v_{j})$. 
From $P'$ we can then build a configuration $C$ with $q$ channels for $G$ by replacing all nodes $u_i$ by $u$ and deleting all nodes $uv_{g,1}$ and $uv_{g,2}$. 
The proof concludes by proving that $P'$ is not maximum if $C$ isn't.
Formally:

\begin{theorem}
\label{the:equivalence-maximum}
Assume $h$ concave.
From a maximum partition of the nodes for $G'$, we deduce in linear time a maximum configuration with $q$ channels for $G$.
\end{theorem}



\begin{proof}
Let $P'$ be any maximum partition for $G'$.
%Note that for any $u,v \in V'$, then $|P'(u_{i}) \cap P'(u_{j})| \in \{0,1\}$.
We prove several properties for $P'$.

a) For any $u \in V$, we have $X(u_{i}) \neq X(u_{j})$ for any $i, j$, $1 \leq i < j \leq q$, because $w'_{u_{i},u_{j}} = -\infty$.

b) For any $u,v \in V$ such that $w_{u,v} = -\infty$, we have $X(u_{i}) \neq X(v_{j})$ for any $i, j$, $1 \leq i, j \leq q$, because $w'_{u_{i},v_{j}} = -\infty$.

c) For any $u,v \in V$ such that $w_{u,v} > 0$, if there exist $i, j$, $1 \leq i, j \leq q$, such that $X(u_{i}) = X(v_{j})$, then we claim there exists $g$, $1 \leq g \leq q$, such that $X(u_{i}) = X(v_{j}) = X(uv_{g,1})$.
By contradiction.
If $X(u_{i}) = X(v_{j})$ and $X(u_{i}) = X(v_{j}) \neq X(uv_{g,1})$ for any $g$, $1 \leq g \leq q$, then we show there exists a  partition $P''$ for $G'$ such that $f(P'') > f(P')$.
Indeed, we proved before that $X(u_{i'}) \neq X(u_{j'})$ and $X(v_{i'}) \neq X(v_{j'})$ for any $i', j'$, $1 \leq i' < j' \leq q$.
Thus, there exists $g$, $1 \leq g \leq q$, such that $X(uv_{g,1}) \neq X(u_{i'})$ and $X(uv_{g,1}) \neq X(v_{i'})$ for any $i'$, $1 \leq i' \leq q$.
We get two cases:
\begin{enumerate}
\item if $X(uv_{g,1}) \neq X(y)$ for any $y \in V'$, then we add $uv_{g,1}$ in the group of $u_{i}$ and $v_{j}$ and we get $f(P'') = f(P') + 2 (h(g,w_{u,v}) - h(g-1,w_{u,v}))$.
\item if $X(uv_{g,1}) = X(uv_{g,2})$, then $X(uv_{g,1}) \neq X(y)$ for any $y \in V'$ by construction of $G'$.
Thus, we add $uv_{g,1}$ in the group of $u_{i}$ and $v_{j}$ and we get $f(P'') = f(P') + 2 (h(g,w_{u,v})-h(g-1,w_{u,v})) - 6 ( h(g,w_{u,v})-h(g-1,w_{u,v}) )/4 > f(P')$.
\end{enumerate}

d) For any $u,v \in V$ such that $w_{u,v} > 0$, if there exist $i, j, g$, $1 \leq i, j, g \leq q$, such that $X(u_{i}) = X(v_{j}) = X(uv_{g,1})$, then for any $g' < g$, we claim there exists $i', j'$, $1 \leq i', j' \leq q$, such that $X(u_{i'}) = X(v_{j'}) = X(uv_{g',1})$.
By contradiction.
If there exists $g' < g$ such that $X(u_{i'}) \neq  X(uv_{g',1})$ or $X(v_{j'}) \neq X(uv_{g',1})$ for any $i', j'$, $1 \leq i', j' \leq q$, then we again show there exists a partition $P''$ for $G'$ such that $f(P'') \geq f(P')$.
Indeed, as $h$ is concave, we have $h(g',w_{u,v})-h(g'-1,w_{u,v}) \geq h(g,w_{u,v})-h(g-1,w_{u,v})$ because $g' < g$.
There are three cases.
\begin{enumerate}
\item Without loss of generality, if for some $i'$, $1 \leq i' \leq q$, $X(u_{i'}) = X(uv_{g',1})$ and so, $X(v_{j'}) \neq X(uv_{g',1})$ for any $j'$, $1 \leq j' \leq q$, then we add $uv_{g',1}$ to the group of $u_{i}$ and $v_{j}$, and we add $uv_{g,1}$ to the group with $uv_{g,2}$.
We get the partition $P''$ such that $f(P'') = f(P') - (h(g',w_{u,v})-h(g'-1,w_{u,v})) + 2(h(g',w_{u,v})-h(g'-1,w_{u,v})) - 2(h(g,w_{u,v})-h(g-1,w_{u,v})) +  6 (h(g,w_{u,v})-h(g-1,w_{u,v}))/ 4 > f(P')$, because $X(uv_{g',1}) \neq X(uv_{g',2})$ and because $h$ is such that $h(g',w_{u,v})-h(g'-1,w_{u,v}) \geq h(g,w_{u,v})-h(g-1,w_{u,v})$.
\item If $X(u_{i'}) \neq X(uv_{g',1})$, $X(v_{j'}) \neq X(uv_{g',1})$ for any $i', j'$, $1 \leq i', j' \leq q$, and $X(uv_{g',1}) \neq X(uv_{g',2})$, then we add $uv_{g',1}$ to the group of $u_{i}$ and $v_{j}$, and we add $uv_{g,1}$ to the group with $uv_{g,2}$.
We obtain the partition $P''$ such that $f(P'') = f(P') - 2(h(g,w_{u,v})-h(g-1,w_{u,v})) + 2(h(g',w_{u,v})-h(g'-1,w_{u,v})) + 6 (h(g,w_{u,v})-h(g-1,w_{u,v}))/4 > f(P')$ by the choice of $h$.
\item If $X(u_{i'}) \neq X(uv_{g',1})$, $X(v_{j'}) \neq X(uv_{g',1})$ for any $i', j'$, $1 \leq i', j' \leq q$, and $X(uv_{g',1}) = X(uv_{g',2})$, then we add $uv_{g',1}$ to the group of $u_{i}$ and $v_{j}$, and we add $uv_{g,1}$ to the group with $uv_{g,2}$.
We obtain the partition $P''$ such that $f(P'') = f(P') - 2(h(g,w_{u,v})-h(g-1,w_{u,v})) + 2(h(g',w_{u,v})-h(g'-1,w_{u,v})) - 6 (h(g',w_{u,v})-h(g'-1,w_{u,v}))/4 + 6 (h(g,w_{u,v})\\-h(g-1,w-{u,v}))/4 > f(P')$ by the choice of $h$.
\end{enumerate}

To summarize, any maximum partition $P'$ for $G'$ is such that:
for any $u \in V$, $X(u_{i}) \neq X(u_{j})$ for any $i \neq j$, $1 \leq i,j \leq q$;
for any $u, v \in V$ such that $w_{u,v} = -\infty$, $X(u_{i}) \neq X(v_{j})$ for any $i, j$, $1 \leq i,j \leq q$;
for any $u, v \in V$ such that $w_{u,v} > 0$, then there exists $g$, $0 \leq g \leq q$, such that for any $g' \leq g$, there exists $i, j$, $1 \leq i, j \leq q$, such that $X(u_{i}) = X(v_{j}) = X(uv_{g',1})$, and for all $g' > g$, $X(uv_{g',1}) = X(uv_{g',2})$ and so, $X(uv_{g',1}) = \{uv_{g',1},uv_{g',2}\}$.

We get that any maximum partition $P'$ for $G'$ is such that one can always write $f(P') = c + f'(P')$ where $c$ is the constant $\sum_{u,v \in V, w_{u,v} > 0} \sum_{g=1}^{q}  6(h(g,w_{u,v}) -h(g-1,w_{u,v}))/4$, and $f'(P') = \sum_{u,v \in V, w_{u,v} > 0} \sum_{g=1}^{q} \ind{\exists i,j, X(u_{i}) = X(u_{j})} (h(g,w_{u,v})-h(g-1,w_{u,v}))/2$.

We now construct the corresponding configuration $C$ with $q$ channels for $G$.
For any group $X_{j} \in P$, we construct the group $X_{j}' \in C$ as follows.
For any $u \in V$, $u \in X_{j}'$ if, and only if, there exists $i$, $1 \leq i \leq q$, such that $u_{i} \in X_{j}$.
Clearly, the construction of $G'$ and the construction of $C$ can be done in linear time on the size of $G$.

By construction, we get that $f(C) = 4 f'(P')$.

We now prove that if $P'$ is maximum for $G'$, then $C$ is maximum for $G$.
First suppose $P'$ is maximum for $G'$.
By contradiction.
Suppose there exists a configuration $C'$ with $q$ channels for $G$ such that $f(C') > f(C)$.
We prove that there exists a partition $P''$ for $G'$ such that $f(P'') > f(P')$.
We construct $P''$ as follows.
For any group $X_{i_{q}} \in C'$, we construct the group $X_{i_{q}}'$ for $P''$ as follows:
sequentially, for any $u,v \in X_{i_{q}}$, there exist $i, j$, $1 \leq i,j \leq q$ such that $u_{i}$ and $u_{j}$ are not yet in one group in $P''$.
If there exist, we choose $u_{i}$ and/or $v_{j}$ that are yet in group $X_{i_{q}}'$.
Furthermore, if $w_{u,v} > 0$, we choose the smallest $g$, $1 \leq g \leq q$, such that $uv_{g,1}$ is not yet in one group in $P''$.
We add $u_{i}$, $u_{j}$, and $uv_{g,1}$ in group $X_{i_{q}}'$.

We get that $f(P'') = c + f'(P'')$ where $f'(P'') = f(C')/4$ by construction. 

Thus, we get $f(P'') > f(P')$ because $f'(P'') > f'(P')$.
A contradiction because $P'$ is maximum for $G'$.
Finally, $C$ is maximum for $G$.
\end{proof}
\fi






Note that, in our extended model with multichannels, the total utility of the players can only improve as the number of channels $q$ gets larger, because more configurations are available. Unfortunately, we also prove that computing the minimum number of channels that guarantee a given threshold global utility is hard to approximate.

\begin{theorem}
\label{the:min-q-pas-APX}
Given $U \geq 1$, computing $q^{*}$, the minimum $q$ for which there exists a configuration $C$ satisfying $f(C) \geq U$, cannot be approximated within $n^{1-\varepsilon}$ for any $\varepsilon > 0$ in polynomial time, unless P=NP.
\end{theorem}





However, in spite of this complexity, we prove that collusions and multiple channels have in general a beneficial effect on the price of anarchy, which is the ratio of the worst stable equilibrium to this optimal.
Nash Equilibria obtained by the dynamic of the system satisfy a general bound that improves with $q$, in contrast with worst Nash Equilibria that are always arbitrarily bad.
Finally, we show that higher order stability, although it is significantly harder to obtain in general, potentially improve this bound significantly.


%We first show that stable configurations arise naturally as the result of our greedy dynamics.
%Second, we study general bounds on the efficiency of stable configurations in comparison with the maximum.

% Increasing the number of channels clearly increases the global utility, that is for any graph $D$, there exists a configuration $C$ for $D$ with $q$ channels such that $f(C) > f(C')$ for any configuration $C'$ with $q' < q$ channels for $D$.
% Furthermore, as we have shown for the graph of Figure~\ref{fig:triangle} (Section~\ref{sec:model}), allowing users to have interaction with several channels, can stabilize the system.
% Indeed, the graph $D$ described in Figure~\ref{fig:triangle} does not admit a $2$-stable configuration with a single channel while there always exists a $k$-stable configuration with $q \geq 2$ channels for any $k \geq 1$.
% 
% Another good news is that, with $W=\{-M\} \cup W^{+}$ and for any concave function $h$, computing a maximum configuration with $q \geq 2$ channels can be reduced to the case single channel (Section~\ref{ssec:transfo}).
% However, computing the minimum number of channels that guarantees a certain global utility, cannot be approximated in polynomial time within any constant (Section~\ref{ssec:hardness-q-min}).










%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lem:mcp-not-additive}
The problem of finding a maximum configuration cannot be approximated within any additive constant in polynomial time, unless P=NP.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%

%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $\alpha \geq 0$ be any constant.
We will prove that there does not exist a polynomial algorithm for computing a configuration $C$ with single channel for a digraph $D$ such that $f(C') - f(C) \leq \alpha$ for any configuration with single channel $C'$ for $D$.
By contradiction.
Assume that such an algorithm exists.

Consider three finite disjoint sets $X$, $Y$, and $Z$, and consider $T$ a subset of $X \times Y \times Z$.
We suppose that $|X| = |Y| = |Z|$.
We construct the digraph $D=(V,A,w)$ as follows.
We set $V = X \cup Y \cup Z$.
For any $x \in X, y \in Y, z \in Z$, we set $w(x,y) = w(y,z) = w(x,z) = -M$ if and only if $(x,y,z) \notin T$ ($w(x,y) = w(y,z) = w(x,z) = 1$ if and only if $(x,y,z) \in T$).
Furthermore:
\begin{itemize}
\item $w(x_1,x_2) = -M$ for any $x_1,x_2 \in X$;
\item $w(y_1,y_2) = -M$ for any $y_1,y_2 \in Y$;
\item $w(z_1,z_2) = -M$ for any $z_1,z_2 \in Z$.
\end{itemize}

Note that any maximum configuration with single channel $C = (V_1, \ldots, V_c)$ is such that $|V_i| \leq 3$ for any $i$, $1 \leq i \leq c$.
Thus, for any configuration with single channel $C$, then $f_{u}(C) \leq 2$ for any $u \in V$.

We prove that there exists a maximum configuration with single channel $C$ such that $f(C) = 2|V|$ if and only if there exists $3$-dimensional matching $M \subseteq T$ with $|M| = \frac{|V|}{3}$.
From the previous remark, if $f(C) = 2|V|$, then $f_{u}(C) = 2$ for any $u \in V$.
Thus, $C$ is composed of $\frac{|V|}{3}$ triples and it means that there is $3$-dimensional matching $M \subseteq T$ with $|M| = \frac{|V|}{3}$.
Finally, the problem of deciding if there exists a maximum configuration with single channel $C$ for $D$ such that $f(C) = 2|V|$, is equivalent to the problem of deciding if there exists a $3$-dimensional matching $M \subseteq T$ with $|M| = \frac{|V|}{3}$, which is NP-complete~\cite{Kar72}.

If there does not exist such a configuration with single channel for $D$, then $f(C) \leq 2|V|-4$ for any configuration with single channel $C$ for $D$.

Let $x$ be any integer such that $x > \frac{\alpha}{4}$.
Let $D^{1}=(V^{1},A^{1},w^{1}), \ldots, D^{x}=(V^{x},A^{x},w^{x})$ be $x$ copies for $D$.
We construct the digraph $D^{*}=(V^{*},A^{*},w^{*})$ by the disjoint union of the $x$ copies $D^{1}, \ldots, D^{x}$ and we set $w^{*}(u,v) = -M$ for any $u,v$ such that $u \in V^{i}$, $v \in V^{j}$, and $i \neq j$, $1 \leq i,j \leq x$.
We only consider configurations with single channel $C^{*}=(V^{*}_{1}, \ldots, V^{*}_{c^{*}})$ for $D^{*}$ such that two nodes $u,v$ are such that $V^{*}_{i^{*}} \cap V^{*}_{j^{*}} = \emptyset$, $u \in V^{*}_{i^{*}}$ and $v \in V^{*}_{j^{*}}$,if $u \in V^{i}$, $v \in V^{j}$, and $i \neq j$, $1 \leq i,j \leq x$.

By previous remark, if any configuration with single channel $C^{*}$ for $D^{*}$ is such that $f(C^{*}) < 2x|V|$, then any configuration with single channel $C^{*}$ for $D^{*}$ is such that $f(C^{*}) < x(2|V|-4)$.

By assumption, if there exists a configuration with single channel $C^{*}$ for $D^{*}$ such that $f(C^{*}) = 2x|V|$, then the polynomial algorithm finds it because of the $\alpha$-additive approximation.
Indeed, otherwise we would find a configuration with single channel $C'^{*}$ such that $f(C^{*}) < x(2|V|-4)$ and $f(C'^{*}) < f(C^{*}) - \alpha$.
Thus, we would have a polynomial algorithm for the problem of computing a maximum configuration for the digraph $D$.
A contradiction (unless P=NP) because, even for such instances, this problem is NP-complete.
Thus, there does not exist such a polynomial algorithm.
Finally, the problem cannot be approximated within any additive constant $\alpha \geq 0$, unless P=NP.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%




%\subsection{Maximum configuration}
%\label{ssec:transfo}


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let us constraint ourselves to the set of weights $\{-M,1\}$.
By contradiction, suppose there exists a polynomial-time algorithm $A$, such that for any graph $D$ we have $f(A(D)) \geq n^{\epsilon - 1} OPT(D)$.
We can use algorithm $A$ to compute an independent set of the conflict graph of $D$.
To do this, it suffices to take the largest group in $A(D)$.
Moreover, we know by~\cite{}, the \MIS cannot be approximated within any $n^{\frac{\epsilon}{2}- 1}$-ratio in polynomial time, unless P=NP.
Then, if P $\neq$ NP, there are graphs $D$ such that the largest group in $A(D)$ has size lesser than $n^{\frac{\epsilon}{2} - 1}|MIS(D)|$, where $MIS(D)$ denotes a maximum independent set of the conflict graph of $D$.
Especially, for such a graph $D$, we have $f(A(D)) < n.(n^{\frac{\epsilon}{2} - 1}|MIS(D)| - 1)n^{\frac{\epsilon}{2} - 1}|MIS(D)| < n^{\epsilon - 1}(|MIS(D)| - 1)|MIS(D)|$.
However, the utility of the configuration with single group $\{MIS(D)\}$ for $D$ is already $(|MIS(D)| - 1)|MIS(D)|$.
So, we have $f(A(D)) <  n^{\epsilon - 1} OPT(D)$, which is a contradiction unless P = NP.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%

%However, we show that using $q>1$ channels adds in general no particular difficulty to that computation. 

% we prove that as long as $\setW\subseteq\{-M\}\cup \NatInt^*$ the problem of computing a maximum configuration with $q$ channels is not more difficult than the problem of computing such a configuration for a graph with single channel obtained using a linear transformation described in Definition~\ref{def:transformation}.


%%%%% DEBUT DE DEFINITION COMMENTEE %%%%%
\iffalse
\begin{definition}
\label{def:transformation}
For any graph $D=(V,A,w)$ with $\setW \subseteq \{-M\} \cup \NatInt$, 
let $D'=(V',A',w')$ be as follows. \\
\textbf{a)} For any $u \in V$, we have $q$ nodes $u_{1},u_{2}, \ldots, u_{q} \in V'$ and we set $w'(u_{i},u_{j}) = -M$ for any $i,j$, $1 \leq i < j \leq q$; \\
\textbf{b)} For any $u,v \in V$ such that $w(u,v) \in \{-M,0\}$, we set $w'(u_{i},v_{j}) = w(u,v)$ for any $i,j$, $1 \leq i, j \leq q$; \\
\textbf{c)} For any $u,v \in V$ such that $w(u,v) > 0$, for any $g$, $1 \leq g \leq q$, we have two nodes $uv_{g,1}, uv_{g,2} \in V'$, as shown in Figure~\ref{fig:transformation}, such that for any $i, j$, $1 \leq i, j \leq q$: 
\\
$\bullet$ $w'(u_{i},uv_{g,1}) = w'(v_{i},uv_{g,1}) = (h(g,w(u,v)) - h(g-1,w(u,v)))/2$; \\
$\bullet$ $w'(u_{i},v_{j}) = 0$; \\
$\bullet$ $w'(uv_{g,1},uv_{g,2}) = 3 (h(g,w(u,v)) - h(g-1,w(u,v)))/4$; \\
$\bullet$ $w'(y,uv_{g,2}) = -M$, $\forall y \notin \{ uv_{g,1},uv_{g,2} \}$; \\
$\bullet$ $w'(uv_{g,1},uv_{g',1}) = -M$, $\forall g' \neq g$, $1 \leq g' \leq q$; \\
$\bullet$ $w'(y,uv_{g,1}) = 0,\forall y\! \notin\!\{u_{i}, v_{i}, uv_{g',1}, uv_{g,2}, 1\!\!\leq i, g'\!\!\!\leq q\}$.
\end{definition}
\fi
%%%%% FIN DE DEFINITION COMMENTEE %%%%%



%%%%% DEBUT DE FIGURE COMMENTEE %%%%%
\iffalse
\begin{figure}[t]
\centerline{\includegraphics[width=0.8\linewidth]{Figures/Transformation.pdf}}
\vspace{-0.4cm}
\caption{Representation in the graph D' of an edge (u,v) with positive weight in Definition~\ref{def:transformation}.}
\label{fig:transformation}
\vspace{-0.2cm}
\end{figure}
\fi
%%%%% FIN DE FIGURE COMMENTEE %%%%%


%%%%% DEBUT D'EXPLICATION COMMENTEE %%%%%
\iffalse
Let $C'$ be a maximum single channel configuration in $D'$. Note that $|C'(u_{i}) \cap C'(u_{j})| = 0$ for any $i\neq j$, and $|C'(u_{i}) \cap C'(v_{j})| = 1$ if, and only if, a unique $uv_{g,1}$ exists such that $|C'(u_{i}) \cap C'(uv_{g,1}) \cap C'(v_{j})| = 1$. From $C'$ we can then build a configuration $C$ with $q$ channels by replacing all nodes $u_i$ by $u$ and deleting all nodes $uv_{x,1}$ and $uv_{x,2}$. The proof concludes by proving that $C'$ is not maximum if $C$ isn't.
Formally:
\fi
%%%%% FIN D'EXPLICATION  COMMENTEE %%%%%



% \begin{theorem}
% \label{the:equivalence-maximum}
% Assume $h$ concave.
% We can construct $G'$ in polynomial time from any given graph $G$ such that: from a maximum configuration with single channel for $G'$, we deduce in linear time a maximum configuration with $q$ channels for $G$.
% \end{theorem}
% 


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $C = (V_{1}, \ldots, V_{c})$ be any maximum configuration with single channel for $D'$.
Note that for any $u,v \in V'$, then $|C(u_{i}) \cap C(u_{j})| \in \{0,1\}$.
We prove several properties for $C$.

a) For any $u \in V$, we have $|C(u_{i}) \cap C(u_{j})| = 0$ for any $i, j$, $1 \leq i < j \leq q$, because $w'(u_{i},u_{j}) = -M$.

b) For any $u,v \in V$ such that $w(u,v) = -M$, we have $|C(u_{i}) \cap C(v_{j})| = 0$ for any $i, j$, $1 \leq i, j \leq q$, because $w'(u_{i},v_{j}) = -M$.
By contradiction.
If $|C(u_{i}) \cap C(v_{j})| = 1$ and $|C(u_{i}) \cap C(v_{j}) \cap C(uv_{x,1})| = 0$ for any $x$, $1 \leq x \leq q$, then there exists a a configuration $C'$ with single channel for $D'$ such that $f(C') > f(C)$.
Indeed, we proved before that $|C(u_{i'}) \cap C(u_{j'})| = 0$ and $|C(v_{i'}) \cap C(v_{j'})| = 0$ for any $i', j'$, $1 \leq i' < j' \leq q$.
Thus, there exists $x$, $1 \leq x \leq q$, such that $|C(uv_{x,1}) \cap C(u_{i'})| = 0$ and $|C(uv_{x,1}) \cap C(v_{i'})| = 0$ for any $i'$, $1 \leq i' \leq q$.
We get two cases:
\begin{enumerate}
\item if $|C(uv_{x,1}) \cap C(y)| = 0$ for any $y \in V'$, then we add $uv_{x,1}$ in the group of $u_{i}$ and $v_{j}$ and we get $f(C') = f(C) + 2 (h(x,w(u,v)) - h(x-1,w(u,v)))$.
\item if $|C(uv_{x,1}) \cap C(uv_{x,2})| = 1$, then $|C(uv_{x,1}) \cap C(y)| = 0$ for any $y \in V'$ by construction of $D'$.
Thus, we add $uv_{x,1}$ in the group of $u_{i}$ and $v_{j}$ and we get $f(C') = f(C) + 2 (h(x,w(u,v))-h(x-1,w(u,v))) - 6 ( h(x,w(u,v))-h(x-1,w(u,v)) )/4 > f(C)$.
\end{enumerate}

d) For any $u,v \in V$ such that $w(u,v) > 0$, if there exist $i, j, x$, $1 \leq i, j, x \leq q$, such that $|C(u_{i}) \cap C(v_{j}) \cap C(uv_{x,1})| = 1$, then for any $x' < x$, there exists $i', j'$, $1 \leq i', j' \leq q$, such that $|C(u_{i'}) \cap C(v_{j'}) \cap C(uv_{x',1})| = 1$.
By contradiction.
If there exists $x' < x$ such that $|C(u_{i'}) \cap C(v_{j'}) \cap C(uv_{x',1})| = 0$ for any $i', j'$, $1 \leq i', j' \leq q$, then there exists a configuration $C'$ with single channel for $D'$ such that $f(C') \geq f(C)$.
As $h$ is concave, we have $h(x',w(u,v))-h(x'-1,w(u,v)) \geq h(x,w(u,v))-h(x-1,w(u,v))$ because $x' < x$.
There are three cases.
\begin{enumerate}
\item Without loss of generality, if for some $i'$, $1 \leq i' \leq q$, $|C(u_{i'}) \cap C(uv_{x',1})| = 1$, and so $|C(v_{j'}) \cap C(uv_{x',1})| = 0$ for any $j'$, $1 \leq j' \leq q$, then we add $uv_{x',1}$ to the group of $u_{i}$ and $v_{j}$, and we add $uv_{x,1}$ to the group with $uv_{x,2}$.
We get the configuration $C'$ such that $f(C') = f(C) - (h(x',w(u,v))-h(x'-1,w(u,v))) + 2(h(x',w(u,v))-h(x'-1,w(u,v))) - 2(h(x,w(u,v))-h(x-1,w(u,v))) +  6 (h(x,w(u,v))-h(x-1,w(u,v)))/ 4 > f(C)$ because $|C(uv_{x',1}) \cap C(uv_{x',2})| = 0$ and because $h$ is such that $h(x',w(u,v))-h(x'-1,w(u,v)) \geq h(x,w(u,v))-h(x-1,w(u,v))$.
\item If $|C(u_{i'}) \cap C(uv_{x',1})| = 0$, $|C(v_{j'}) \cap C(uv_{x',1})| = 0$ for any $i', j'$, $1 \leq i', j' \leq q$, and $|C(uv_{x',1})| \cap C(uv_{x',2})| = 0$, then we add $uv_{x',1}$ to the group of $u_{i}$ and $v_{j}$, and we add $uv_{x,1}$ to the group with $uv_{x,2}$.
We obtain the configuration $C'$ such that $f(C') = f(C) - 2(h(x,w(u,v))-h(x-1,w(u,v))) + 2(h(x',w(u,v))-h(x'-1,w(u,v))) + 6 (h(x,w(u,v))-h(x-1,w(u,v)))/4 > f(C)$ by the choice of $h$.
\item If $|C(u_{i'}) \cap C(uv_{x',1})| = 0$, $|C(v_{j'}) \cap C(uv_{x',1})| = 0$ for any $i', j'$, $1 \leq i', j' \leq q$, and $|C(uv_{x',1}) \cap C(uv_{x',2})| = 1$, then we add $uv_{x',1}$ to the group of $u_{i}$ and $v_{j}$, and we add $uv_{x,1}$ to the group with $uv_{x,2}$.
We obtain the configuration $C'$ such that $f(C') = f(C) - 2(h(x,w(u,v))-h(x-1,w(u,v))) + 2(h(x',w(u,v))-h(x'-1,w(u,v))) - 6 (h(x',w(u,v))-h(x'-1,w(u,v)))/4 + 6 (h(x,w(u,v))\\-h(x-1,w(u,v)))/4 > f(C)$ by the choice of $h$.
\end{enumerate}

To summarize, any maximum configuration $C$ for $D'$ is such that:
for any $u \in V$, $|C(u_{i}) \cap C(u_{j})| = 0$ for any $i, j$, $1 \leq i,j \leq q$;
for any $u, v \in V$ such that $w(u,v) = -M$, $|C(u_{i}) \cap C(v_{j})| = 0$ for any $i, j$, $1 \leq i,j \leq q$;
for any $u, v \in V$ such that $w(u,v) > 0$, then there exists $x$, $0 \leq x \leq q$, such that for any $x' \leq x$, there exists $i, j$, $1 \leq i, j \leq q$, such that $|C(u_{i}) \cap C(v_{j}) \cap C(uv_{x',1})| = 1$, and for $x' > x$, $|C(uv_{x',1}) \cap C(uv_{x',2})| = 1$ and so $|C(uv_{x',1})| = 2$.

We get that any maximum configuration $C$ for $D'$ is such that $f(C) = c(C) + f'(C)$ where $c(C)$ is the constant \\$\sum_{u,v \in V, w(u,v) > 0} \sum_{x=1}^{q}  6(h(x,w(u,v)) -h(x-1,w(u,v)))/4$ and $f'(C) = \sum_{u,v \in V, w(u,v) > 0} \sum_{x=1}^{q} \ind{\exists i,j, |C(u_{i}) \cap C(u_{j})|=1} \\2(h(x,w(u,v))-h(x-1,w(u,v)))/4$.

We now construct the corresponding configuration $C_{q}$ for $D$.
For any $V_{j} \in C$, we construct the group $V_{j'} \in C_{q}$ as follows.
For any $u \in V$, $u \in V_{j'}$ if, and only if, there exists $i$, $1 \leq i \leq q$, such that $u_{i} \in V_{j}$.
Clearly, the construction of $D'$ and the construction of $C_{q}$ can be done in linear time on the size of $D$.

By construction, we get that $f(C_{q}) = 4 f'(C)$.

We now prove that if $C$ with single channel is maximum for $D'$, then $C_{q}$ with $q$ channels is maximum for $D$.
Suppose $C$ is maximum for $D'$.
By contradiction.
Suppose there exists a configuration $C'_{q}$ with $q$ channels for $D$ such that $f(C'_{q}) > f(C_{q})$.
We prove that there exists a configuration $C'$ with single channel for $D'$ such that $f(C') > f(C)$.
We construct $C'$ as follows.
For any $V_{i_{q}} \in C'_{q}$, we construct the group $V_{i'_{q}}$ for $C'$ as follows:
sequentially, for any $u,v \in V_{i_{q}}$, there exist $i, j$, $1 \leq i,j \leq q$ such that $u_{i}$ and $u_{j}$ are not yet in one group in $C'$.
If there exist, we choose $u_{i}$ and/or $v_{j}$ that are yet in group $V_{i'_{q}}$.
Furthermore, if $w(u,v) > 0$, we choose the smallest $x$, $1 \leq x \leq q$, such that $uv_{x,1}$ is not yet in one group in $C'$.
We add $u_{i}$, $u_{j}$, and $uv_{x,1}$ in group $V_{i'_{q}}$.

We get that $f(C') = c(C') + f'(C')$ where $c(C') = c(C)$ and $f'(C') = f(C'_{q})/4$ by construction. 

Thus, we get $f(C') > f(C)$ because $f'(C') > f'(C)$.
A contradiction because $C$ is maximum for $D'$.
Finally, $C_{q}$ with $q$ channels is maximum for $D$.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%








% \subsection{Finding the necessary number of channels}
% \label{ssec:hardness-q-min}
% 
% We have shown that for a given value of $q$ obtaining optimal configurations is equivalent to a single channel, which remains computationally prohibitive. Another potential technique is to compute configuration while treating $q$ as a variable. Indeed, if $q$ is not limiting, users can obtain the maximum achievable utility for this system, by interacting separately with all their positive neighbors. Hence it could be that one can deduce from a graph the minimum value $q^*$ needed to reach a given utility. Unfortunately, as we can show with another transformation (Theorem~\ref{the:min-q-pas-APX}), no polynomial algorithm can find a correct approximation even if $\mathcal{W}=\{-M,0,1\}$. 
% 
% % Even if computing the maximum configuration is an NP-complete problem and cannot be approximated, we know that increasing the number of channels increase the global utility and we aim at computing a sufficient and small number of channels that guarantees relatively high global utility.
% % Thus, an important problem is to find the smallest number of channels that guarantees a global utility greater than a given threshold.
% % By Theorem~\ref{thm:stability:k=1}, such a configuration with $q$ channels is always $1$-stable.
% % We prove in Theorem~\ref{the:min-q-pas-APX} that the problem cannot be approximated within $|V|^{1-\varepsilon}$ for any $\varepsilon > 0$ in polynomial time, unless P=NP.
% 
% 
% \vspace{-0.2cm}
% \begin{theorem}
% \label{the:min-q-pas-APX}
% Given $U \geq 1$, computing $q^{*}$, the minimum $q$ for which there exists a configuration $C$ satisfying $f(C) \geq U$, cannot be approximated within $|V|^{1-\varepsilon}$ for any $\varepsilon > 0$ in polynomial time, unless P=NP.
% \end{theorem}
% 
% 
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
We construct the digraph $D=(V,A,w)$ as follows.
Let $D_{1}=(V_{1},A_{1},w_{1})$ be any digraph such that $w_{1}(u,v) \in \{-M,0\}$ for any $u,v \in V_{1}$.
Let $V=V_{1} \cup \{u, v_{1}, v_{2}, \ldots, v_{|V_{1}|}\}$.
We set $w(u,x) = N$ for any $x \in V_{1}$.
We set $w(u,v_{i}) = 1$ for any $i$, $1 \leq i \leq |V_{1}|$.
We set $w(v_{i},x) = -M$ for any $x \in V_{1}$ and for any $i$, $1 \leq i \leq |V_{1}|$.

Let $U = 2 |V_{i}|$.
Thus, if there exists a configuration $C$ for $D$ with $q$ channels such that $f(C) \geq U$, then $|C(u) \cap C(x)| \geq 1$ for any $x \in V \setminus \{u\}$.
Indeed there are exactly $2 |V_{i}|$ edges with weights $1$.
Thus, by construction of $D$, the problem remains to minimize the number of groups containing node $u$.
Clearly by construction, we have $|V_{i}|$ groups of size $2$ composed of $\{u,v_{i}\}$ for any $i$, $1 \leq i \leq |V_{i}|$.
Then, $u$ must be in one group with each $x \in V_{1}$.
As $w_{1}(u,v) \in \{-M,0\}$ for any $u,v \in V_{1}$, then we have to partition the nodes $V_{1}$ into groups without arcs with weight $-M$, and we have to minimize the number of groups.
Thus, the problem remains to find the chromatic number of the graph induced by arcs with weight $-M$.
As for all $\varepsilon > 0$, approximating the chromatic number within $n^{1-\varepsilon}$ is NP-hard~\cite{Zuck}, then we get the result.
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%




%%%%% DEBUT DE SECTION COMMENTEE %%%%%
\iffalse
\def\KL{{\sc KL Algorithm}\xspace}

\subsection{Computation of stable configurations}
\label{sec:stabcomput}

Theorems~\ref{thm:stability:k=1} and \ref{thm:stability:ktree} give sufficient conditions for the existence of a $k$-stable configuration.
The following greedy algorithm summarizes the constructive proofs.

Consider $q$ and $k$ as constant integers.
We take as an input a graph $D=(V,A,w)$,
and we first compute the configuration $C_0$ with $q$ channels, that is only composed of $q$ singleton groups per nodes of $V$.
Then we make iterations:
for every $i \geq 1$, the $i^{th}$ step of the greedy algorithm consists in finding a $k$-deviation for $C_{i-1}$, enumerating if necessary all the possible subsets.

\vspace{0.05cm}

\noindent
$\bullet$ If there exists a $k$-deviation, we compute the new configuration $C_{i}$, and an $i+1^{th}$ step of the algorithm starts. \\
$\bullet$ If there does not exist a $k$-deviation, then the configuration $C_{i-1}$ is $k$-stable.

\vspace{0.05cm}

This algorithm was first defined and used in~\cite{Kleinberg:2010ul} in order to compute stable configurations with single channel for the specific set $\mathcal{W}=\{-M,1\}$. It functions anytime the global utility increases at each step of the greedy algorithm, which is the case under the conditions of Theorems~\ref{thm:stability:k=1} and \ref{thm:stability:ktree}. Since the global utility is upper-bounded by a polynomial in $|V|$, it converges in polynomial time. It always yields a Nash Equilibrium, and under additional conditions on the weights and graphs, a $k$-stable configuration.

Note that, outside the conditions of the above theorems, this algorithm does not necessarily converge for $k \geq 2$, even for graphs where a $k$-stable configuration exists. This holds even for single channel: as an example, replace in Figure \ref{fig:triangle} (left) all edges with $w(u,v) = -M$ by edges with null weight $w(u,v) = 0$.
In the original graph, starting from a configuration where no enemies share a group, any $2$-deviation also induces a valid $2$-deviation in the new graph. Since the greedy algorithm in the original graph cannot converge for $k=2$ and will never put enemy in the same group, this implies an infinite series of $2$-deviation exists in the new graph. Thus, whereas in the new graph, a configuration where all nodes are in a single group is trivially stable for all $k$, greedy heuristics can be fooled not to find it. Although striking, this example is not a real surprise since we previously showed that deciding on the existence of a stable configuration is NP-complete.
\fi
%%%%% FIN DE SECTION COMMENTEE %%%%%



\subsection{Efficiency of Nash Equilibrium}
\label{sec:nashefficiency}

Since we proved there is few hope we can compute efficient configurations in polynomial time, our goal is now to study the efficiency of any stable configuration, and especially the ones that we can compute by using our dynamic system (extended to many channels).

We start by studying the efficiency of the largest class of stable configurations: Nash Equilibria ($k=1$).
%To simplify the analysis, we consider that $h$ takes only integer values; results hold in the general case with an additional constant.
Let us suppose $q$ to be fixed in the context.
For any graph $G$, we denote by $C^+$ (resp. $P^+$ when $q=1$) a maximum configuration with $q$ channels (resp. partition); the \emph{worst case} $C_k^-$ (resp. $P_k^-$) denotes a configuration with the minimum utility that is obtained in a $k$-stable configuration using $q$ channels (resp. partition).
We first show in Lemma~\ref{poa:infinite-ratio} that Nash Equilibria can be arbitrarily bad:


\begin{lemma}
\label{poa:infinite-ratio}
Assume here $q$ equals $1$.
Let $a,b > 0$ be two integers.
With $\mathcal{W} \supseteq \{-\infty,0,b\}$ or $\mathcal{W} \supseteq \{-a,b\}$, for any $R \geq 1$, there are graphs $G=(V,w)$ such that $f(P^+) \geq R$ and $f(P_1^-) = 0$.
\end{lemma}


%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{poa:infinite-ratio}
Given a positive integer $b$ and a set $\mathcal{W}$ such that $\{-M,0,b\} \subseteq \mathcal{W}$, for any $R \geq 1$, there are graphs $D=(V,A,w)$ with $f(C^+) \geq R$ and $f(C_1^-) = 0$.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%



%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $n' \geq \sqrt{R/2b}$ be an integer.
Let $D = (V,A,w)$ with $V = V_1 \cup V_2 \cup \{ v_{1}, v_{2}\}$, such that $|V_1| = |V_2| = n'$. 
For any $u,v \notin\{ v_{1}, v_{2}\}$, we set $w(u,v) = b$ if $u$ and $v$ are not in the same subset $V_i$, and $w(u,v) = 0$ otherwise. 
Moreover, $v_{1}$ ($v_{2}$, respectively) is enemy with any vertex of $V_{2}$ ($V_{1}$, respectively), and for any $u \in V_{1}$, any $v \in V_2$, we have $w(u,v_{1}) = w(v,v_{2}) = w(v_1,v_2) = 0$. 
Configuration $C$ containing $( V_1 \cup \{v_{1}\}, V_2 \cup \{v_{2}\})$ $q$ times is $1$-stable for $D$ and $f(C) = 0$.\footnote{This holds, for instance, if we choose $h(0,w) =0$, $h(g+1,w) = w$ for the proof.}
Furthermore, a maximum configuration with single channel for $D$ is $C^+ = ( V_1 \cup V_2, \{v_1,v_2\} )$  and $f(C^+) = 2bn'^2 \geq R$.
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%






%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{poa:infinite-ratio-2}
Given two positive integers $a,b$ and a set $\mathcal{W}$ such that $\{-a,b\} \subseteq \mathcal{W}$, for any $R \geq 1$, there are graphs $D=(V,A,w)$ with $f(C^+) \geq R$ and $f(C_1^-) = 0$.
\end{lemma}
\fi
%%%%% DEBUT DE LEMME COMMENTE %%%%%


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $n' \geq \frac{R}{2b(b+a)}$ be an integer.
Let $d = 2n'b$, and $n = 2n'(b+a)+1$.
First observe that $n > d$.
We claim that there exists a $d$-regular graph $G$ with $n$ vertices.
Indeed, let us choose $G$ such that the vertices in $G$ are labeled by the integers of $\mathbb{Z}_n$; for all $i,j \in \mathbb{Z}_n$, there is an edge $(i,j)$ in $G$ if, and only if, $j \equiv i - d/2 + \alpha$ (mod $n$), for every $0 \leq \alpha \leq d$ such that $\alpha \neq d/2$.

We now define the graph $D = (V,A,w)$ as follows.
The vertices in $D$ are the vertices in $G$.
For all $i,j \in \mathbb{Z}_n$, $i \neq j$, $w(i,j) = -a$ if $(i,j)$ is an edge of $G$, and $w(i,j) = b$ otherwise.

We have that $C = (V)$ is a $1$-stable configuration with single channel for $D$.
Furthermore, for all $i \in \mathbb{Z}_n$, $f_i(C) = -da + (n-d-1)b = 0$.

On the other hand, $C_p = (\{0,1\}, \{2,3\}, \ldots, \{n-3,n-2\}, \{n-1\})$ is a configuration with single channel for $D$ such that $f(C_p) = b(n-1) \geq R$.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%




%It is typically in noone's particular interest, and would unlikely emerge from the dynamics of local users.

%\paragraph{Greedy Nash Equilibria are always non-degenerate}


On the other hand, such situation is an oddity as precised in Lemma~\ref{greedy:upper-bound-gal}.
We now denote by $C^{\textrm{d}-}_{1}$ the worst equilibrium obtained under the dynamic of the system.
Also, recall that $w_p$ is the maximum weight of $\mathcal{W}$.


\begin{lemma}
\label{greedy:upper-bound-gal}
Given integers $q, n \geq 1$ and a set $\mathcal{W}$ such that $\mathcal{W}^+ \neq \emptyset$, for any graph $G=(V,w)$ with $\mathcal{W}$, we have $f(C^+)/f(C^{\textrm{d}-}_{1}) = O(h(q,w_p)n)$.
\end{lemma}





%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $D=(V,A,w)$ be a graph with $m_+$ the number of edges with positive weights.
We choose $D$ as an input for the greedy algorithm.
It takes $s \geq 0$ steps for computing a $1$-stable configuration $C_s$ with $q$ channels for $D$.
Note that $f(C_s) \geq s$ because the global utility strictly increases at each step (Theorem~\ref{thm:stability:k=1}). 

Let us denote $V_s$ the set of nodes $u$ such that there is at least one of their $q$ groups in $C_s$ that is not a singleton group.
We prove that $n_s \leq \ 2s$, where $n_s = |V_s|$.
Indeed, at each step of the algorithm, any vertex $v$ has at most one of its singleton groups that has been modified into another, larger group.
%Thus it takes at least $1$ step for a given vertex $v$ not having $q$ singleton groups anymore.
Furthermore, any such step modifies the singleton groups of at most two distinct vertices.

As a consequence, there are at most $nn_s \leq 2sn$ edges $(u,v)$ in $A$ such that $w(u,v) > 0$ and either $u \in V_s$ or $v \in V_s$.
Moreover, note that there does not exist any couple of vertices $u,v \in V \setminus V_s$, such that $w(u,v) > 0$, because $C_s$ is $1$-stable. 
Hence, $2sn \geq m_+$, and so $f(C^+)/f(C_s) \leq 2h(q,w_p)m_+/s = O(h(q,w_p)n)$.
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%



The upper-bound above, if it were tight, would imply that increasing of the number of channels might deteriorate the quality of the lowest computable Nash Equilibria.
On the contrary, we prove in Lemma~\ref{lemma:positive-impact} that the number of channels may have a positive impact for some  sets of weights. 

%\begin{lemma}
%Given two integers $q,n \geq 1$,
%for any digraph $D=(V,A,w)$, with any set of symmetric weights $W$, we have $\frac{f(C^+)}{f(C_1)} = O((1 + 2\frac{n}{q})h(q,w_{max}))$, if the two following conditions hold:
%\begin{itemize}
%\item  $|V| \leq n$;
%\item for every $w(u,v) \in W$, either $w(u,v) \geq 0$, or $w(u,v) = -M$.
%\end{itemize}
%\end{lemma}


\begin{lemma}
\label{lemma:positive-impact}
Given integers $q,n \geq 1$, and a set $\mathcal{W} = \mathcal{W}^+ \cup \{-\infty\}$ such that $\mathcal{W}^+ \neq \emptyset$, for any graph $G = (V,w)$ with $\mathcal{W}$, we have $f(C^+)/f(C^{\textrm{d}-}_{1}) = O((1 + 2n/q)h(q,w_p))$.
\end{lemma}






\subsection{Efficiency of higher order stability}
\label{sec:stabilityefficiency}

Increasing $k$ beyond 1 restricts further the set of stable configurations; they may even sometimes cease to exist. However, before this happens, we can expect the worst case configurations, and hence our general bounds, to improve.
We prove in Theorem~\ref{poa:upper-bound:kgeq2} that it is generally the case considering single channel case (the existence of a stable configuration is not guaranteed, but the result holds if it exists). 
As we constrain ourselves to partitions of the nodes anew, we will denote the configurations $P$ instead of $C$ in the sequel.

%providing it exists)(such as when conditions of Theorem~\ref{thm:stability:ktree} are satisfied) we have:
% As $k$-stable configurations may not exist for $k \geq 2$, definitions below only concern graphs $D = (V, A,w)$ such that there is a $k$-stable configuration for $D$.
% Moreover, we now only consider the single channel model.
%, as for $q \geq 2$, new degenerate stable configurations arise, with a negative global utility.


\begin{theorem}
\label{poa:upper-bound:kgeq2}
Given $\mathcal{W}$, any graph $G = (V,w)$ with weights in $\setW$ satisfies, $f(P^+)/f(P_k^-) = O(\Delta_+)$
for $k\geq 2$, where 
$\Delta_+=\max_{v\in V} |\lset u \dimset w_{u,v} > 0 \rset|$.
% we denote by $d_+(v)$ the number of edges $(u,v)$ such that $w(u,v) > 0$, and $\Delta_+ = \max_{v \in V } d_+(v)$. \\
\end{theorem}




%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Again, let $m_+$ be the number of edges $(u,v) \in E$ such that $w(u,v) > 0$.
We have that $f(C^+) \leq 2m_+w_p$.
Moreover, for every edge  $(u,v)$ of $E$ such that $w(u,v) > 0$, for any $k$-stable configuration $C_k$ for $D$, either $f_{u}(C_k) > 0$ or $f_{v}(C_k) > 0$.
Indeed, suppose $f_{u}(C_k) = f_{v}(C_k) = 0$. 
Then $\{u,v\}$ breaks $C_k$ by founding a new group, which is a contradiction.
Thus, there is at least $m_+/\Delta_+$ vertices $v$ of $V$ such that  $f_{v}(C_k) > 0$, as the same node cannot be counted more than $\Delta_+$ times.
Consequently, $f(C^+)/f(C_k^-) = O(\Delta_+) = O(|V|)$.
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%


In other words, we show that for $k\geq 2$ stable partitions are with a multiplicative factor of the optimal given by the maximum degree of a node in the friendship graph.

We define the \emph{price of $k$-anarchy} $p_a(n,k)$ as the greatest ratio $f(P^+)/f(P_k^-)$ obtained for a graph $G$ with $n$ nodes.
By considering a worst case degree, we have $p_a(n,k) = O(n)$. 
For a given $k$, this bound is tight: we can even construct a graph with $\setW\subseteq \NatInt$ and any other non trivial weights such that $f(P^+)/f(P_k^-) = \Omega(n)$. 


 \begin{lemma}
 \label{poa:lower-bound-1-2}
 Let $k$ be any integer $k \geq 2$.
 Given positive integers $b,b'$ such that $b' < b$, and a non-negative integer $a$, there is a graph $G=(V,w)$:
 \begin{itemize}
 \vspace{-0.2cm}
 \item with $\mathcal{W} \supset \{-a,b\}$, such that $\frac{f(P^+)}{f(P_k^-)}  \geq  \frac{ (k+1)\lfloor \frac{n}{(k+1)^2} \rfloor - 1}{k}$.
 \vspace{-0.2cm}
 \item  with $\mathcal{W} \supset \{b,b'\}$, such that $\frac{f(P^+)}{f(P_k^-)} \geq 1 + \frac{b'}{b}\frac{kb(\lfloor \frac{n}{kb} \rfloor - 1)}{kb-1}$.
 \end{itemize}
 \end{lemma}


%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{poa:lower-bound-1}
Given an integer $k \geq 2$, an integer $a \geq 0$, and an integer $b > 0$, for any set of weights $\mathcal{W}$ such that $-a,b \in \mathcal{W}$, there are graphs $D=(V,A,w)$ with $\mathcal{W}$ such that $\frac{f(C^+)}{f(C_k^-)}  \geq  \frac{ (k+1)\lfloor \frac{n}{(k+1)^2} \rfloor - 1}{k}$.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%

\iffalse
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\begin{proof}
a) Case $\mathcal{W} \supset \{-a,b\}$\\

\noindent
Let $n' = (k+1)^2 \lfloor \frac{n}{(k+1)^2} \rfloor \leq n$.
We build $G = (V,w)$ such that $|V| = n'$, as follows.
The vertices in $V$ are labeled $v_{i,j}$, with $1 \leq i \leq k+1$, and with $1 \leq j \leq n'/(k+1)$.
For every $1 \leq i \leq k+1$, the \emph{row} $L_i$ is the set $\{ v_{i,1}, v_{i,2}, \ldots, v_{i,\frac{n'}{k+1}}\}$.
In the same way, for every $1 \leq j \leq \frac{n'}{k+1}$, the \emph{column} $C_j$ is the set $\{v_{1,j}, \ldots, v_{k+1,j}\}$.
Furthermore, vertices $v_{i,j}$ and $v_{l,t}$ are friends, that is $w_{v_{i,j} , v_{l,t}} = b > 0$, if, and only if, either $i = l$ or $j = t$. 
Otherwise, $w_{v_{i,j} , v_{l,t}} = -a \leq 0$.\\

\noindent
Let us consider $P = \{ L_1, L_2, \ldots, L_{k+1} \}$ for $G$.
We have $f(P) =   n'b(\frac{n'}{k+1}-1)$.
On the other hand, we present $P' = \{ C_1, C_2, \ldots, C_{\frac{n'}{k+1}} \}$, and we claim that $P'$ is a $k$-stable partition for $G$.
Indeed, observe that for any $1 \leq j \leq \frac{n'}{k+1}$, any vertex $v_{i,j} \in C_j$ has one, and only one friend, in any other column. Hence, if $v_{i,j}$ were part of a subset $S$ that breaks $P'$, then after the $k$-deviation, $v_{i,j}$ would have, at most, $k$ friends in its group, which is already the case in $C_j$.
As a consequence, there is no vertex that can strictly increase its utility by a $k$-deviation, and so, the claim is proved.
However, $f(P') = n'bk$.
Finally, $\frac{f(P^+)}{f(P_k^-)} \geq  \frac{f(P)}{f(P')} = \frac{\frac{n'}{k+1}-1}{k} = \frac{ (k+1)\lfloor \frac{n}{(k+1)^2} \rfloor - 1}{k}$.\\
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%



%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{poa:lower-bound-2}
Given an integer $k \geq 2$, and two positive integers $b,b'$ such that $0 < b' < b$, for every $\mathcal{W}$ such that there is $b,b'\in \mathcal{W}$, there are graphs $D=(V,A,w)$ with $\mathcal{W}$ such that $\frac{f(C^+)}{f(C_k^-)} \geq 1 + \frac{b'}{b}\frac{kb(\lfloor \frac{n}{kb} \rfloor - 1)}{kb-1}$.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
 b) Case $\mathcal{W} \supset \{b,b'\}$\\

\noindent
This time, let $n' = kb \lfloor \frac{n}{kb} \rfloor$.
We build $G = (V,w)$ such that $|V| = n'$, as follows.
The set of vertices is partitioned  into $\frac{n'}{kb}$ parts, denoted $V_1, V_2, \ldots, V_{\frac{n'}{kb}}$, of equal size $kb$. 
For every couple of vertices $u,v$, $w_{u,v} = b$ if $u$ and $v$ are in the same part $V_i$, with $1 \leq i \leq \frac{n'}{kb}$, and $w_{u,v} = b'$ otherwise.

Obviously, a maximum (stable) partition for $G$ is $P = \{ V \}$, and $f(P) = n'[b(kb-1)+b'(n' - kb)]$.

Furthermore, we claim that $P' = \{ V_1, V_2, \ldots, V_{\frac{n'}{kb}} \}$ is a $k$-stable partition too. 
Indeed, any vertex $v$ that might break $P'$, by joining a coalition $S$ whose size is greater or equal to $k$, would have its individual utility after the deviation that is at most $(k-1)b + kbb' = kb(1+b') - b \leq kb^2 - b = (kb-1)b$. 
Hence $P'$ is $k$-stable, and $f(P') = n'b(kb-1)$.

Finally, $\frac{f(P)}{f(P')} = 1 + \frac{b'}{b}\frac{n' - kb}{kb-1} = 1 + \frac{b'}{b}\frac{kb(\lfloor \frac{n}{kb} \rfloor - 1)}{kb-1} $.  
\end{proof}
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\fi


% The last result is a bit surprising, because there are only positive weights and still, the ratio remains linear in the size of the graph. 
% A promising open problem is to prove new bounds as $k$ is allowed to grow with $n$.


==> Long/SAUVEGARDE/extensions-long-SAUVEGARDE.tex <==
\def\MIS{{\sc Maximum Independent Set problem}\xspace}

\section{Extensions of coloring games}
\label{sec:extensions}

All theoretical model of social dynamics should consider whether the overall behavior of the model is not too limited by some simplifying assumptions. We prove this is not the case, as our results extend to account for various situations in the formation of social groups. 

% captures Our model simplifies several aspects of the interaction between the nodes.
% For instance, it does not allow asymmetrical relations, \eg directed graphs.
% It does not allow group interactions either, with more than two nodes involved at the same time. 
% At last, another interesting extension is to consider more general graph decompositions, rather than only partitions.
% From a practical point of view, those three aspects may greatly benefit to our modelization of the Social Networks.
% 
% We will briefly present those three extended models in this section.
% Then we will show how the results in the previous parts can still be applied to them.

\subsection{Asymmetry and Gossiping}

Studying directed graphs rather than undirected graphs is a natural generalization.
In this case, we may not have that $w_{uv} = w_{vu}$ for all nodes $u,v$.
However, even if modest generalization of the model, asymmetrical weights lead to intractability.
This can be seen with a simple digraph $D=(\{u,v\},w)$ such that $w_{uv} > 0$ whereas $w_{vu} < 0$.
Furthermore, we prove in Theorem~\ref{theorem:oneStableConfigurationProblemNP} that it is NP-hard even to decide whether there exists a $1$-stable partition.
This result holds even when an upper-bound for the number of groups is known.
%We use in our reduction the multi-way partitioning number problem, which is NP-complete~\cite{Korf2009}.


\begin{theorem}
\label{theorem:oneStableConfigurationProblemNP}
For any $k \geq 1$, deciding whether there exists a $k$-stable partition for a given digraph $D=(V,w)$ is NP-hard, even if the number of groups is upper-bounded by any constant $g \geq 2$.
\end{theorem}


The same kind of pathological deviations arises with gossip.
In this extension, which is still symmetrical, the nodes that are willing to merge their groups are allowed to do so, even without the agreement of some users in their respective groups.
The $k$-deviations we studied so far are allowed as well.
One can easily check that, in the uniform case, there is a valid $1$-deviation whenever there exists a gossip-deviation. 
However, a first negative result has been proved in~\cite{Kleinberg:2010ul}: when $\mathcal{W}=\{-\infty,1,N\}$, it is NP-hard to decide whether a given weighted graph admits a gossip-stable partition.
We prove the same result when $\mathcal{W}=\{-\infty,0,1\}$.
Thus, Theorem \ref{NPKL} shows that gossiping makes the stability problem intractable, even for slight extensions of the original model of~\cite{Kleinberg:2010ul}.
%For our reduction, we use 3-coloring problem, that consists in determining whether there exists a proper $3$-coloring of a given graph $G=(V,E)$, a well known NP-complete problem~\cite{Dailey1980}.
%a well known NP-complete problem, even on planar graphs of degree $4$~\cite{Dailey1980}.
%A $k$-coloring of $G$ is a function $c : V \rightarrow \{1, \ldots, k\}$.
%The coloring is proper if $(u,v) \in E$ implies $c(u) \neq c(v)$.

\begin{theorem}
\label{NPKL}
Deciding whether there exists a $2$-stable, gossip-stable partition for a given graph $G=(V,w)$ is NP-hard, even with $\mathcal{W}=\{-\infty,0,1\}$.
\end{theorem}





%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $G$ be an instance for the 3-coloring problem.
We define the graph $D=(V,A,w)$ as follows.
For any vertex $v$ of $G$ there are five vertices $v_1,v_2,v_{c_1},v_{c_2},v_{c_3}$ in $V$.
We say that $v_{c_i}$ is a colored vertex, and that it has the color $i$.
There are also three special vertices in $V$, namely $c_1,c_2$ and $c_3$. 

For any vertex $v$ of $G$ we set $w(v_1,v_2) = 1$,  $w(v_1,v_{c_1}) = w(v_1,v_{c_2}) = w(v_1,v_{c_3}) = 1$,  $w(v_2,v_{c_1}) = w(v_2,v_{c_2}) = w(v_2,v_{c_3}) = 1$, and $w(v_{c_1},v_{c_2}) = w(v_{c_1},v_{c_3}) = w(v_{c_2},v_{c_3}) = -M$.
For any vertices $u,v$ in $G$, and for any $i,j\in{\{1,2,3\}}$, $i \neq j$, we also set $w(c_i,v_{c_i}) = w(c_i,u_{c_i}) = 1$, $w(c_i,c_j) = -M$, and $w(u_{c_i},c_j) = w(u_{c_i},v_{c_j}) = -M$.
In the case when $u$ and $v$ are adjacent in $G$, we set the weights $w(v_t,u_l) = -M$, for any $t,l\in{\{1,2\}}$.
Every other weight equals $0$.

We have that, for any $i$, and for any vertex $v$ of $G$, $v_{c_i}$ and $c_i$ gossip when they are not in the same group, because $w(v_{c_i},c_i) = 1$ and their enemies are the same. 
Furthermore, vertices $v_1$ and $v_2$ gossip when they are not in the same group too.
We now suppose there exists a gossip-stable configuration $C$ such that none of the vertices $v_{c_i}$ for $i\in{\{1,2,3\}}$ is in the same group as $v_1$ and $v_2$,
and we claim that there is a contradiction. 
Indeed, all the colored vertices that are in the same group as $v_1$ and $v_2$, if any, have the same color $i$, because otherwise there would be enemies in the group and $C$ would not be stable.
Thus, there is at least one vertex $v_{c_i}$ that breaks the configuration by joining the group of $v_1$ and $v_2$, because $w(v_{c_i},v_1) + w(v_{c_i},v_2) = 2$ whereas $w(v_{c_i},c_i) = 1$. 
A contradiction.

Finally, there can be only three groups in any gossip-stable configuration for $D$.
Moreover, we claim those three groups are equivalent to a proper $3$-coloring of $G$.
Indeed, suppose $C$ is a gossip-stable configuration for $D$, with only three groups.
We have that neither $c_1$ and $c_2$, nor $c_2$ and $c_3$, nor $c_3$ and $c_1$ are in the same group in $C$, because they are enemies.
Thus we can define a $3$-coloring of $G$ in the following way: for every vertex $v$ of $G$, $c(v) = i$ if, and only if, $v$ and $c_i$ are in the same group in $C$, with $1 \leq i \leq 3$.
This $3$-coloring is proper, because otherwise there would be enemies in at least one group in $C$. 

Conversely, suppose that we have a proper $3$-coloring $c$ of $G$.
We define the configuration  $C = \{ V_1, V_2, V_3 \}$ as follows.
For every $1 \leq i \leq 3$, $c_i \in V_i$, and any colored vertex $v_{c_i}$ is in $V_i$ too.
Furthermore, for all vertex $v$ of $G$, we have that $v_1,v_2 \in V_{c(v)}$.
By construction, there is no enemies in any of the three groups.
Moreover, we claim that there is no gossiping between any two vertices that are in different groups.
Indeed, there can only be gossiping between two vertices $v_j$ and $v_{c_i}$, with $j \in \{1,2\}$, $i \in \{1,2,3\}$, and $v_j \notin V_i$; however, the very definition of the configuration $C$ implies that $v_{c_i}$ has, at least, one enemy in the group of $v_j$, namely $c(v)$, and so, there is no gossiping at all.
To conclude, we claim that any subset $S$, $|S| \leq 2$, does not break the configuration $C$.
Indeed, the vertices in $S$ can only found a new group in $C$, by the very definition of the weights $w$ in $D$.
Furthermore, for all vertex $u \in D$, we have that $f_{u}(C) \geq 1$.
Hence, there is no vertex in $D$ that can strictly increase its utility by a $2$-deviation, and so, $C$ is a gossip stable configuration.   
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%


%Whereas the introduction of $N$ as a weight may be a strong constraint, the study  of $\{ -M, 0, 1\}$ seems far more natural and realistic. Thus Theorem \ref{NPKL} shows that gossiping makes the stability problem intractable, even for slight extensions of the original model of~\cite{Kleinberg:2010ul}. 
%That is the main reason why we decide to focus on cases where gossip is not admitted.



%\subsubsection{Asymmetrical Relations knowing an upper-bound on the number of groups}

%In fact, even when the number of groups in the configuration is given and fixed, deciding if there exists a $1$-stable configuration with asymmetric weights is NP-hard.
%In our reduction, we use partition problem, that consists in determining if there exists a partition of a given set of integers $S$ into two subsets $S_{1}$ and $S_{2}$ such that $\sum_{s_{1} \in {S_{1}}}s_{1} = \sum_{s_{2} \in {S_{2}}} s_{2}$.
%Partition problem is well known to be NP-complete~\cite{Kar72}.




%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{theorem}
\label{theorem:oneStableConfigurationProblemNP}
For any $k \geq 1$, deciding whether there exists a $k$-stable configuration for a given digraph $D=(V,A,w)$ is NP-hard, even if the number of groups is upper-bounded by $2$.
\end{theorem}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%

%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Consider an instance $S$ of Partition problem.
Let us call $T = \sum_{s\in{S}}s$.
We define the digraph $D=(V,A,w)$ as follows. 
The set of vertices is $V = S \cup {\{z,u,v\}}$.
For all $s_{1}, s_{2} \in{S}$ we set $w(s_{1},s_{2}) = - s_{2}$, $w(s_{1},u) = w(s_{1},v) = T - s_{1} + 1$, $w(u,s_{1}) = w(v,s_{1}) = 0$, and finally $w(s_{1},z) = - w(z,s_{1}) = s_{1}$. 
We also set $w(u,v) = w(v,u) = -M$, that $w(u,z) = w(v,z) = 0$, and that $w(z,u) = w(z,v) = T + 1$.
Such a digraph $D$ can be built in polynomial time.

First, in any stable configuration for $D$, we get that $u$ and $v$ must be in two different groups because they are enemies.
Furthermore, for all vertex $x\notin{\{u,v\}}$, $w(u,x) = w(v,x) = 0$, and so the other vertices do not matter for $u$ and $v$. 
Hence for any configuration $C$ such that $u$ and $v$ are already in two different groups, and for any $k$, there is no subset that contains $u$ or $v$ and that may break the configurationl.

Moreover, we recall that $w(z,s) < 0$ for any $s \in S$. 
Consequently, in any configuration $C$ for $D$ such that $z$ is neither in the same group as $u$, nor $z$ is in the same group as $v$, we get that $f_{z}(C) \leq 0$, whereas in any configuration $C'$ such that $z$ is in the same group as $u$ or $z$ is in the same group as $v$, we get that $f_{z}(C') \geq{1}$ because $\sum_{s \in {S}}w(z,s) = -T$ and $w(z,u)=w(z,v)=T+1$.

Hence, for any stable configuration for $D$, we conclude that either $z$ is in the same group $V_0$ as $u$, or $z$ is in the same group $V_1$ as $v$. Without any loss of generality, suppose $z$ in the same group $V_0$ as $u$.
We claim that any vertex $s$ in $S$ must be also in the same group $V_0$ as $u$ and $z$ or in the same group $V_1$ as $v$.
Indeed, otherwise we would have that $f_{s}(C) \leq 0$, since $w(s,s') \leq 0$ for any $s'\in{S}$; however such a configuration $C$ is not $1$-stable, because if vertex $s$ joins the group $V_1$, then $f_{s}(C') > 0$, with $C'$ being the new configuration, due to the fact that $w(s,v) = T - s + 1 > 0$, and $T - s = - [ \sum_{s'\in{S}} w(s,s') ]$.
Thus, there can be only two groups in a stable configuration of $D$.

Let $C = \{V_0, V_1\}$ be a configuration for $D$ such that $u$ and $v$ are not in the same group in $C$, and $S_i = \{ s_i \in {S} | s_i \in {V_i} \}, i \in{\{0, 1\}}$.
We can assume that $S_0, S_1$ is a partition of $S$.
Let us call $T_i = \sum_{s_i\in{S_i}}s_i$.
By definition of $w$, for any $i \in{\{0,1\}}$, for all vertex $s_i$ of $S_i$, we get that $f_{s_{i}}(C) = T + 1 - \sum_{s'_i\in{S_i}}s'_i + c_{s_i} = T - T_i + 1 +  c_{s_i} = T_{1-i} + 1 + c_{s_i}$, where the value of $ c_{s_i}\in{\{0,s_i\}}$ depends on whether $z$ is in $V_i$. In the same way, one can prove that if $z$ is in $V_j$ for some $j \in {\{0,1\}}$ then $f_{z}(C) = T_{1-j} + 1$.

It is important to notice that there is no subset of $V$ that breaks the configuration $C$ in creating a new group. Indeed, $u$ and $v$ cannot be part of such a subset, and it cannot contain $z$ either, because $z$ must be in the group of $u$ or in the group of $v$.
Furthermore, in any subset of $S$ that is taken as a new group, all of the individual utilities are non positive, whereas they were positive in the original groups

Let $s \in{S}$ be a vertex of $V_i$ for some $i$, such that $T_i \leq{T_{1-i}}$. We get that $f_{s}(C) \geq{ T_{1-i} + 1}$.
Consequently, $s$ has no interest in moving into $V_{1-i}$, whatever it is a collective move or not, because in such a new configuration $C'$ we get that the new size of group $V_i$ is $T_i' \leq T_i - s$, and $f_{s}(C')  \leq{ T_i' + s + 1} \leq{ (T_i - s) + s + 1 = T_i + 1 } \leq{ T_{1-i} + 1}$.
We prove in a similar way that vertex $z$ has no interest in leaving the group $V_i$ when  $T_i \leq{T_{1-i}}$. Therefore if $S_0,S_1$ is a solution for the Partition problem, then $T_0 = T_1$, that is $T_i \leq T_{1-i}$ for all $i\in{\{0,1\}}$, and so for every $k\geq{1}$ we get that $C$ is a $k$-stable configuration for $D$.

Conversely, let us suppose that  $S_0,S_1$ is not a solution for the Partition problem, that is $T_i < T_{1-i}$ for some $i$, and let us show that $C$ is not a  $1$-stable configuration for $D$.
Obviously, $z$ moves into $V_{i}$ provided $z$ belongs to $V_{1-i}$.
So we now assume that $z$ is in $V_{i}$. Then any singleton $\{s_{1-i}\}$ with $s_{1-i} \in{S_{1-i}}$ breaks the configuration , because in the new configuration $C'$ where vertex  $s_{1-i}$ has moved into group $V_i$ we get that $f_{s_{1-i}}(C') = T_{1-i} + 1$, that is strictly greater than $f_{s_{1-i}}(C) = T_i + 1$.

Finally, for any $k \geq 1$, there is a $k$-stable configuration $C$ for the digraph $D$ if and only if there is a solution to the Partition problem for the set $S$.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%


%Note that we have upper-bounded the number of groups by $2$ only to ease the proof.
%Actually, the problem remains NP-hard for any upper-bound $g \geq 2$ for the number of groups.
%It suffices to replace partition problem by multi-way partitioning number problem, which is also NP-complete (see~\cite{Korf2009}).
%On the other hand, a necessary and sufficient condition for a digraph $D=(V,A,w)$ to have a $k$-stable configuration that contains only one group is that for all subset $S$ of $V$, with $|S| \leq k$, there is a vertex $u \in S$ such that $\sum_{v \in V} w(u,v) \geq \sum_{v' \in S} w(u,v')$.






%\subsubsection{Sufficient conditions to tractability}

%An idea that was first suggested in~\cite{KL12} was to constrain ourselves to the following rules.
%For all nodes $u,v$, either $uv$ is a conflict edge and so, $w(u,v) = w(v,u) = -M$, or $w(u,v), w(v,u) > 0$.
%This is still not enough, as there are digraphs $D$ that follow these rules such that there does not exist any $1$-stable configuration for $D$.
%One of them is presented in Figure~\ref{}.

%On the other hand, we may impose the stronger constraint that for all vertex $u$, there exists a weight $w_u$ such that for all vertex $v \neq u$, either $uv$ is a conflict edge or $w(v,u) = w_u$.
%That rule is inspired from the Social Status theory in the Social Networks (see~\cite{}).
%Especially, if $w_u = 1$ for any vertex $u$ of $V$, we are back to~\cite{KL12} with the symmetric set of weights $\{-M,1\}$.\\

%Let $D=(V,A,w)$ such that $w$ follows both the rules that are mentioned above.
%Also, let $C = (V_1, \ldots, V_c)$ be a configuration for $D$.
%For every group $V_i \in C$, we consider the parameter $s(V_i) = \sum_{v \in V_i} w_v$.
%Particularly, if we go back to the case $\{-M,1\}$, then we get that $s(V_i) = |V_i|$.
%By using that parameter function $s$, one can adapt the proofs in~\cite{KL12}.
%Hence, we have that there exists a $k$-stable configuration for $D$, for every $k \geq 1$.
%Especially, if $k=1$, then our dynamic system reaches a $1$-stable  configuration for $D$ in polynomial time.
%This can be shown by using the potential function $\varphi (C) = \sum_{i=1}^c s(V_i)^2$.


\subsection{Multi-modal relationship}

Our model so far is heavily biased towards pairwise relationship, as the utility of a player depends on the sum of her interaction with all other members of the groups. In reality, more subtle interaction occur: one may be interested to interact with either friend $u$ or $v$, but would not like to join a group where both of them are present. 
%Our goal is now to include group interactions between more than $2$ nodes.
%, for any maximum size of group $t \geq 2$.
%An infinite value for $t$ is allowed too.

Our analysis also generalize to this case. 
We define a coloring game over a weighted undirected hypergraph $H = (V,w)$, with $w$ a weight function from $\mathcal{P}_t(V)$ to $\mathbb{N}$, where $\mathcal{P}_t(V)$ denotes the subsets in $V$ of size at most $t$.
Note that $t = \infty$ is allowed by our model.
The utility of a node $u$ in partition $P$ now equals: 
\(\sum_{ \{u\} \subseteq A \subseteq X(u), \\|A| \leq t} w_{A}.\)

We prove in Lemma~\ref{lemma:hypergraph-1-stable} that $1$-stability is guaranteed. 
Interestingly, the proof uses a different potential function than the global utility: $\phi (P) = \sum_{i=1}^n \sum_{A \subseteq X_i,\\ |A| \leq t} w(A)$.
%Then the proof is quite the same as for the case of graphs.
%It does not correspond to the global utility in this model, because we must take into account there are hyperedges that do not have the same size.
%However, if we go back to our symmetrical model of graphs, then $\phi (C)$ equals half of $f(C)$.

\begin{lemma}
\label{lemma:hypergraph-1-stable}
For every hypergraph $H = (V,w)$, there exists a $1$-stable partition.
\end{lemma}



\iffalse
Note this assumed that players of a subset all receive the same gain. We also have proved that if that is not the case, the game is not stable even for $k=1$.


We give the proof for those new degenerate cases when $t=3$.

For every hyperedge $\{u_1,u_2,u_3\}$, let us denote by $w_{u_1}(u_2,u_2)$ the utility received by $u_1$ when $u_2$ and $u_3$ are in the same group than $u_1$.
That utility comes in addition to $w(u_1,u_2)$ and $w(u_1,u_3)$


%%%%% DEBUT DE LEMME COMMENTE %%%%%
\begin{lemma}
There exists a hypergraph $H = (V,E,w)$, with $\mathcal{W} = \{-M,1\}$ and asymmetrical group relations, such that there does not exist any $1$-stable configuration for $H$. 
\end{lemma}
%%%%% DEBUT DE LEMME COMMENTE %%%%%



%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\begin{proof}
Consider the hypergraph $H=(V,E)$ depicted in Figure~\ref{fig:example-4} with $V=\{u_0,u_1,u_2,u_3\}$ (the node labeled $i$ in the figure corresponds to $u_i$).
We set $w_{u_i}(u_i,u_j)=1$ for any $i,j \in \{0,1,2,3\}$, $i \neq j$.
Furthermore, we assume that each node has a unique transitive restriction:
\begin{itemize}
\item $w_{u_i}(u_{i+1},u_{i+2})=-M$ ($i$, $i+1$, and $i+2$ are taken modulo $4$);
\item otherwise the transitive utility is $1$.
\end{itemize}

The edges on Figure~\ref{fig:example-4} represent the unique restriction for each of the four nodes.
For example, the blue node $u_0$ does not want both $u_1$ and $u_2$ in its group because of the blue edge.

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.55]{Figures/example-4}
\end{center}
\caption{Counter-example for stability in the asymmetrical transitive model.}
\label{fig:example-4}
\end{figure}

We will prove that there does not exist a $1$-stable configuration $C$ for this instance by considering all the cases.

First, if $C$ is composed by a unique group, then the utility of each node is $-M$. Any node can forms its singleton group to get a utility of $1$.

Consider any configuration $C$ composed of one group of size $3$ and one group of size $1$.
The first group is composed of $u_i$, $u_{i+1}$, and $u_{i+2}$ for some $i$ (the values are taken modulo $4$).
Then, the utility of $u_i$ is $-M$ because $w_{u_i}(u_{i+1},u_{i+2})=-M$.
In that case, node $u_i$ can strictly improve its utility by joining the group of $u_{i-1}$ (its utility will be $2$ instead of $-M$).

Consider any configuration $C$ composed of two groups $V_1$, $V_2$ of size $2$.
There are two cases.
Consider first the case where $V_1=\{u_i,u_{i+1}\}$ and $V_2=\{u_{i+2},u_{i+3}\}$ for some $i$ (the value are taken modulo $4$).
In that case, utility of node $u_i$ is $2$ and can be $3$ if $u_i$ joins the other group $V_2$.
Indeed, recall that the unique transitive restriction for $u_i$ is between $u_{i+1}$ and $u_{i+2}$: $w_{u_i}(u_{i+1},u_{i+2})=-M$.
The other case is when $V_1=\{u_i,u_{i+2}\}$ and $V_2=\{u_{i+1},u_{i+3}\}$ for some $i$ (the values are taken modulo $4$).
In that case, $u_{i+2}$ can strictly improve its utility (from $2$ to $3$) by joining the other group $V_2$.
Again, the unique transitive restriction for $u_{i+2}$ is between $u_{i+3}$ and $u_i$.

Finally, if $C$ is composed of four singleton groups, then any node can strictly improve its utility by joining any of the three other nodes (the utility is $2$ instead of $1$).
\end{proof}
\fi

Moreover, all results on uniform games generalize.
Formally, it holds because for any group $X_j \in P$, the vertices $u$ in $X_j$ have a utility $\sum_{\{u\} \subset A \subseteq X_j,\\ |S| \leq t} w(A) = \sum_{i=1}^{t-1} \binom{|X_j| - 1}{i}$, which is monotically increasing in the size of their group. 

%Also, observe that in the case $\{-M,1\}$, we still have there exists a stable configuration for every $k$.
%Indeed, given a hypergraph $H = (V,E,w)$, let $C = \{ V_1, \ldots, V_c \}$ be a $1$-stable partition for $H$.
%Then, for any group $V_j \in C$, the vertices $u$ in $V_j$ have a utility $\sum_{\{u\} \subset S \subseteq V_j,\\ |S| \leq t} w(S) = \sum_{i=1}^{t-1} \binom{|V_j| - 1}{i}$, which is monotically increasing in the size of their group.
%Consequently, any deviation in our transitive model is also a deviation in our graph coloring game.
%Hence the whole results in Section~\ref{section:algorithms} can still be applied.

Given a general hypergraph $H=(V,w)$, we define the friendship hypergraph $H^+$ in the same way as the friendship graph in Section~\ref{subsec:-m01}.
A Berge cycle in $H^+$ is a sequence $v_0, e_0, v_1, \ldots, v_{p-1},e_{p-1}, v_0$, such that:
\begin{itemize}
\item $v_0, v_1, \ldots, v_{p-1}$ are pairwise different vertices;
\item $e_0, e_1, \ldots, e_{p-1}$ are pairwise different hyperedges;
\item for all $0 \leq i \leq p-1$, $v_i, v_{i+1} \in E_i$. 
\end{itemize}

If subsets of nodes have weights in $\mathcal{W}=\{-\infty,0,1\}$, there still exists a $k$-stable partition for a hypergraph $H$ if the girth of the friendship hypergraph $H^{+}$ is at least $k+1$. Note that it does not imply $2$-stability in general because the girth of a hypergraph may be $2$.


%\subsubsection{Set of weights $\{-M,0,1\}$}

%Our last contribution to this model is to prove our stability result about girth still holds for $\{-M,0,1\}$.

\begin{lemma}
\label{lem:hypergraph-1}
Let $H=(V,E)$ be an acyclic hypergraph, with $c$ connected components.
Then $|V| = \sum_{e \in E} (|e|-1) + c$.
\end{lemma}

\iffalse
That easy result extends the well-known property of forests to the hypergraphs.
We can now prove the following:
\fi


%%%%% DEBUT DE COROLLAIRE COMMENTE %%%%%
\begin{corollary}
Given an integer $k \geq 1$ and a hypergraph $H = (V,w)$ with $\mathcal{W} = \{-\infty,0,1\}$, there is a $k$-stable partition for $H$ if the girth of the friendship hypergraph $H^{+}$ is at least $k+1$.
\end{corollary}
%%%%% FIN DE COROLLAIRE COMMENTE %%%%%


We will omit the proof as it is quite the same as for Theorem~\ref{thm:stability:ktree}.
%Unfortunately, it does not imply anymore that there always exists a $2$-stable partition, because the girth of a hypergraph may be $2$.
%We can adapt the counter-example of Figure~\ref{fig:counter-examples} (left) to show that, indeed, there exists a hypergraph $H$ with $\mathcal{W} = \{-M,0,1\}$ such that there does not exist any $2$-stable partition for $H$.
In particular, there always exists a $2$-stable partition if the friendship hypergraph is simple, that is the intersection of two different hyperedges has size at most $1$.






\subsection{Multichannels}

Finally, one assumption of our model is that nodes form a partition, hence they are limited to a single channel to interact with their peers. 
In reality participants in social networks may engage in multiple groups. 
This motivates to extend partitions of the nodes $P$ into multisets, that we call  'configurations'.
We denote such a configuration $C$, and it is said to use $q$ channels if each user participate (at most) to $q$ groups.
As a user can always form singleton groups, we can assume that $|X(u)|=q$ for any $u$, where $X(u)$ now denotes the set of all groups in $C$ that contain $u$. 
In other words $C = (X_1,X_2,\ldots,X_{qn})$.
Note that partitions of the nodes $P$ are exactly configurations with a single channel.

The utility of $u$ depends on the number of groups that $u$ shares with each peer:
% \begin{equation}
% 	f__{u}(C) = \sum_{v \in V} h\left( \sum_{i}\ind{\{u,v\} \subset V_i}\vf w(u,v) \right)\ff 
% \end{equation}
\begin{equation}
	f_{u}(C) = \sum_{v \in V} h\left( \left| X(u)\cap X(v) \right| \vf w_{u,v} \right)\vf 
	\label{eq:userutility}
\end{equation}
where $h(g,w)$ is a function that measures the utility of sharing $g$ groups with a node with weight $w$.
%where $C(u)$ denotes the set of clubs in which $u$ participates, and $h(g,w)$ is a function that measures the utility of sharing $g$ groups with a node with weight $w$.
Note that we assume, without loss of generality, that
\[
\begin{disarray}{l}
	h(0,.)=0\vf h(.,0)=0 \midwor{and} \forall w\in\RelInt \vf h(1,w)=w \vf \\
% \forall w\in\Real\vf h(0,w)=0 \midwor{and} h(1,w)=w \vf 
% \forall g\in\NatInt\vf h(g,0)=0 \vf \\
\forall g\in\NatInt \vf w\mapsto h(g,w) \midwor{is a non-decreasing function,} \\
\forall w\in\RelInt \vf g\mapsto w\cdot h(g,w) \midwor{is a non-decreasing function.}
\end{disarray}
\]
%The first three equalities generalize our notion of indifference and the definition of weight. The fourth property ensures that weight always remain an actual expression of preferences. 
The last property simply ensures that $h(g,w)$ increases with $g$ when $w$ is positive, and decreases with $g$ when $w$ is negative. 
As an example: $h(g,w)=s(g)\cdot w$, for $s$ a non-decreasing function that initially takes values $0$ and $1$, always satisfies these properties.
Especially, when $s(g)=\ind{g>0}$:
\vspace{-0.2cm}
\begin{equation}
	f_{u}(C) = \sum_{v \in V} \ind{ X(u)\cap X(v) \neq \emptyset} \cdot w(u,v) \ff 
	\label{eq:userutility1channel}
\end{equation}
\vspace{-0.2cm}

%%%%% DEBUT DE FIGURE COMMENTE %%%%%
\iffalse
\begin{figure}[t]
\centerline{\includegraphics[width=\linewidth]{Figures/TriangleWPart.pdf}}
\vspace{-0.7cm}
\caption{Weights and 1-stable conf (example).}
\vspace{-0.45cm}
\label{fig:triangle}
\end{figure}
\fi
%%%%% DEBUT DE FIGURE COMMENTE %%%%%



%In order to motivate the multichannels model, we present an example of preferences by symmetric weights in Figure~\ref{fig:triangle}~(left), where enemies are connected by dashed lines. We assume here that the utility of a user follows Eq.(\ref{eq:userutility1channel}). With a single channel, and $k=1$, several stable configurations exist (see \eg Figure~\ref{fig:triangle}~(right)), while no configuration can be stable for $k\geq 2$. Indeed no single channel configuration is $2$ stable unless it contains either $\{u_1,v_2,v_3\}$, $\{v_1,u_2,v_3\}$, or $\{v_1,v_2,u_3\}$. Suppose $\{u_1,v_2,v_3\} \in C$. Among remaining nodes, $u_2$ and $u_3$ are enemies and hence in different groups; $v_1$ will then join $u_2$ as shown on the Figure. Hence, there is a $2$-deviation for $C$, namely: nodes $v_1$ and $v_2$ leave their respective groups, and join the group already containing $u_3$ to form a positive triangle.
%Using more channels can be beneficial, the following configuration 
%$
%\{u_1,v_2,v_3\}, \{v_1,u_2,v_3\}, \{v_1,v_2,u_3\}, 
%\{u_1\}, \{u_2\}, \{u_3\}
%$ \\ 
%uses only 2 channels and is $k$-stable for every $k \geq 1$.




%\subsubsection{Stability properties with multichannels}



Using the same potential function as before, \eg global utility, it follows that there always exists a $1$-stable configuration with $q$ channels.
It is now natural to wonder what is the behavior of $k(\mathcal{W})$ when the number of channels is higher than $1$.
While it may have none or positive effects, we show that it is not always the case.
%, even if the function $h$ is as simple as $h(0,w) = 0$, $h(g+1,w) = (1 + \varepsilon g)w$, where $\varepsilon > 0$ is arbitrarily small.
%\footnote{$M$ must be taken as large as $\varepsilon$ is small, for we should have $\varepsilon M > |V|\cdot h(q,\max\lset w(u,v)\dimset u,v\in V \rset )$ if we want to avoid that two vertices $u,v$ such that $w(u,v) = -M$ end in the same group.}.
Indeed, even for uniform games, Lemma~\ref{lem:contre-exemple-q=2} proves $k(\mathcal{W}) \leq 2$ with $2$ channels while $k(\mathcal{W}) = \infty$ with single channel. 
The idea is to emulate a weight $w_{u,v} = 0$ by forcing nodes $u$ and $v$ to be in a predetermined group.



\begin{lemma}
\label{lem:contre-exemple-q=2}
Let us fix $h$ is as $h(0,w) = 0$, $h(g+1,w) = (1 + \varepsilon g)w$, where $\varepsilon > 0$ is arbitrarily small.
There exists a graph $G=(V,w)$ with $\mathcal{W}=\{-\infty,1\}$ such that any configuration with $2$ channels for $G$ is not $3$-stable.
\end{lemma}



%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
We use the counter-example $D_{q=1}=\\(V_{q=1},A_{q=1},w_{q=1})$ of Lemma~\ref{lem:counter-example} for the proof.
Note that, for each node $u \in V_{q=1}$, there exists at most one node $v \in V_{q=1}$ such that $w_{q=1}(u,v) = 0$.

Given a clique $K=(V,A)$ or order $p > 2|V_{q=1}|$, we set $w(u,v) = 1$ for any $u,v \in V$.
We now assume that $\varepsilon < 1/p$ for the rest of the proof, and we construct the graph $D_{q=2}=(V_{q=2},A_{q=2},w_{q=2})$ as follows.
For any node $u \in V_{q=1}$ such that $w_{q=1}(u,v) \neq 0$ for any $v \in V_{q=1}$, we add a copy of $K$, denoted $K_{u}=(V_{u},A_{u})$.
We set $w_{q=2}(u,x) = 1$ for any $x \in V_{u}$.
For any edge $(u,v) \in A_{q=1}$ such that $w_{q=1}(u,v) = 0$, we add another copy of $K$, denoted $K_{(u,v)}=(V_{(u,v)},A_{(u,v)})$.
We set $w_{q=2}(u,x) = w_{2}(v,x) = 1$ for any $x \in V_{(u,v)}$.
Furthermore, we set $w_{q=2}(u,v) = 1$.
Finally, for any graph $K_{u}$, with $u \in V_{q=1}$, we set $w_{q=2}(y,x) = -M$ for any $y \in V_{q=1} \setminus \{u\}$ and for any $x \in V_{u}$.
Similarly, for any graph $K_{(u,v)}$, with $(u,v) \in A_{q=1}$, we set $w_{q=2}(y,x) = -M$ for any $y \in V_{q=1} \setminus \{u,v\}$ and for any $x \in V_{(u,v)}$.\\

\noindent
First, we get that for any $u,v \in V_{q=1}$ such that $w(u,v) = 0$, for any $x,y \in V_{(u,v)}$, $|C(x) \cap C(y)| = 2$  in any $3$-stable configuration $C = (V_{1}, \ldots, V_{c})$ with $2$ channels for $D_{q=2}$.

As $\epsilon M > n$, we have that any $x \in V_{(u,v)}$ cannot be in a group containing any node $y \in V_{q=2} \setminus (A_{(u,v)} \cup \{u,v\})$.

We first prove that in any $3$-stable configuration $C=(V_1,\ldots,V_c)$ with $2$ channels for $D_{q=2}$, we have $|C(x) \cap C(y)| \neq 1$, for any $x,y \in V_{(u,v)}$.
By contradiction.
Assume there exist $x,y \in V_{(u,v)}$ such that $|C(x) \cap C(y)| = 1$.
Without loss of generality, assume that $f_x(C) \geq f_y(C)$.
Then, there exists a $1$-deviation: $y$ reaches the group $V_i$ such that $x \in V_i$ and $y \notin V_i$.
In that case, $f_y(C') > f_y(C)$, where $C'$ is the configuration for $D$ after the previous $1$-deviation.
Indeed, $f_y(C') = f_x(C) + \epsilon$.

Thus, we assume that, in any $3$-stable configuration $C=(V_1,\ldots,V_c)$ with $2$ channels for $D_{q=2}$, we have $|C(x) \cap C(y)| \neq 1$, for any $x,y \in V_{(u,v)}$.
Furthermore, if there exist $x,y \in V_{(u,v)}$ such that $|C(x) \cap C(y)| = 0$, then there exist two groups $V_{x_1}$ and $V_{x_2}$ such that $x \in V_{x_1}$, $x \in V_{x_2}$, and $V_{x_1} = V_{x_2}$, and there exist two groups $V_{y_1}$ and $V_{y_2}$ such that $y \in V_{y_1}$, $y \in V_{y_2}$, and $V_{y_1} = V_{y_2}$.
Thus, $f_x(C) = (1+\epsilon)(|V_{x_1}|-1)$, and $f_y(C) = (1+\epsilon)(|V_{y_1}|-1)$.
Without loss of generality, suppose $f_x(C) \geq f_y(C)$.
Then, there exists a $1$-deviation: $y$ leaves $V_{y_1}$ and reaches $V_{x_1}$.
We get $f_y(C') = |V_{x_1}| + |V_{y_2}| - 1 > f_y(C)$ because $\epsilon < \frac{1}{p}$.
Thus, in any $3$-stable configuration $C=(V_1,\ldots,V_c)$ with $2$ channels for $D_{q=2}$, we have for any $x,y \in V_{(u,v)}$, $|C(x) \cap C(y)| = 2$, and so, the claim is proved.\\

\noindent
Then, by the choice of $0 < \varepsilon < 1/p$ with $p > 2|V_{1}|$, there exist two groups $V_{i}$ and $V_{j}$, $1 \leq i < j \leq c$, such that $V_{i} = V_{(u,v)}$ and $V_{j} = V_{(u,v)} \cup \{u,v\}$.
Indeed, otherwise there exists a $1$-deviation for $C$, because by construction $|V_{(u,v)}| > f_{u}(C')$, with $C'$ being any configuration with $2$ channels for $D_{q=1}$.
We obtain the same result for copies $K_{u}$.
To summarize, after setting the groups from the previously necessary conditions for having a $3$-stable configuration with $2$ channels for $D_{q=1}$, each node $u \in V \setminus V_{q=1}$ belongs to exactly $2$ groups, and each node $u \in V_{q=1}$ belongs to exactly $1$ group.

Thus, there exists a $3$-stable configuration for $D_{q=2}$ with $2$ channels if, and only if, there exists a $3$-stable configuration for $D_{q=1}$ with single channel.
Indeed, any two nodes $u,v \in V_{q=1}$ such that $w_{q=1}(u,v) = 0$, are already in a same group.
Thus, by the choice of the function $h$, this mimics a weight $\varepsilon$ between these two nodes for determining the other groups, that is quite the same as a weight $0$, because $\varepsilon$ is arbitrarily small (see Corollary \ref{cor:mn}).
Finally, there does not exists a $3$-stable configuration for $D_{q=2}$ with $2$ channels because there does not exist a $3$-stable configuration for $D_{q=1}$ with single channel by Lemma~\ref{lem:counter-example}.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%


In the case of general weights, a stability criterion depending on $q$ has yet to be found.
We prove in Theorem~\ref{the:chaotic-behavior} that any chaotic behavior may be observed between any two consecutive numbers of channels.

\iffalse
\begin{lemma}
\label{lemma:counter-symmetric-1}
There exists a graph $G=(V,w)$ with $\mathcal{W}=\{-\infty,-4,2,6,7\}$.such that any partition of the nodes for $G$ is not $2$-stable.
\end{lemma}
\fi

\iffalse
\begin{proof}
Let $G_1=(V,w)$ be the graph built as follows.
Let $V=\{u_{1},u_{2},u_{3},u_{4}\}$.
We set $w_{u_{1},u_{2}} = w_{u_{1},u_{3}} = -\infty$, $w_{u_{1},u_{4}}=7$, $w_{u_{2},u_{4}}=6$, $w_{u_{3},u_{4}}=2$, and $w_{u_{2},u_{3}}=-4$.

For any $k \geq 1$, any $k$-stable partition $P$ for $G_1$ is such that $f_{u}(P) \geq 0$ for any $u \in V$.
Thus, for any $k \geq 1$, the following configurations for $G_1$ are not $k$-stable:
\begin{itemize}
\item $P=\{\{u_{1}\},\{u_{2},u_{3},u_{4}\}\}$ as $f_{u_3}(P) = -2 < 0$;
\item $P=\{\{u_{1}\},\{u_{2},u_{3}\},\{u_{4}\}\}$ as $f_{u_3}(P) = -4 < 0$;
\item $P=\{\{u_{1},u_{4}\},\{u_{2},u_{3}\}\}$ as $f_{u_3}(P) = -4 < 0$;
\item any configuration $P=\{X_{1},X_{2},X_{3},X_{4}\}$ ($X_{i}$ may be empty for some $i$, $1 \leq i \leq 4$) such that $u_{1},u_{2} \in X_{i}$ and/or $u_{1},u_{3} \in X_{i}$ for some $i$, $1 \leq i \leq 4$.
\end{itemize}

Thus, it remains to prove the result for the other configurations for $G_1$.
\begin{itemize}
\item Consider the partition $P=\{\{u_{1}\},\{u_{2}\},\{u_{3}\},\{u_{4}\}\}$ for $G_1$.
$P$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(P') = f_{u_4}(P) + 7 = 7$ where $P'=\{\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\}\}$ is the resulting configuration after this $1$-deviation.

\item Consider the partition $P=\{\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\}\}$ for $G_1$.
$P$ is not $2$-stable because $u_{2}$ and $u_{4}$ can reach group $\{u_{3}\}$.
Indeed, $f_{u_2}(P') = f_{u_2}(P) + 6 - 4 = f_{u_2}(P) + 2 = 2$ and $f_{u_4}(P') = f_{u_4}(P) -7 + 6 + 2 = f_{u_4}(P) + 1 = 8$ where $P'=\{\{u_{1}\},\{u_{2},u_{3},u_{4}\}\}$ is the resulting configuration for $G_1$ after this $2$-deviation.

\item Consider the configuration $P=\{\{u_{1}\},\{u_{2},u_{4}\},\{u_{3}\}\}$ for $G_1$.
$P$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(P') = f_{u_4}(P) -6 + 7 = f_{u_4}(P) + 1 = 7$ where $P'=\{\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\}\}$ is the resulting configuration for $G_1$ after this $1$-deviation.

\item Consider the configuration $P=\{\{u_{1}\},\{u_{2}\},\{u_{3},u_{4}\}\}$ for $G_1$.
$P$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(P') = f_{u_4}(P) -2 + 7 = f_{u_4}(P) + 5 = 7$ where $P'=\{\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\}\}$ is the resulting configuration for $G_1$ after this $1$-deviation.
\end{itemize}

Finally, any partition $P$ for $G_1$ is not a $2$-stable configuration for $G_1$.
\end{proof}
\fi

\iffalse
\begin{corollary}
\label{cor:base}
Let us fix $h$ is as $h(0,w) = 0$, $h(g+1,w) = (1 + \varepsilon g)w$, where $\varepsilon > 0$ is arbitrarily small.
Given any integer $q \geq 1$, there exists a graph $G_q=(V_q,w^q)$ with $\mathcal{W}=\{-\infty,-4,2,6,7,N\}$ such that any configuration $C$ with $q$ channels for $G_q$ is not $2$-stable, whereas there always exists a $2$-stable configuration $C'$ with $q' \neq q$ channels for $G_q$.
\end{corollary}
\fi

\iffalse
\begin{proof}
We arbitrarily select $\epsilon < 1/N$.
Let $G_1 = (V_1,w^1)$ be the graph that is presented in the proof of Lemma~\ref{lemma:counter-symmetric-1} (we re-use the same notations for the vertices in $G_1$).
We build the graph $G_q$ as follows.
First, the set of vertices is $V_q = V_1 \cup \{x_1, \ldots, x_{q-1}\}$.
For any $u,v \in V_1$, ${w_q}_{u,v} = w^1_{u,v}$.
Furthermore, for any $1 \leq i < j \leq q-1$, $w^q_{x_i,u_4} = w^q_{x_j,u_4} = N$, $w^q_{x_i,x_j} = w^q_{x_i,v} = w^q_{x_j,v} = -\infty$ for any $v \in V_1 \setminus \{u_4\}$.

We have that, for any $q' < q$, $C_{q'} = ( \{u_4,x_1\}, \ldots, \{u_4,x_{q'}\}, \{u_1\}^1, \ldots, \{u_1\}^{q'}, \{u_2\}^1, \ldots, \{u_2\}^{q'}, \{u_3\}^1, \ldots, \{u_3\}^{q'}, \{x_1\}^1, \ldots, \{x_1\}^{q'-1}, \ldots, \{x_{q'}\}^1, \ldots, \{x_{q'}\}^{q'-1}, \\\{x_{q'+1}\}^1, \ldots, \{x_{q'+1}\}^{q'}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'})$ is a $2$-stable configuration with $q'$ channels for $G_q$.

However, in any stable configuration $C_q$ with $q$ channels for $G_q$, we necessarily have $\{u_4,x_i\}$ as a group in $C_q$ (without repetitions), for any $1 \leq i \leq q-1$. As there does not exist any $2$-stable configuration with single channel for $G_1$, there does not exist any $2$-stable configuration with $q$ channels for $G_q$.

If $q' = q+1$, then $C_{q'} = ( \{u_4,x_1\}, \ldots, \{u_4,x_{q-1}\},\{u_4,u_1\}, \{u_4,u_2\}, \{u_1\}^1, \ldots, \{u_1\}^{q'-1}, \{u_2\}^1, \ldots, \{u_2\}^{q'-1}, \\\{u_3\}^1, \ldots, \{u_3\}^{q'}, \{x_1\}^1, \ldots, \{x_1\}^{q'-1}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'-1})$ is a $2$-stable configuration with $q'$ channels for $G_q$.

Finally, if $q' \geq q+2$, then $C_{q'} = ( \{u_4,x_1\}^1, \ldots, \{u_4,x_1\}^{q'-q-1}, \\\{u_4,x_2\}, \ldots, \{u_4,x_{q-1}\},\{u_4,u_1\}, \{u_4,u_2\}, \{u_4,u_3\}, \{u_1\}^1, \ldots, \\\{u_1\}^{q'-1}, \{u_2\}^1, \ldots, \{u_2\}^{q'-1}, \{u_3\}^1, \ldots, \{u_3\}^{q'-1}, \{x_1\}^1, \ldots, \\\{x_1\}^{q+1}, \{x_2\}^1, \ldots, \{x_2\}^{q'-1}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'-1})$ is a $2$-stable configuration with $q'$ channels for $G_q$.
\end{proof}
\fi

\begin{theorem}
\label{the:chaotic-behavior}
For any sequence of positive integers $q_{1}, q_{2}, \ldots, q_{p}$, and for any sequence $1 \leq i_{1} < i_{2} < \ldots < i_{l} \leq p$, there exists a graph $G=(V,w)$ such that there is a $2$-stable configuration with $q_j$ channels for $G$ if, and only if, $j \neq i_{t}$, for every $1 \leq t \leq l$.
\end{theorem}


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
For any $1 \leq t \leq l$, let $D_{q_{i_t}}$ be the graph in the proof of Corollary~\ref{cor:base} such that there exists a $2$-stable configuration with $q'$ channels for $D_{q_{i_t}}$ if, and only if, $q' \neq q_{i_t}$.
By convention, $D_0$ is any graph such that there always is a $2$-stable configuration with $q$ channels for $D_0$; for instance, we may assume that all the weights for $D_0$ are positive.

Then we build a graph $D$ from $D_0, D_{q_{i_1}}, \ldots D_{q_{i_l}}$, such that any vertices $u,v$ that are not in the same graph $D_q$ are enemies (e.g. $w(u,v) = -M$).
In so doing, every graph $D_q$ is independent of the other ones, and so, there is a $2$-stable configuration with $q'$ channels for $D$ if, and only if, there exists a $2$-stable configuration with $q'$ channels for every $D_{q_{i_t}}$, $1 \leq t \leq l$. 
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%



%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lemma:counter-symmetric-1}
Let $W=\{-M,-4,2,6,7\}$.
There exists a graph $G=(V,E,w)$ such that any configuration $C$ with single channel for $G$ is not $2$-stable.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%



%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $D=(V,A,w)$ be the graph built as follows.
Let $V=\{u_{1},u_{2},u_{3},u_{4}\}$.
We set $w(u_{1},u_{2}) = w(u_{1},u_{3}) = -M$, $w(u_{1},u_{4})=7$, $w(u_{2},u_{4})=6$, $w(u_{3},u_{4})=2$, and $w(u_{2},u_{3})=-4$.

For any $k \geq 1$, any $k$-stable configuration $C$ with single channel for $D_1$ is such that $f_{C}(u) \geq 0$ for any $u \in V$.
Thus, for any $k \geq 1$, the following configurations for $D$ are not $k$-stable:
\begin{itemize}
\item $C=(\{u_{1}\},\{u_{2},u_{3},u_{4}\})$ as $f_{u_3}(C) = -2 < 0$;
\item $C=(\{u_{1}\},\{u_{2},u_{3}\},\{u_{4}\})$ as $f_{u_3}(C) = -4 < 0$;
\item $C=(\{u_{1},u_{4}\},\{u_{2},u_{3}\})$ as $f_{u_3}(C) = -4 < 0$;
\item any configuration $C=(V_{1},V_{2},V_{3},V_{4})$ ($V_{i}$ may be empty for some $i$, $1 \leq i \leq 4$) such that $u_{1},u_{2} \in V_{i}$ and/or $u_{1},u_{3} \in V_{i}$ for some $i$, $1 \leq i \leq 4$.
\end{itemize}

Thus, it remains to prove the result for the other configurations for $D$.
\begin{itemize}
\item Consider the configuration $C=(\{u_{1}\},\{u_{2}\},\{u_{3}\},\{u_{4}\})$ for $D$.
$C$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(C') = f_{u_4}(C) + 7 = 7$ where $C'=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ is the resulting configuration with single channel for $D$ after this $1$-deviation.

\item Consider the configuration $C=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ for $D$.
$C$ is not $2$-stable because $u_{2}$ and $u_{4}$ can reach group $\{u_{3}\}$.
Indeed, $f_{u_2}(C') = f_{u_2}(C) + 6 - 4 = f_{u_2}(C) + 2 = 2$ and $f_{u_4}(C') = f_{u_4}(C) -7 + 6 + 2 = f_{u_4}(C) + 1 = 8$ where $C'=(\{u_{1}\},\{u_{2},u_{3},u_{4}\})$ is the resulting configuration for $D$ after this $2$-deviation.

\item Consider the configuration $C=(\{u_{1}\},\{u_{2},u_{4}\},\{u_{3}\})$ for $D$.
$C$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(C') = f_{u_4}(C) -6 + 7 = f_{u_4}(C) + 1 = 7$ where $C'=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ is the resulting configuration for $D$ after this $1$-deviation.

\item Consider the configuration $C=(\{u_{1}\},\{u_{2}\},\{u_{3},u_{4}\})$ for $D$.
$C$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(C') = f_{u_4}(C) -2 + 7 = f_{u_4}(C) + 5 = 7$ where $C'=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ is the resulting configuration for $D$ after this $1$-deviation.
\end{itemize}

Finally, any configuration $C$ with single channel for $D$ is not a $2$-stable configuration for $D$.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%

%%%%% DEBUT DE COROLLAIRE COMMENTE %%%%%
\iffalse
\begin{corollary}
\label{cor:base}
Let $W=\{-M,-4,2,6,7\}$.
Given an integer $q \geq 1$, there exists a graph $G_q=(V_q,E_q,w_q)$ such that any configuration $C$ with $q$ channels for $G$ is not $2$-stable, whereas there always exists a $2$-stable configuration $C'$ with $q' \neq q$ channels for $G$.
\end{corollary}
\fi
%%%%% DEBUT DE COROLLAIRE COMMENTE %%%%%


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
We arbitrarily select $\epsilon < 1/N$.
Let $D_1 = (V_1,A_1,w_1)$ be the graph that is presented in the proof of Lemma~\ref{lemma:counter-symmetric-1} (we re-use the same notations for the vertices in $D_1$).
We build the graph $D_q$ as follows.
First, the set of vertices is $V_q = V_1 \cup \{x_1, \ldots, x_{q-1}\}$.
For any $u,v \in V_1$, $w_q(u,v) = w_1(u,v)$.
Furthermore, for any $1 \leq i < j \leq q-1$, $w(x_i,u_4) = w(x_j,u_4) = N$, $w(x_i,x_j) = w(x_i,v) = w(x_j,v) = -M$ for any $v \in V_1 \setminus \{u_4\}$.

We have that, for any $q' < q$, $C_{q'} = ( \{u_4,x_1\}, \ldots, \{u_4,x_{q'}\}, \\\{u_1\}^1, \ldots, \{u_1\}^{q'}, \{u_2\}^1, \ldots, \{u_2\}^{q'}, \{u_3\}^1, \ldots, \{u_3\}^{q'}, \\ \{x_1\}^1, \ldots, \{x_1\}^{q'-1}, \ldots, \{x_{q'}\}^1, \ldots, \{x_{q'}\}^{q'-1}, \\\{x_{q'+1}\}^1, \ldots, \{x_{q'+1}\}^{q'}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'})$ is a $2$-stable configuration with $q'$ channels for $D_q$.

However, in any stable configuration $C_q$ with $q$ channels for $D_q$, we necessarily have $\{u_4,x_i\}$ as a group in $C_q$ (without repetitions), for any $1 \leq i \leq q-1$. As there does not exist any $2$-stable configuration with single channel for $D_1$, there does not exist any $2$-stable configuration with $q$ channels for $D_q$.

If $q' = q+1$, then $C_{q'} = ( \{u_4,x_1\}, \ldots, \{u_4,x_{q-1}\},\\\{u_4,u_1\}, \{u_4,u_2\}, \{u_1\}^1, \ldots, \{u_1\}^{q'-1}, \{u_2\}^1, \ldots, \{u_2\}^{q'-1}, \\\{u_3\}^1, \ldots, \{u_3\}^{q'}, \{x_1\}^1, \ldots, \{x_1\}^{q'-1}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'-1})$ is a $2$-stable configuration with $q'$ channels for $D_q$.

Finally, if $q' \geq q+2$, then $C_{q'} = ( \{u_4,x_1\}^1, \ldots, \{u_4,x_1\}^{q'-q-1}, \\\{u_4,x_2\}, \ldots, \{u_4,x_{q-1}\},\{u_4,u_1\}, \{u_4,u_2\}, \{u_4,u_3\}, \{u_1\}^1, \ldots, \\\{u_1\}^{q'-1}, \{u_2\}^1, \ldots, \{u_2\}^{q'-1}, \{u_3\}^1, \ldots, \{u_3\}^{q'-1}, \{x_1\}^1, \ldots, \\\{x_1\}^{q+1}, \{x_2\}^1, \ldots, \{x_2\}^{q'-1}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'-1})$ is a $2$-stable configuration with $q'$ channels for $D_q$.
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%




==> Long/SAUVEGARDE/oldabstract.tex <==
Various social networks, and some computational problems, require the formation of groups in the presence of \emph{de facto} antagonistic relationships denoting local incompatibility.
This can be posed as a vertex graph coloring problem, and the configurations attainable under these constraints through coordinated algorithms (\eg aiming to use the least amount of colors) are well characterized. In contrast, when groups are formed in a distributed manner by self-interested nodes, we know surprisingly little of the configurations that emerge from the dynamics of such a \emph{coloring game}. Collusions -- multiple players joining a new group together so that they \emph{all} improve their scores -- are likely to occur in such group formation settings; they greatly affect the stability and efficiency of the configurations. 

This paper characterizes the convergence of coloring games, revealing their intricate complexity properties and proving that previous bounds are arbitrarily loose. First, in a uniform game, we show that sequences of moves relate to physics models of condensed matter and integer partition. Moreover, we prove that combinatorial complexity of coloring games suddenly increases: no polynomial bound exists should this analysis fails. This solves an open problem and explains the failure of previous proposed methods using potential functions. In non-uniform games where nodes preferences are given in a set of weights, we prove generally the maximum collusion size that guarantees convergence. As we show, deciding the convergence beyond this point is never computationally feasible. 
Our results extend to variants where nodes join multiple groups, have asymmetrical weights, and utility goes beyond pair-wise relationship. Finally, we show these games create a tension between stability and efficiency, as collusions and the use of  multiple colors both have a beneficial effect on the price of anarchy.

==> Long/SAUVEGARDE/unweighted-long-k=3,4-SAUVEGARDE.tex <==


\subsection{Non polynomial lower bound for k > 3}

As seen above, we already showed that $L(4,n)=O(e^{\sqrt{n}})$, which is already much better than what additive potential function methods can attain~\cite{Kleinberg:2010ul}.
However, the computational cost of $4$-deviations is unknown. We resolve this problem by proving $L(4,n)$ cannot be bounded polynomially.

\begin{theorem}
\label{lem:lower-bound-4}
$L(4,n) = \Omega(n^{a\ln(n)})$ where $a>0$.
\end{theorem}

\begin{proof}
Let $G^{\emptyset}=(V,E)$ with $|E|=0$.
Suppose $n=|V|=cL$ where $c,L$ are positive integers.
We first construct a partition $C^{0}$ for $G^{\emptyset}$ for which the vector of partition $v(C^{0})=(v_{1}, v_{2}, \ldots, v_{n})$ is such that for any $j$, $1 \leq j \leq L$, $v_{j} = c$, and for any $j$, $L+1 \leq j \leq n$,   $v_{j} = 0$.
Clearly this partition can be obtained with a sequence of $1$-deviations.
In the following, we only consider groups of sizes at most $L$.

We introduce the notion of \emph{reverse vector of difference}.
Starting from partition $C^{0}$, we define the initial reverse vector of difference as $v^{0} = (v^{0}(1),v^{0}(2),\ldots, v^{0}(L))$ where, for any $j$, $1 \leq j \leq L$, $v^{0}(j)=v_{L-j+1}-c$ represents the number of groups of size $L-j+1$ minus the initial number $c$.
The vector of difference $v$ for a configuration $C$, is such that, for any $j$, $1 \leq j \leq L$, $v(j)$ represents the difference between the number of groups of size $L-j+1$ that have been created and the number of groups of size $j$ that have been removed, in the sequence of deviations from $v^{0}$ to $v$.


A reverse vector of difference $v$ is \emph{c-balanced} if, for any $j$, $1 \leq j \leq L$, $v(j) \geq -c$.
Any sequence of deviations must induce a $c$-balanced vector (there are exactly $c$ groups of each size at most $L$ at the beginning).

%We consider vector of difference instead of configurations or partitions.

%such that $l(1) > 2^{T+1}3$ and $2^{T-1}l(1) \leq L$.








We only consider $4$-deviations that consist in creating five groups of sizes $p$, $p-2$, $p-2$, $p-2$, $p-2$, and removing five groups of sizes $p-4$, $p-1$, $p-1$, $p-1$, $p-1$ for some $p$, $5 \leq p \leq L$.
We consider such a $4$-deviation because it strictly decreases the global utility and so it will allow us to construct long sequences.
We define an elementary vector of difference $\phi_{L-p+1}$ of size $L$: $\phi_{L-p+1} = (\ldots,1,-4,4,0,-1,\ldots)$
where dots represent $0$ values, $1$ corresponds to the group of size $p$ that has been created, $-4$ corresponds to the four groups of size $p-1$ that have been removed, etc.
The first $1$ at index $L-p+1$ means that a group of $L-p+1$ has been created, $-4$ is at index $L-p+2$, etc.
Given a reverse vector of difference $v$ (corresponding to a current partition $C$), the reverse vector of difference $v'$ for $C'$ obtained after a $4$-deviation for $C$, is $v' = v + \phi_{L-p+1}$.

In other words,
\begin{equation*}
\phi_{L-p+1}(j) =
\begin{cases}
1 & \mbox{if $j = L-p+1$} \\
-4 & \mbox{if $j = L-p+2$} \\
4 & \mbox{if $j = L-p+3$} \\ 
-1 & \mbox{if $j = L-p+5$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}

%redefined above
\iffalse
We associate with any such a $4$-deviation, an elementary reverse vector of difference $\phi_{L-p+1}$ is  defined as follows:
$\phi_{p}(L-p+1) = 1$,
$\phi_{p}(L-p+2) = -4$,
$\phi_{p}(L-p+3) = 4$,
$\phi_{p}(L-p+5) = -1$,
$\phi_{p}(j) = 0$ for any $j$, $1 \leq j \leq L$, $j \notin \{L-p+1, L-p+2,L-p+3,L-p+5\}$.
\fi

We define notations for $1$-deviations that consist in creating two groups of sizes $p$, $q$, and removing two groups of sizes $p-1$, $q+1$, for some $p, q$, $3 \leq q+2 \leq p \leq L$.
We define an elementary vector of difference $\phi_{L-p+1,L-q+1}$ of size $L$: \\
\vspace{-0.2cm}
\begin{equation*}
\phi_{L-p+1,L-q+1} =
\begin{cases}
(\ldots,1,-1,\ldots,-1,1,\ldots) & \mbox{if $p > q+2$} \\
(\ldots,1,-2,1,\ldots) & \mbox{if $p = q+2$}
\end{cases}
\end{equation*}
where the first $1$ (index $L-p+1$) corresponds to the group of size $p$ that has been created.
The second value $1$ (index $L-q+1$) corresponds to the group that has been created.


In other words,
\begin{equation*}
\phi_{L-p+1,L-q+1}(j) =
\begin{cases}
1 & \mbox{if $j = L-p+1$} \\
-1 & \mbox{if $j = L-p+2$} \\
-1 & \mbox{if $j = L-q$} \\ 
1 & \mbox{if $j = L-q+1$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}






We now define a particular sequence of $1$-deviations.
For any $j_{1}, j_{2}, d$ such that $1 \leq j_{1} < j_{1}+d \leq j_{2}-d < j_{2} \leq L$, we define $\phi_{j_{1},j_{1}+d,j_{2}-d,j_{2}} = \sum_{j=0}^{d-1} \phi_{j_{1}+j,j_{2}-j } =$

\vspace{-0.3cm}

\begin{equation*}
%\phi_{j_{1},j_{1}+d,j_{2}-d,j_{2}} =
\begin{cases}
(\ldots,1,\ldots,-1,\ldots,-1,\ldots,1,\ldots) & \mbox{if $j_{1}+d \neq j_{2}-d$} \\
(\ldots,1,\ldots,-2,\ldots,1,\ldots) & \mbox{if $j_{1}+d = j_{2}-d$}
\end{cases}
\end{equation*}

\vspace{-0.1cm}

Given a reverse vector of difference $v$ and an integer $r$, $1 \leq r \leq L$, we define $v'=\Phi(v,r)$ as follows:
\vspace{-0.1cm}
\begin{equation*}
\begin{cases}
\mbox{$v'(j+r-1) = v(j)$} & \mbox{$\forall j$, $1 \leq j \leq L-r+1$,} \\
\mbox{$v'(j)=0$} & \mbox{$\forall j$, $1 \leq j < r$.}
\end{cases}
\end{equation*}

\vspace{-0.1cm}

The size $s$ of a reverse vector of difference $v$ is such that $v(s) \neq 0$ and $v(j) = 0$ for any $j$, $s+1 \leq j \leq L$.

We define the notion of \emph{symmetric vector}.
A reverse vector of difference $v$ is symmetric if for any $j$, $1 \leq j \leq s$, $v(j)=v(s-j+1)$ where $s$ is the size of $v$.
%Note that $v^{1}$ is symmetric.
%We prove a useful claim.

\begin{claim}
\label{claim:symmetry}
Let $v$ be any symmetric vector of difference of size $s$.
Then, for any positive integers $r$ and $d$, $1+(r-1)d \leq s$, $v' = \sum_{h=0}^{r-1} \Phi(v,1+h d)$ is a symmetric vector.
\end{claim}

\begin{proof}
Vector $v'$ has size $s' = (r-1)d+s$.
Let first suppose that $r$ is even.
$v' = \sum_{h=0}^{r/2-1} \Phi(v,1+h d) +  \sum_{h=r/2}^{r-1} \Phi(v,1+h d)$.
We prove that, for any $r'$, $0 \leq r' \leq r/2-1$, $y_{r'} = \sum_{h=0}^{r'} \Phi(v,1+h d) +  \sum_{h=r-1-r'}^{r-1} \Phi(v,1+h d)$ is a symmetric vector.
Note that the size of $y_{r'}$ is $s' = (r-1)d+s$ for any $r'$, $0 \leq r' \leq r/2-1$.

By induction on $r'$.
Suppose $r'=0$.
We have $y_{0} = \Phi(v,1)+\Phi(v,1+(r-1)d)$.
For any $j$, $1 \leq j \leq (r-1)d+s$, $y_{0}(j)=v(j)+v(j-(r-1)d)$.
As $v$ is a symmetric vector of size $s$, then $v(j-(r-1)d) = v(s-j+(r-1)d+1)$, and so $v(j-(r-1)d) = v(s'-j+1)$ because $y_{0}$ has size $s'$.
Thus, we get $y_{0}(j)=v(j)+v(s'-j+1)$.
We deduce that $y_{0}(s'-j+1)=v(s'-j+1)+v(s'-(s'-j+1)+1)$, and so $y_{0}(s'-j+1)=v(s'-j+1)+v(j)$.
As a result, $y_{0}$ is a symmetric vector.

Suppose it is true for $r'$, $0 \leq r' \leq r-2$, we prove it is also true for $r'+1$.
Vector $y_{r'}$ is a symmetric vector.
We have $y_{r'+1} = y_{r'} + \Phi(v,1+(r'+1) d)+ \Phi(v,1+(r-r'-2) d)$.
First, if $j \leq (r+1)d$, then $y_{r'+1}(j)-y_{r'}(j) = 0$ by construction.
Also, $y_{r'+1}(j)-y_{r'}(j) = 0$ for any $j$, $(r-r'-2)d+s \leq j \leq s'$.
For any $j$, $1 \leq j \leq (r-1)d+s$, $y_{r'+1}(j)-y_{r'}(j)=v(j-(r'+1)d)+v(j-(r-r'-2) d)$.
Let $x_{1} = (r+1)d+1$ and let $x_{2}=(r-r'-2)d+s-1$.
Consider the sub-vector $y'_{r'}$ of $y_{r'}$ defined as follows: $y'_{r'}=(y_{r'}(x_{1}), y_{r'}(x_{1}+1), \ldots, y_{r'}(x_{2}-1), y_{r'}(x_{2}))$.
Clearly $y'_{r'}$ is a symmetric vector because $x_{1}-1=s'-x_{2}$.
Thus, we can apply proof for case $r'=0$ to show that $y'_{r'+1} = \Phi(v,1+(r'+1) d)+ \Phi(v,1+(r-r'-2) d)$ is a symmetric vector.
So $y_{r'+1}$ is a symmetric vector.


Finally, for any $r'$, $0 \leq r' \leq r/2-1$, $y_{r'}$ is a symmetric vector.
We get that $v'$ is a symmetric vector.

Consider now that $r$ is odd.
We set $v''= \sum_{h=0}^{(r-1)/2-1} \Phi(v,1+h d) +  \sum_{h=(r-1)/2+1}^{r-1} \Phi(v,1+h d)$.
Using the previous induction, we prove that $v''$ is symmetric vector.
We now prove that $v' = v'' + \Phi(v,1+d(r-1)/2)$ is a symmetric vector.
Let $v''' = \Phi(v,1+d(r-1)/2)$.
We have $v'''(j)=v'''((r-1)d+s-j)$ because $d\frac{r-1}{2}+1-1=d(r-1)+s-d\frac{r-1}{2}-s$.
Finally, $v'$ is a symmetric vector because $v''$ is symmetric.
\end{proof}







Let $l(1), T \geq 1$ be any two integers such that $2^{T-1} l(1) \leq L$.
We will explain this choice at the end of the proof.
For any $i$, $1 \leq i \leq T-1$, we construct the vector $v^{i+1}$ from $v^{i}$ such that these vectors have a special property, called \emph{Good Property} (Definition~\ref{def:good}).


%Note that $v^{1}$ is obtained with a special construction that is not explained here.
%The vector $v^{1}$ has been constructed by applying consecutive $4$-deviations: $\phi_{1}, \phi_{2}, \phi_{3}, \ldots$


We first construct $v_{1}$.
Let $t = l(1)-1$.

We now construct $z^{1} = (\sum_{j=1}^{t} \phi_{j})+\phi_{2,3,3,4} + \phi_{t+1,t+2,t+2,t+3} + \phi_{t+4,t+5,t+6,t+7} + \phi_{2,4,4,6}$.
For any $j$, $1 \leq j \leq L$:
\begin{equation*}
z^{1}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-1 & \mbox{if $j = 2$} \\
-1 & \mbox{if $j = 3$} \\
1 & \mbox{if $j = 6$} \\
1 & \mbox{if $j = t+2$} \\
-1 & \mbox{if $j = t+5$} \\
-1 & \mbox{if $j = t+6$} \\
1 & \mbox{if $j = t+7$} \\
0 & \mbox{if $j \notin \{1,2,3,6,t+2,t+5,t+6,t+7\}$}
\end{cases}
\end{equation*}

We now construct $z^{2} = \sum_{j=1}^{t-4} \Phi(z^{1},j)$.
For any $j$, $1 \leq j \leq L$:
\begin{equation*}
z^{2}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-1 & \mbox{if $j = 3$} \\
-1 & \mbox{if $j = 4$} \\
-1 & \mbox{if $j = 5$} \\
-1 & \mbox{if $j = t-3$} \\
1 & \mbox{if $j = t-1$} \\
1 & \mbox{if $j = t$} \\
1 & \mbox{if $j = t+1$} \\
1 & \mbox{if $j = t+2$} \\
1 & \mbox{if $j = t+3$} \\
1 & \mbox{if $j = t+4$} \\
-1 & \mbox{if $j = t+6$} \\
-1 & \mbox{if $j = 2t-2$} \\
-1 & \mbox{if $j = 2t-1$} \\
-1 & \mbox{if $j = 2t$} \\
1 & \mbox{if $j = 2t+2$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}

%We get:
%$z^{2}(1) = 1$,
%$z^{2}(3) = -1$,
%$z^{2}(4) = -1$,
%$z^{2}(5) = -1$,
%$z^{2}(t-4) = 1$,
%$z^{2}(t-2) = 1$,
%$z^{2}(t-1) = 1$,
%$z^{2}(t) = 1$,
%$z^{2}(j) = 0$ for any $j$, $1 \leq j \leq t$, $j \notin \{1,3,4,5,t-4,t-2,t-1,t,\}$,
%and $z^{2}(2t-j+1) = z^{2}(j)$ for any $j$, $1 \leq j \leq t$.


We finally construct $v^{1} = z^{2} + \phi_{5,t,t+3,2t-2} + 
\phi_{t-3,t-1,t+4,t+6}$.

For any $j$, $1 \leq j \leq L$:
\begin{equation*}
v^{1}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-1 & \mbox{if $j = 3$} \\
-1 & \mbox{if $j = 4$} \\
1 & \mbox{if $j = t+1$} \\
1 & \mbox{if $j = t+2$} \\
-1 & \mbox{if $j = 2t-1$} \\
-1 & \mbox{if $j = 2t$} \\
1 & \mbox{if $j = 2t+2$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}


The intuitive idea is that such consecutive $4$-deviations, called \emph{cascade}, balance the vector of difference.
$v^{1}$ has the Good Property and Claim~\ref{claim:c-0-balanced} shows that each vector of difference from $v^{0}$ to $v^{1}$ is $c_{1}$-balanced (for some constant $c_{1}$).

For any $i$, $1 \leq i \leq T-1$, we denote by $s^{i}$ the size of the reverse vector of difference $v^{i}$, and set $l(i)=s^{i}/2$.
Note that the size of $v^{1}$ depends on the choice of $l(1)$, $s^{1}=2l(1)$.


\begin{definition}
\label{def:good}
$v^{i}$ has the Good Property if $s^{i}$ is even and if there exists $t^{i}_{1}$, $t^{i}_{2}$ with $1 < t^{i}_{1} < t^{i}_{2} < 2 t^{i}_{1}-1$, $t^{i}_{2} \leq 2^{i}$, such that for any $j$, $1 \leq j \leq L$:
\begin{equation*}
v^{1}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-1 & \mbox{if $j = t^{i}_{1}$} \\
-1 & \mbox{if $j = t^{i}_{2}$} \\
1 & \mbox{if $j = l(i)$} \\
1 & \mbox{if $j = l(i)+1$} \\
-1 & \mbox{if $j = 2l(i)-t^{i}_{2}+1$} \\
-1 & \mbox{if $j = 2l(i)-t^{i}_{1}+1$} \\
1 & \mbox{if $j = 2l(i)$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}
\end{definition}


\begin{claim}
\label{claim:c-0-balanced}
There exists a constant $c_{1}$ such that every reverse vector of difference from $v^{0}$ to $v^{1}$, is $c_{1}$-balanced.
\end{claim}

%We first construct the reverse vector of difference $v^{1}$ from $v^{0}$ before constructing our generic sequence of deviations.

%Note that $v^{1}$ has the Good Property.




In order to build $v^{i+1}$ from $v^{i}$, we define an intermediary construction.
For any $i$, $1 \leq i \leq T-1$, we define $u^{i+1} = \sum_{j=0}^{\alpha(i)} \Phi(v^{i},1+j (t^{i}_{1}-1))$ where $\alpha(i)$ is the largest even integer $j$ such that $t^{i}_{2} + j(t^{i}_{1}-1) < l(i)$.
We now prove that if $v^{i}$ has the Good Property, then it is possible to construct $u^{i+1}$ and $v^{i+1}$ such that $v^{i+1}$ has the Good Property.
We will prove in Claim~\ref{claim:c-balanced} that our constructive proof makes each vector of difference $c$-balanced (for some $c$ defined later).

Figure~\ref{fig:cascade} represents the construction of $u^{2}$ (and $v^{2}$) from the vector $v^{1}$.
The vector $v^{1}$ is applied a larger number of times and the starting point is shifted in order to balance the vectors of differences.
This cascade technique is used recursively.
The vector $v^{3}$ is obtained by applying a cascade of vectors $v^{2}$, and so on.
We prove that this construction uses a large number (non polynomial) of deviations and as the vector will be enough balanced, the number of nodes will remain small compared to the number of deviations. 



\begin{figure}[t]
\centerline{%\includegraphics[width=0.5\linewidth]{Figures/Unstablek4noborder.pdf}
\includegraphics[width=1\linewidth]{Figures/Sequencek4.pdf}}
\caption{Long sequence using recursive cascades.}
\vspace{-0.25cm}
\label{fig:cascade}
\end{figure}

\vspace{-0.1cm}

\begin{claim}
\label{claim:etape-induction}
For any $i$, $1 \leq i \leq T-1$, if $v^{i}$ has the Good Property, then there exists a sequence of deviations from $u^{i+1}$ to $v^{i+1}$ such that $v^{i+1}$ has the Good Property.
\end{claim}
\vspace{-0.3cm}
\begin{proof}
For some $i$, $1 \leq i \leq T-1$, suppose that $v^{i}$ has the Good Property.
By construction there exists $t^{i+1}_{1}$ and $t^{i+1}_{2}$ such that, for any $j$, $1 \leq j \leq t^{i+1}_{2}$:
\begin{equation*}
u^{i+1}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-1 & \mbox{if $j = t^{i+1}_{1}$} \\
-1 & \mbox{if $j = t^{i+1}_{2}$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}
where $t^{i+1}_{1}=t^{i}_{2}$ and $t^{i+1}_{2}=2t^{i}_{1}-1$.

%By construction $u^{i+1}(1) = 1$, $u^{i+1}(t^{i+1}_{1})=u^{i+1}(t^{i+1}_{2})=-1$, and $u^{i+1}(j) = 0$ for other $j \leq t^{i+1}_{2}$ where $t^{i+1}_{1}=t^{i}_{2}$ and $t^{i+1}_{2}=2t^{i}_{1}-1$.

We get $1 < t^{i+1}_{1} < t^{i+1}_{2}$ because $1 < t^{i}_{2} < 2t^{i}_{1}-1$ by hypothesis.
Also, $t^{i+1}_{2} < 2 t^{i+1}_{1}-1$ because $2t^{i}_{1}-1 < 2 t^{i}_{2}-1$.
Finally, $t^{i+1}_{2} \leq 2^{i+1}$ because $t^{i+1}_{2} < 2t^{i+1}_{1} = 2t^{i}_{2} \leq 2^{i}2$.
By Claim~\ref{claim:symmetry}, we obtain the properties for the end of the vector.

Note that $l(i+1) \leq 2 l(i)$.
Furthermore $s^{i+1}=\alpha(i)(t^{i}_{1}-1)+s^{i}$.
As $\alpha(i)$ and $s^{i}$ are even integers, then $s^{i+1}$ is even.

By Claim~\ref{claim:symmetry}, we get that $u^{i+1}$ is a symmetric vector, that is for any $j$, $1 \leq j \leq 2l(i+1)$, $u^{i+1}(j)=u^{i+1}(2l(i+1)-j+1)$.
Furthermore, by the choice of $\alpha(i)$, we get that there exist $j_{1}, j_{2}$, $t^{i+1}_{2} < j_{1} < j_{2} < 2l(i)-t^{i}_{1}+1$, such that for any $j$, $t^{i+1}_{2} \leq j \leq 2l(i)-t^{i}_{1}+1$:
\begin{equation*}
u^{i+1}(j) \in 
\begin{cases}
\{-1,0\} & \mbox{if $t^{i+1}_{2} < j \leq j_{1}$} \\
\{0,1\} & \mbox{if $j_{1} < j < j_{2}$} \\
\{-1,0\} & \mbox{if $j_{2} \leq j < 2l(i)-t^{i}_{1}+1$}
\end{cases}
\end{equation*}


%for any $j$, $t^{i+1}_{2} < j \leq j_{1}$, $u^{i+1}(j) \in \{-1,0\}$; \\
%for any $j$, $j_{1} < j < j_{2}$, $u^{i+1}(j) \in \{0,1\}$; \\
%for any $j$, $j_{2} \leq j < 2l(i)-t^{i}_{1}+1$, $u^{i+1}(j) \in \{-1,0\}$.\\

\noindent
Furthermore:\\
$\sum_{j=t^{i+1}_{2}+1}^{j_{1}} u^{i+1}(j)
+\sum_{j=j_{2}}^{2l(i)-t^{i}_{1}} u^{i+1}(j) = -\sum_{j=j_{1}+1}^{j_{2}-1} u^{i+1}(j)$.

As $u^{i}(l(1))=1$, $u^{i+1}(l(i)+\frac{\alpha(i)}{2}(t^{1}_{1}-1))=1$.
Also, $u^{i+1}(l(i)+1+\frac{\alpha(i)}{2}(t^{1}_{1}-1))=1$.
As $\alpha(i)$ is even, we get $u^{i+1}(l(i+1))=1$ because $l(i)+\frac{\alpha(i)}{2}=\frac{s^{i+1}}{2}$.
Recall that $s^{i+1}=\alpha(i)(t^{i}_{1}-1)+s^{i}$.
Thus, $u^{i+1}(l(i+1)+1)=1$.

We now prove that there exists a sequence of $1$-deviations in order to construct $v^{i+1}$ with the Good Property.
As $u^{i+1}$ is a symmetric vector (Claim~\ref{claim:symmetry}), if $u^{i+1}(j)=-1$ for any $j$, $t^{i+1}_{2} < j \leq j_{1}$, then $u^{i+1}(2l(i+1)-j+1)=-1$.
Let $j$ such that $u^{i+1}(j)=-1$ and $t^{i+1}_{2} < j \leq j_{1}$.
By previous remark and again by symmetry, there exists $j'$, $j_{1} < j' < j_{2}$, $j' \notin \{l(i+1),l(i+1)+1\}$, such that $u^{i+1}(j') = u^{i+1}(2l(i+1)-j'+1)=1$.

We construct $z^{i+1}_{1} = u^{i+1} + \phi_{j,j',2l(i+1)-j'+1,2l(i+1)-j+1}$.
This construction clearly keeps the symmetry property.
As $\sum_{j=t^{i+1}_{2}+1}^{j_{1}} u^{i+1}(j)
+\sum_{j=j_{2}}^{2l(i)-t^{i}_{1}} u^{i+1}(j) = -\sum_{j=j_{1}+1}^{j_{2}-1} u^{i+1}(j)$, then we can find another $4$-uplet $(j,j',2l(i+1)-j'+1,2l(i+1)-j+1)$, $j' \notin \{l(i+1),l(i+1)+1\}$, to construct
$z^{i+1}_{2} = z^{i+1}_{1} + \phi_{j,j',2l(i+1)-j'+1,2l(i+1)-j+1}$.
And so on until $v^{i+1} = z^{i+1}_{f}$ where $f = \frac{1}{2}\sum_{j=j_{1}+1}^{j_{2}-1} u^{i+1}(j)$

The vector of difference $v^{i+1}$ has the Good Property.
%such that for any $j \geq 1$, $v^{i+1}(j)=0$ but
%$v^{i+1}(1)=1$,
%$v^{i+1}(t^{i+1}_{1})=-1$, 
%$v^{i+1}(t^{i+1}_{2})=-1$, 
%$v^{i+1}(l(i+1))=1$,
%$v^{i+1}(l(i+1)+1)=1$, 
%$v^{i+1}(2l(i+1)-t^{i+1}_{2}+1)=-1$,
%$v^{i+1}(2l(i+1)-t^{i+1}_{1}+1)=-1$, and 
%$v^{i+1}(2l(i+1))=1$.
%So $v^{i+1}$ has the good Property.
\end{proof}



%\begin{claim}
%\label{claim:property-v-i}
%For any $i$, $1 \leq i \leq T-1$, we can construct $v^{i+1}$ from $u^{i+1}$ (itself obtained from $v^{i}$) such that $v^{i+1}$ has the Good Property.
%\end{claim}

%\begin{proof}
%We prove the result by induction.
%As seen before, $v^{1}$ has the Good property.
%Suppose now it is true for any $i' \leq i$.
%We prove it is true for $i+1$.
%By Claim~\ref{claim:etape-induction}, we can construct $v^{i+1}$ from $u^{i+1}$ such that $v^{i+1}$ has the Good Property.
%\end{proof}

\vspace{-0.2cm}

As $v^{1}$ has the Good Property, we deduce that for any $i$, $1 \leq i \leq T$, $v^{i}$ has the Good Property.

\vspace{-0.1cm}

\begin{claim}
\label{claim:c-balanced}
For any $i$, $1 \leq i \leq T$, any vector $v$ of difference in the sequence from $v^{0}$ to $v^{i}$, is $(c_{1}+i-1)$-balanced where $c_{1}$ is the constant defined in Claim~\ref{claim:c-0-balanced}.
\end{claim}
\begin{proof}
%Let $c_{1}$ be a constant such that vectors of difference are $c_{1}$-balanced before obtaining vector of difference $v_{1}$, that is for all the vectors from $v^{0}$ to $v^{1}$.
We prove the result by induction on $i$.
The vector $v^{0}$ is $0$-balanced by definition.
Claim~\ref{claim:c-0-balanced} proves the result for $i=1$.
Suppose it is true for any $i' \leq i \leq T-1$.
We prove that it is true for $i+1$.
%Suppose that the current vector of difference is $v^{i}$.
We construct $v^{i+1}$ from $v^{i}$ as described in the proof of Claim~\ref{claim:etape-induction}.
Recall that we first build $u^{i+1} = \sum_{j=0}^{\alpha(i)} \Phi(v^{i},1+j (t^{i}_{1}-1))$ where $\alpha(i)$ is the largest even integer $j$ such that $t^{i}_{2} + j(t^{i}_{1}-1) < l(i)$.

For any $b$, $0 \leq b \leq \alpha(i)-1$, consider $y^{i+1}_{b} = \sum_{j=0}^{b}\Phi(v^{i},1+j (t^{i}_{1}-1))$.
We prove that each vector of difference from $v^{i}$ to $y^{i+1}_{b}$ is $(c_{1}+i)$-balanced.
By induction on $b$.
%We prove by induction that each vector of difference before reaching configuration corresponding to $u'_{b}$ is $(c_{1}+i)$-balanced.
%By induction on $b$.
It is true for $b=0$.
Indeed by the first induction hypothesis, each vector of difference from $v^{0}$ to $\Phi(v^{i},1)$, is $(c_{1}+i-1)$-balanced.
Suppose it is true for any $b' \leq b \leq \alpha(i)-1$.
We prove it is true for $b+1$.
By Claim~\ref{claim:etape-induction}, $y^{i+1}_{b}$ is $1$-balanced because $\Phi(v^{i},1)$ is $1$-balanced (the values of the vector belong to the set $\{-1,0,1\}$).
By definition $y^{i+1}_{b+1}=y^{i+1}_{b}+\Phi(v^{i},1+(b+1)(t^{i}_{1}-1))$.
By the first induction hypothesis, each sequence of $\Phi(v^{i},1+(b+1)(t^{i}_{1}-1))$ is $(c_{1}+i-1)$-balanced.
Since $y^{i+1}_{b}$ is $1$-balanced, each vector of difference from $y^{i+1}_{b}$ to $y^{i+1}_{b+1}$, is $(c_{1}+i)$-balanced.
Thus, $u^{i+1}$ is $(c_{1}+i)$-balanced.

To conclude, it remains to prove that each vector of difference from $u^{i+1}$ to $v^{i+1}$, is $(c+i)$-balanced.
Consider the last $1$-deviations described in the proof of Claim~\ref{claim:etape-induction}.
Every deviation consists in replacing values $-1$ and $1$ by $0$.
Thus, $v^{i+1}$ is $(c+i)$-balanced.
%, and that concludes the first induction proof.
\end{proof}






For any $i$, $1 \leq i \leq T$, let $S_{i}$ be the sequence of deviations from $v^{0}$ to $v^{i}$.


\begin{claim}
\label{claim:taille-de-l}
For any $i$, $1 \leq i \leq T-1$, $l(i) \leq 2^{i-1} l(1)$.
\end{claim}

\begin{proof}
By induction on $i$.
It is clearly true for $i = 1$.
Suppose it is true for any $i' \leq i$.
We prove it is true for $i+1$.
By construction, $l(i+1) \leq 2l(i)$.
Thus, $l(i+1) \leq 2^{i-1} 2 l(1)$ by induction hypothesis.
Finally we get $l(i+1) \leq 2^{i} l(1)$.
\end{proof}






\begin{claim}
\label{claim:taille-sequence-1}
For any $i$, $1 \leq i \leq T-1$, $|S_{i+1}| \geq (\frac{l(i)}{2^{i}} -3) |S_{i}|$.
\end{claim}

\begin{proof}
$|S_{i+1}| = \alpha(i) |S_{i}|$ with $\alpha(i)$ is the largest even integer $j$ such that $t^{i}_{2} + j(t^{i}_{1}-1) < l(i)$.
%We get $\alpha(i)=\lfloor \frac{l(i)-t^{1}_{2}}{t^{i}_{1}-1}-1 \rfloor + 1$.
Thus $\alpha(i) \geq \lfloor \frac{l(i)-2^{i+1}+1}{2^{i}-1}\rfloor$ because $t^{i}_{1}, t^{i}_{2} \leq 2^{i}$.
So $|S_{i+1}| \geq (\frac{l(i)}{2^{i}} -3) |S_{i}|$. 
\end{proof}




\begin{claim}
\label{claim:taille-sequence-2}
For any $i$, $1 \leq i \leq T-1$, and for any $l(1) > 2^{i+1}3$, then $|S_{i}| \geq \frac{l(1)^{i-1}|S_{1}|}{2^{i}}$.
\end{claim}

\begin{proof}
First note that $l(1) \geq l(i)$ for any $i \geq 1$.
As $l(1) > 2^{i+1}3$, we get that $\frac{l(i)}{2^{i}} -3 \geq \frac{l(i)}{2^{i+1}}$.
By Claim~\ref{claim:taille-sequence-1}, we get $|S_{i+1}| \geq \frac{l(i)}{2^{i+1}} |S_{i}|$.
Thus, $|S_{i}| \geq \frac{l(1)^{i-1}|S_{1}|}{2^{i}}$.
\end{proof}



We proved that $|S_{T}| \geq \frac{l(1)^{T-1}|S_{1}|}{2^{T}}$ and $l(T) \leq 2^{T-1} l(1)$.

By Claim~\ref{claim:c-balanced}, $c = c_{1}+T-1$ guarantees the feasibility of the sequence of deviations from $v^{0}$ to $v^{T}$.
Thus, $n = 2^{T-1} l(1) (c_{1}+T-1)$ is sufficient to construct a valid  sequence.
For any $l(1)$, set $T = \lfloor log_2(l(1)/6) \rfloor -1$.
We choose $L \geq 2^{T-1}l(1)$ as consequence.
We obtain that for any $n$, there exists a sequence of $1$ and $4$-deviations $S$ of length $\Omega(n^{a log_{2}(n)})$ for some constant $a > 0$.
$\qed$
\end{proof}





\subsection{k=3}

We prove a lower bound when $k=3$ using the same techniques.
Obviously, we cannot apply cascades a large number of times since any sequence of $3$-deviations is of size $O(n^{3})$.




\begin{lemma}
\label{lem:lower-bound-3}
$L(3,n) = \Omega(n^{2})$.
\end{lemma}

\begin{proof}
Recall that any partition $\P$ is represented by $\Lambda=(\lambda_{n}, \ldots, \lambda_{i}, \ldots, \lambda_{1})$ where $\lambda_{i}$ represents the number of groups of size $i$,  $1 \leq i \leq n$.
We only consider $3$-deviations that consist in creating $1$ group of size $p$, removing $3$ groups of size $p-1$, creating $3$ groups of $p-2$, and removing $1$ group of size $p-3$, for some $p$.
More precisely we focus on $3$-deviation from $P$ to $P'$ such that $\Lambda'-\Lambda=(\ldots,0,1,-3,3,-1,0,\ldots)$ where $\Lambda$ and $\Lambda'$ are the vectors of partitions $P$ and $P'$, respectively.
We define the vector $\gamma[p]$ of size $n$ such that:
\begin{equation*}
\begin{cases}
\gamma_{p}[p] = 1 \\
\gamma_{p-1}[p] = -3 \\
\gamma_{p-2}[p] = 3 \\
\gamma_{p-3}[p] = -1 \\
\gamma_{j}[p] = 0 & \mbox{otherwise}
\end{cases}
\end{equation*}

Given the vector $\Lambda$ of a partition $\P$, the $3$-deviation considered here is such that $\Lambda' = \Lambda + \gamma[p]$, for some $p$, where $\Lambda'$ represents the new partition after the deviation.

Let $\P$ the partition represented by $\Lambda=(0,\ldots,0,\lambda_{L}=c,\ldots,\lambda_{1}=c)$.
The number of nodes is $O(cL^{2})$.

Let $t \leq \frac{L-1}{4}$.

We first do $t+1$ consecutive $3$-deviations $\gamma[L], \ldots, \gamma[L-t]$ from $\P$ to $\P^{1}$.
We get $\Lambda^{1} = \Lambda + \gamma^{1}[L]$ where $\Lambda^{1}$ is the vector of $\P^{1}$ and $\gamma^{1}[L] = \sum_{i=L-t}^{L} \gamma[i]$ is such that:
\begin{equation*}
\begin{cases}
\gamma^{1}_{L}[L] = 1 \\
\gamma^{1}_{L-1}[L] = -2 \\
\gamma^{1}_{L-2}[L] = 1 \\
\gamma^{1}_{L-t-1}[L] = -1 \\
\gamma^{1}_{L-t-2}[L] = 2 \\
\gamma^{1}_{L-t-3}[L] = -1 \\
\gamma^{1}_{j}[L] = 0 & \mbox{otherwise.}
\end{cases}
\end{equation*}

We repeat the sequence $\gamma^{1}$ starting from $L-1, L-2, \ldots, L-t+2$.
That corresponds to $t-1$ consecutive sequences $\gamma^{1}[L], \ldots, \gamma^{1}[L-t+2]$ from $\P$ to $\P^{2}$.
We get $\Lambda^{2} = \Lambda + \gamma^{2}[L]$ where $\Lambda^{2}$ is the vector of $\P^{2}$ and $\gamma^{2}[L] = \sum_{i=L-t+2}^{L} \gamma^{1}[i]$ is such that:
\begin{equation*}
\begin{cases}
\gamma^{2}_{L}[L] = 1 \\
\gamma^{2}_{L-1}[L] = -1 \\
\gamma^{2}_{L-t+1}[L] = -1 \\
\gamma^{2}_{L-t}[L] = 1 \\
\gamma^{2}_{L-t-1}[L] = -1 \\
\gamma^{2}_{L-t-2}[L] = 1 \\
\gamma^{2}_{L-2t}[L] = -1 \\
\gamma^{2}_{L-2t-1}[L] = 1 \\
\gamma^{2}_{j}[L] = 0 & \mbox{otherwise.}
\end{cases}
\end{equation*}

We repeat the sequence $\gamma^{2}$ starting from $L-1, L-2, \ldots, L-t+4$.
That corresponds to $t-3$ consecutive sequences $\gamma^{2}[L], \ldots, \gamma^{2}[L-t+4]$ from $\P$ to $\P^{3}$.
We get $\Lambda^{3} = \Lambda + \gamma^{3}[L]$ where $\Lambda^{3}$ is the vector of $\P^{3}$ and $\gamma^{3}[L] = \sum_{i=L-t+4}^{L} \gamma^{2}[i]$ is such that:
\begin{equation*}
\begin{cases}
\gamma^{3}_{L}[L] = 1 \\
\gamma^{3}_{L-t+3}[L] = -1 \\
\gamma^{3}_{L-t+2}[L] = -1 \\
\gamma^{3}_{L-t}[L] = -1 \\
\gamma^{3}_{L-3t+3}[L] = 1 \\
\gamma^{3}_{L-3t+1}[L] = 1 \\
\gamma^{3}_{L-4t}[L] = -1 \\
\gamma^{3}_{j}[L] = 0 & \mbox{otherwise}
\end{cases}
\end{equation*}

We finally repeat the sequence $\gamma^{3}$ from $L-1, L-2, \ldots, L-t+1$.
That corresponds to $t$ consecutive sequences $\gamma^{3}[L], \ldots, \gamma^{3}[L-t+1]$ from $\P$ to $\P^{4}$.
We get $\Lambda^{4} = \Lambda + \gamma^{4}[L]$ where $\Lambda^{4}$ is the vector of $\P^{4}$ and $\gamma^{4}[L] = \sum_{i=L-t+1}^{L} \gamma^{3}[i]$.
As $\gamma^{3}[i]$ has a constant number of non zero values, then for any $j$, $1 \leq j \leq L$, $\gamma^{4}_{j}[L] \geq -c$ where $c \geq 4$.

Set $t = \theta(L)$ such that $t \leq \frac{L-1}{4}$.
We get that the total number of $3$-deviations is $\theta(t^{4}) = \theta(L^{4})$.
Recall that the number of nodes is $O(cL^{2})=O(L^{2})$.
\end{proof}












\iffalse
\begin{lemma}
\label{lem:lower-bound-3}
$L(3,n) = \Omega(n^{2})$.
\end{lemma}

\begin{proof}
This proof is similar to the proof for $k=4$ but it is simpler since we construct only $v^{1}, v^{2}, v^{3}, v^{4}$.

We only consider here $3$-deviations that consist in creating $1$ group of size $p$, removing $3$ groups of size $p-1$, creating $3$ groups of $p-2$, and removing $1$ group of size $p-3$, for some $p$.
Let $\phi_{L-p+1}$ be the vector of difference corresponding to a $3$-deviation defined as follows.
For any $j$, $1 \leq j \leq L$:
\begin{equation*}
\phi_{j} = 
\begin{cases}
1 & \mbox{if $j = L-p+1$} \\
-3 & \mbox{if $j = L-p+2$} \\
3 & \mbox{if $j = L-p+3$} \\
-1 & \mbox{if $j = L-p+4$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}

We start from the vector of difference $v^{0}=(0,0,\ldots)$.

Set $v^{1}=\sum_{i=1}^{t}\phi_{i}$.
For any $j$, $1 \leq j \leq L$,
\begin{equation*}
v^{1}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-2 & \mbox{if $j = 2$} \\
1 & \mbox{if $j = 3$} \\
-1 & \mbox{if $j = t+1$} \\
2 & \mbox{if $j = t+2$} \\
-1 & \mbox{if $j = t+3$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}


Set $v^{2}=\sum_{i=1}^{t-2}\Phi(v^{1},i)$.
For any $j$, $1 \leq j \leq L$,
\begin{equation*}
v^{2}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-1 & \mbox{if $j = 2$} \\
-1 & \mbox{if $j = t-1$} \\
1 & \mbox{if $j = t$} \\
-1 & \mbox{if $j = t+1$} \\
1 & \mbox{if $j = t+2$} \\
1 & \mbox{if $j = 2t$} \\
-1 & \mbox{if $j = 2t+1$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}


Set $v^{3}=\sum_{i=1}^{t-3}\Phi(v^{2},i)$.
For any $j$, $1 \leq j \leq L$,
\begin{equation*}
v^{3}(j) = 
\begin{cases}
1 & \mbox{if $j = 1$} \\
-1 & \mbox{if $j = t-2$} \\
-1 & \mbox{if $j = t-1$} \\
-1 & \mbox{if $j = t+1$} \\
1 & \mbox{if $j = 3t-2$} \\
1 & \mbox{if $j = 3t$} \\
-1 & \mbox{if $j = 4t+1$} \\
0 & \mbox{otherwise}
\end{cases}
\end{equation*}

Set $v^{4}=\sum_{i=1}^{t}\Phi(v^{3},i)$.
As $v^{3}$ has a constant number of non zero values, then for any $j$, $1 \leq j \leq L$, $v^{4}(j) \geq -c$ where $c \leq 4$.

Clearly, each vector of difference from $v^{0}$ to $v^{4}$ is $c$-balanced where $c$ is constant.
Thus, we get that the total number of $3$-deviations is $\theta(t^{4})$ and the number of nodes is $\theta(t^{2})$.
\end{proof}
\fi



==> Long/SAUVEGARDE/weighted-long-SAUVEGARDE.tex <==
\section{General case: largest collusions}
\label{sec:weighted}

\def\MIS{{\sc Maximum Independent Set problem}\xspace}
\def\SD{{\sc k-Stable decision problem}\xspace}


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%

\iffalse
\begin{proof}
First note that the global utility is upper-bounded.
Let $C_{0}$ be any configuration with $q$ channels for $D$.
If $C_{0}$ is $1$-stable for $D$, we are done.

Otherwise, there exists a vertex $v \in V$ such that $\{v\}$ breaks $C_0$.
We denote $C_{1}$ the configuration with $q$ channels obtained after this $1$-deviation.
By definition $f_{v}(C_1) > f_{v}(C_0)$.
We partition $V \setminus \{v\}$ as follows:
$V_=$ is the set $\{u, |C_{1}(u) \cap C_{1}(v)| = |C_{0}(u) \cap C_{0}(v)|\}$ and $V_{\neq}$ is the set $\{u, |C_{1}(u) \cap C_{1}(v)| \neq |C_{0}(u) \cap C_{0}(v)|\}$.
Observe that $f_{v}(C_1) - f_{v}(C_0) = \sum_{u \in V_{\neq}} h(|C_{1}(u) \cap C_{1}(v)|,w(v,u)) - h(|C_{0}(u) \cap C_{0}(v)|,w(v,u)) > 0$.
We have $f(C_1) - f(C_0) \\
= f_{v}(C_1) - f_{v}(C_0) + \sum_{u \in V_{\neq}} f_{u}(C_1) - f_{u}(C_0) \\
= \sum_{u \in V_{\neq}} h(|C_{1}(u) \cap C_{1}(v)|,w) - h(|C_{0}(u) \cap C_{0}(v)|,w) \\
+  \sum_{u \in V_{\neq}} h(|C_{1}(u) \cap C_{1}(v)|,w) - h(|C_{0}(u) \cap C_{0}(v)|,w) \\ 
 = 2(\sum_{u \in V_{\neq}} h(|C_{1}(u) \cap C_{1}(v)|,w) - h(|C_{0}(u) \cap C_{0}(v)|,w)) \\
 > 0$ where $w = w(u,v)$.
Finally, as $f(C_{1})$ is upper-bounded, we get a $1$-stable configuration with $q$ channels, after a finite number of $1$-deviations.
\end{proof}
\fi

%%%%% FIN DE PREUVE COMMENTEE %%%%%


The uniform case we analyzed so far may be described as a ``clique with enemies'': A pair of nodes may either be connected by an edge with unit weight: $w_{uv}=1$, or they are in conflict: $w_{uv}=-\infty$. 

More generally, a coloring game may be defined with weights taking values in a larger set $\mathcal{W}$. 
In such, nodes choose to interact with each others according to more complex preferences.
In particular, the individual utility may not be related to the size of the sharing group anymore.
Hence we first need a tool to lower-bound the global utility in a more general situation:

\begin{lemma}
\label{lem:util-variations}
Given a graph $G=(V,w)$, let $P$ be a partition of the nodes, let $S = \{v_1, \ldots, v_k\}$ be a $k$-set that breaks $P$, and let $P'$ be the resulting partition.
Then:

\centering
$f(P') - f(P) \geq 2[ k - \sum_{1\leq i,j \leq k}w_{u_i,u_j} + \sum_{\{u_i,u_j \mid X(u_i) = X(u_j)\}}w_{u_i,u_j}]$. 
\end{lemma}


This first proves that $1$-deviations in a general weighted coloring game result in an increased total utility. Hence,

\begin{theorem}
\label{thm:stability:k=1}
For any weighted graph, if only $1$-deviations are allowed, a coloring game always converges in $O(n^2)$ steps. 
\end{theorem}

Theorem~\ref{thm:stability:k=1} proves that all these games admit a partition that is $1$-stable, or equivalently, a Nash-equilibrium. 
However, the general coloring games are much harder to characterize than the uniform case: A $k$-stable partition (with $k>1$) may not necessarily exist, and as a result, the dynamic of the game may not always converge.
It may also fail to converge even when such partitions exist.
We now analyze all games where weights are chosen in a fixed subset $\mathcal{W}$. 
We wish to identify the greatest values of $k$ for which $k$-stability can \emph{always} be attained, that we denote $k(\mathcal{W})$.

COMPLEXITE


% 
% In the sequel, we will denote by $\mathcal{W}$ a set of constant weights for our coloring games.
% % Indeed, it only requires symmetrical relations between nodes to hold.
% 
% On the other hand, we will also prove that bilateral and larger deviations may not be avoided, depending on the set of weights.
% Our goal in this section is to identify the greatest values of $k$ for which $k$-stability can be attained, primarily as a threshold function of the possible values $\mathcal{W}\subseteq \RelInt$ taken by weights.
% % However, we will also prove that $k(\mathcal{W}) \leq 3$ for most sets of weights.
% We characterize all the cases where $k(\mathcal{W})$ is infinite, including previous results~\cite{Kleinberg:2010ul}. 
% We also provide an upper bound for all other cases, which is most generally tight.

% An upper-bound is given in all the cases, and the few sets of weights for which $k(\mathcal{W})$ is not upper-bounded are identified, giving a nice generalization of the result in~.
% Tight bounds are also presented for any extension of the model of clique with enemies and indifference (e.g. $\mathcal{W}=\{-M,0,1\}$).
% To this end, we start by proving a sufficient structural condition for the existence of $k$-stable configuration, for any $k \geq 1$.

% The study of the threshold function has its own interest from a theoretical point of view.
% We complete it with a computational consequence: if one graph in a class does not admit $k$-stable configuration, then it is not only uncertain but it is also NP-hard to decide if such configuration exists in general for the whole class.

% deciding whether there exists a $k$-stable configuration is NP-hard, even if $\mathcal{W}=\{-M,0,1\}$ and $k=3$.

%\subsection{Games with weights $\mathcal{W}=\{-M,0,1\}$}
\subsection{Games with non positive and unit weights}
\label{subsec:-m01}

We first focus on the subsets of $\{-\infty,0,1\} \cup -\mathbb{N}$, the best representative of which is $\mathcal{W} = \{-\infty,0,1\}$, of theoretical importance.
Whereas it does not differ that much from the set $\{-\infty,1\}$, its stability properties are far more constrained. 
If we refer ourselves to the dynamic system, then there may not exist stable partitions whenever the global utility does not increase at each step.  
We prove that in this case $k(\mathcal{W}) = 2$.

Let us first show that $k(\mathcal{W}) \geq 2$.
In fact, Theorem~\ref{thm:stability:ktree} is a global stability result, which is more precise and uses structural properties of the graphs.
Given a network $G=(V,w)$, let us define the "friendship graph" $G^{+} = (V,E^{+})$ of  $G$, where $E^{+} = \{ uv \in E: w(u,v) > 0\}$.
We remind that the \emph{girth} of a graph is the length of its shortest cycle.
By definition, an acyclic graph has infinite girth.


\begin{theorem}
\label{thm:stability:ktree}
Given an integer $k \geq 1$ and a graph $G = (V,w)$ with $\mathcal{W} \subseteq \{-\infty,0,1\} \cup -\mathbb{N}$, there exists a $k$-stable partition for $G$ if the girth of the friendship graph $G^{+}$ is at least $k+1$.
Furthermore, the dynamic always reaches a $k$-stable partition in $O(n^2)$ steps in that case.
\end{theorem}




%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $C_0$ be any configuration for $D$, such that there is no vertices $u$ and $v$ with $w(u,v) = -M$ and $C_0(u) = C_0(v)$.
If $C_0$ is $k$-stable, we are done.
Otherwise there exists a subset $S = \{v_1,v_2, \ldots, v_{|S|}\}$, $|S| \leq k$, such that $S$ breaks $C_0$.
As in the case $k=1$, we will prove the global utility strictly increases after any $k$-deviation.
Let $C_1$ be the new configuration for $D$ that we get after the $k$-deviation.
Actually, we already have that, for any $1 \leq i \leq |S|$, $f_{v_i}(C_1) \geq f_{v_i}(C_0) +1$.
However, we have to be careful with summations, as we may have $v_i$ that benefits from the presence of $v_j$, for some $1 \leq j \leq |S|$, $j \neq i$.
Such improvement of the individual utility of both $v_i$ and $v_j$ cannot be counted twice for the global utility.
Thus, by symmetry, we get $f(C_1) - f(C_0) \geq 
2|S|  - 2\sum_{1 \leq i < j \leq |S|} w(v_i,v_j)$.

Moreover, we claim that for every $1 \leq i < j \leq |S|$, $w(v_i,v_j) \neq -M$, because $M$ is taken large enough so that such an interaction is avoided at any cost, if it does not already exist.
Consequently, either $w(v_i,v_j) = 0$, or $w(v_i,v_j) = 1$.
Hence, by definition of $G^{+}$, $f(C_{1}) - f(C_{0}) \geq 2(|S|-|E_{S}|)$ where $E_{S}$ is the set of edges induced by nodes of $S$ in the friendship graph $G^{+}$.
Furthermore, $G^{+}$ has girth at least $k+1$, that is the induced graph $G_S = (S,E_S)$ is a forest, because $|S| \leq k$, and so $|E_{S}| < |S|$.
Finally, since the global utility is upper-bounded, we get a $k$-stable configuration for $D$ after a finite number of $k$-deviations.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%

Particularly, if $G^{+}$ is cycle-free, then we get there is a $k$-stable partition for $G$, for any $k \geq 1$;
if $G^{+}$ is triangle-free, then there always exists a $3$-stable partition for $G$.
Furthermore, as the girth of any graph is at least $3$, then there always exists a $2$-stable partition.
 
Theorem~\ref{thm:stability:ktree} also shows that such a coloring game takes at most $O(n^2)$ steps to converge. 
Using another sequence construction, one can prove that this bound is indeed tight in the general case.

% By Theorem~\ref{thm:stability:ktree}, for any graph, any sequence of $2$-deviations has size $O(n^{2})$ because the global utility always increases.
% We prove the tightness of this bound using graphs with set of weights $\{0,1\}$.

\begin{lemma}
\label{lem:n-square}
There exists $G=(V,w)$ with $\mathcal{W} = \{0,1\}$ such that there is a sequence of $\theta(n^2)$ $1$-deviations for $G$.
\end{lemma}


Finally, we show that there exists a graph $G$ such that any partition for $G$ is not $3$-stable ($k(\{-\infty,0,1\}) \leq 2$).
The proof is all the more counter-intuitive as it implies there are infinite sequences of deviations that do not change the global utility, even in graphs with only four edges weighted by $0$!


\begin{figure}[t]
\centerline{\includegraphics[width=0.5\linewidth]{Figures/Unstablek4noborder.pdf}
\includegraphics[width=0.5\linewidth]{Figures/Unstablek3ActPass.pdf}}
\caption{Graph that does not admit a k-stable partition with k=4 (left) and k=3 (right).}
\vspace{-0.25cm}
\label{fig:counter-examples}
\end{figure}


We first define the notion of twin vertices and we prove a useful lemma.

\begin{definition}
Let $G=(V,w)$ be a graph, and $u,u' \in V$ be two users.
We say that $u$ and $u'$ are \emph{twins} if and only if $w_{u,u'} > 0$ and for all vertex $v \in V \setminus \{u,u'\}$ $w_{u,v} = w_{u',v}$. 
\end{definition}

\begin{lemma}
\label{lemma:group}
Given a graph $G$, and a $1$-stable partition $P$ for $G$,
for all vertices $u,u'$ such that $u$ and $u'$ are twins, we have that $X(u) = X(u')$. 
\end{lemma}

\begin{proof}
By contradiction.
Suppose $X(u) \neq X(u')$.
By symmetry, we can assume $f_u(P) \leq f_{u'}(P)$.
Thus, $\{u\}$ breaks the partition, as vertex $u$ joins the group of $u'$ because, in this new partition $P'$ for the nodes, we get $f_u(P') = f_{u'}(P) + w_{u,u'} > f_u(P)$.
A contradiction.
Hence $X(u) = X(u')$.
\end{proof}





\begin{lemma}
\label{lem:counter-example}
There exists $G=(V,w)$ with $\mathcal{W} = \{-\infty,0,1\}$ such that there is no $3$-stable partition of the nodes for $G$.
\end{lemma}

\begin{proof}
The set of vertices consists of four sets $A_i$, $0 \leq i \leq 3$, each of equal size $h \geq 2$ and with a special vertex $a_i$, plus four vertices $b_i$, $0 \leq i \leq 3$, and two vertices $c_0$ and $c_1$.
In what follows, indices are taken modulo $2$ for $c_j$, $j \in \{0,1\}$, and they are taken modulo $4$ everywhere else.
Figure~\ref{fig:counter-examples} (right) represents the example with $h=4$. 

The friendship graph $G^+$ here consists of all the edges with weight $1$; the set $E^+$ contains:
\begin{enumerate}
\item all the edges between nodes in $A_i$ ($0\leq i \leq 3$);
\item edges from $b_i$ to $A_i$ ($0\leq i \leq 3$);
\item edges from $b_i$ to $A_{i+1} \setminus \{a_{i+1}\}$ ($0\leq i \leq 3$);
\item edges from $b_i$ to $b_{i-1}$ and $b_{i+1}$ ($0\leq i \leq 3$);
\item edges from $c_0$ to all the $b_i$, and edges from $c_1$ to all the $b_i$;
\item edges from $c_0$ to $A_0 \cup A_2$, and edges from $c_1$ to $A_1 \cup A_3$.
\end{enumerate} 
Moreover, there are four edges with weight $0$, namely the edges $b_i a_{i+1}$.
All the remaining edges have weight $-\infty$. 
That is two nodes in different $A_i,A_{i'}$ are enemies; a user $b_i$ is enemy of $b_{i+2}$ and of the nodes in $A_{i+2}$ and $A_{i+3}$; $c_0$ and $c_1$ are enemies; $c_0$ is enemy of the nodes in $A_1$ and $A_3$, and $c_1$ is enemy of the nodes in $A_0$ and $A_2$. 

We now assume there exists a $3$-stable partition $P$ for $G$.

\begin{claim}
\label{claim:subgrp}
Every $A_i$ is a subgroup in $P$.
\end{claim}


\begin{claim}
\label{claim:contre-2}
$b_i$ is in the same group as $A_i$ or $A_{i+1}$.
\end{claim}


\begin{claim}
\label{claim:contre-3}
There exists an $i$ such that $A_i, b_i$ and $b_{i-1}$ are in the same group. 
\end{claim}


\begin{claim}
\label{claim:contre-4}
There exists an $i$, such that $b_{i}$, $b_{i-1}$ and $c_{i}$ are in the same group as $A_{i}$ in $P$.
Moreover, such a group is unique in $P$, due to the conflict graph in $G$. 
\end{claim}

The proof of Claim~\ref{claim:contre-4} is straightforward using the previous claim.
By symmetry, we assume that $P$ contains the group $\{b_0,b_3,c_0\} \cup A_0$.

Case $1$: the group containing $A_2$ also contains $b_1$ and $b_2$.
Then either $c_1$ is with $A_1$ and a $1$-deviation of $b_1$ to $A_1 \cup \{c_1\}$ breaks $P$, or $c_1$ is not with $A_1$ and a $2$-deviation of $\{b_1,c_1\}$ to $A_1$ breaks $P$.

Case $2$: the group containing $A_2$ only contains $b_2$.
Then either $c_1$ is with $A_3$ and a $2$-deviation of $\{b_2,b_3\}$ to $A_3$ breaks $P$, or $c_1$ is not with $A_3$ and a $3$-deviation of $\{b_2,b_3, c_1\}$ to $A_3$ breaks $P$.

Case $3$: the group containing $A_2$ only contains $b_1$.
In that case, a $1$-deviation from $b_1$ to the group containing $A_1$ breaks $P$.

Case $4$: $A_2$ is a group in $P$.
This implies $b_2$ is with $A_3$.
Then either $c_1$ is with $A_3$ and a $1$-deviation of $b_3$ to $A_3$ breaks $P$, or $c_1$ is not with $A_3$ and a $2$-deviation of $\{b_3, c_1\}$ to $A_3$ breaks $P$.


Finally, there does not exist a $3$-stable partition $P$ for $G$.
\end{proof}

\iffalse
\begin{proof}
We define the graph $G=(V,E,w)$ as follows.
The set of vertices $V$ is partitioned into five subsets: $A_0, A_1, A_2, A_3$ and $\{b_0, b_1, b_2, b_3, c_0, c_1 \}$.
Let $i,i',j,j'$ be four integers (not necessarily distinct), such that $0 \leq i,i',j,j' \leq 3$.
\begin{itemize}
\item First we have that $|A_i| = 4$, and we denote the vertices in $A_i$ by $a_{i,0}, a_{i,1}, a_{i,2} \text{ and } a_{i,3}$.
\item Furthermore, we set $w(a_{i,j},a_{i',j'}) = 1$ if $i=i'$, and $w(a_{i,j},a_{i',j'}) = -M$ otherwise.
\item We also set $w(b_i,a_{i',j}) = 1$ if $i=i'$, or $i' \equiv i + 1$ (mod $4$) and $j \neq i$; $w(b_i,a_{i',j}) = 0$ if $i' \equiv i + 1$ (mod $4$) and $j = i$;  $w(b_i,a_{i',j}) = -M$ otherwise.
\item Moreover, $w(b_i,b_i') = 1$ if $i' \equiv i \pm 1$ (mod $4$); $w(b_i,b_i') = -M$ if $i' \equiv i + 2$ (mod $4$).
\item Finally, for every $0 \leq p \leq 1$, $w(b_i,c_p) = 1$, $w(c_p,a_{i,j}) = 1$ if $i \equiv p$ (mod $2$), and $w(c_p,a_{i,j}) = -M$ otherwise.
\item We also set $w(c_0,c_1) = -M$.
\end{itemize}
Observe that there are only four edges in $G$ whose weight equals $0$.
Figure~\ref{fig:counter-examples} (right) represents the graph $G$.\\

\noindent
We now assume there exists a $3$-stable configuration $C_3$ for $G$.

We first claim that every subset $A_i$ is a subgroup in $C_3$, that is all the vertices in $A_i$ are in the same group in $C_3$.
Indeed, $A_i \setminus \{a_{i,i}\}$ is a subgroup in $C_3$ by Lemma~\ref{lemma:group}.
Then, by contradiction, suppose $a_{i,i}$ is not in the same group as $A_i \setminus \{a_{i,i}\}$.
Observe that all the vertices in $A_i$ share the same enemies.
Moreover, the only friends of $a_{i,i}$ that are not in $A_i$ are $b_i$ and $c_{i \text{ (mod }2)}$.
Thus $f_{a_{i,i}}(C_3) \leq 2$, so, $\{a_{i,i}\}$ breaks $C_3$, and the claim is proved.
At the end, there are, at least, four groups in $C_3$ (one different group for each subset $A_{i}$).\\

\noindent
We now claim that either $b_i$ is in the same group as $A_i$ in $C_3$, or $b_i$ is in the same group as $A_{i'}$ in $C_3$, with $i' \equiv i+1$ (mod $4$).
By contradiction.
One can check that, if $b_i$ is neither in the same group as $A_i$ nor in the same group as $A_{i'}$, we have $f_{b_i}(C_3) \leq 2$, due to the conflict graph in $G$.
On the opposite, if either $b_i$ is in the same group as $A_i$ in $C_3$, or $b_i$ is in the same group as $A_{i'}$ in $C_3$, we get $f_{b_i}(C_3) \geq 3$, and there is no enemy of $b_i$ that is not enemy with the vertices in $A_i$ or that is not enemy with the vertices in $A_{i'}$.
Again, there is a contradiction, as in this case, $C_3$ would not be $1$-stable.

Especially, we claim that there is an $i$, $0 \leq i \leq 3$, such that $b_i$ and $b_{i''}$ are in the same group as $A_i$ in $C_3$, with $i \equiv i'' + 1$ (mod $4$).
To prove this claim, we first recall that $w(b_i,b_{i''}) = 1$.
Then, again, we prove this claim by contradiction.
Suppose that, for every $0 \leq i \leq 3$, there is only one vertex $b_j$ such that $b_j$ and $A_i$ are in the same group.
By the hypothesis, either $j = i$, or $j=i''$.
Furthermore, either $j = i$ for all $i$, or $j = i''$ for all $i$.
We also have that either $c_0$ is in the same group as $A_0$, or $c_0$ is in the same group as $A_2$.
In the same way, we have that either $c_1$ is in the same group as $A_1$, or $c_1$ is in the same group as $A_3$.
Moreover, for every $0 \leq i \leq 3$, $w(c_0,b_i) = w(c_1,b_i) = 1$.
Thus, if $j=i''$ for all $i$, then any subset $\{b_{i''},c_{i'' \text{ (mod }2\text{)}}\}$ breaks the configuration $C_3$, by joining the same group as $A_{i''}$, and so, $j = i$ for all $i$, because $C_3$ is $3$-stable.
We have $f_{b_i}(C_3) = 4$ if $c_{i \text{ (mod }2\text{)}}$ is not in the same group as $b_i$ and $A_{i}$, and  $f_{b_{i}}(C_3) = 5$ otherwise. 
However, remark that there are always two vertices $b_i$ such that  $f_{b_i}(C_3) = 4$, because there are only two vertices $c_{0}, c_{1}$.
Furthermore, if $f_{b_{i}}(C_3) = 4$, then the subset $\{b_{i},c_{i' \text{ (mod }2\text{)}}\}$ breaks the configuration $C_3$, by joining the same group as $A_{i'}$, with $i' \equiv i+1$ (mod $4$).
Hence $C_3$ cannot be $2$-stable, which is a contradiction, and our third claim is proved.

As an immediate consequence, we get that there exists an $i$, $0 \leq i \leq 3$, such that $b_{i}$, $b_{i''}$ and $c_{i \text{ (mod }2\text{)}}$ are in the same group as $A_{i}$ in $C$, with $i \equiv i'' + 1$ (mod $4$).
Such a group is unique in $C_3$, due to the conflict graph in $G$.
By symmetry, suppose that $i = 0$.\\
There are four cases.
\begin{enumerate}
\item If $b_{1}$ and $b_{2}$ are in the same group as $A_{2}$ in $C_3$, then $\{b_{1},c_{1}\}$ breaks the configuration $C_3$, by joining the same group as $A_{1}$.
\item If $b_{2}$ is in the same group as $A_{3}$, and $b_{1}$ and $c_{1}$ are in the same group as $A_{1}$, then $\{b_{2}\}$ breaks the configuration $C_3$, by joining the same group as $A_{2}$.
\item If $b_{2}$ and $c_{1}$ are in the same group as $A_{3}$, then $\{b_{3}\}$ breaks the configuration $C_3$, by joining the same group as $A_{3}$.
\item If $b_{2}$ is in the same group as $A_{2}$, and $b_{1}$ and $c_{1}$ are in the same group as $A_{1}$, then $\{b_{2},b_{3},c_{1}\}$ breaks the configuration $C_3$, by joining the same group as $A_3$. 
\end{enumerate}
Finally, there does not exist a $3$-stable configuration $C_3$ for $G$.
\end{proof}
\fi


Figure~\ref{fig:counter-examples} presents two graphs that are not stable for $k=4$ and $k=3$, respectively.
To keep graphs readable, we use conventions. 
(1) Some cliques of nodes are grouped within a circle (\eg C3 is a clique of 3 nodes); an edge from another node to that circle denotes an edge to \emph{all} elements of this clique.
(2) On the right, we omitted the edges with weights $-\infty$ denoting pairs of enemies. 
These are all the edges between nodes on different sides of a dashed line, unless it was otherwise indicated as a green edge (weight 1) or a white edge (weight 0). We deduce then:


\begin{corollary}
\label{lem:counter-example-2}
Let $\mathcal{W} = \{-\infty,0,1\}$.
Then $k(\mathcal{W}) = 2$.
\end{corollary}





%We show in Lemma~\ref{lem:counter-example} that $k(\mathcal{W}) \leq 2$, and so by Corollary~\ref{cor:stability:k=2}, we get $k(\mathcal{W}) = 2$.








%\begin{corollary}
%\label{cor:stability:k=2}
%Let $\mathcal{W} = \{-M,0,1\}$.
%Any graph admits a $2$-stable configuration.
%\end{corollary}


% Hence, there always exists a configuration that is stable under bilateral deviations with $\mathcal{W}=\{-M,0,1\}$.



%As it was announced, we get $k(\mathcal{W}) \geq 2$.
%Before proving the tightness of this bound, we show in %Lemma~\ref{lem:longest-sequence-M-0-1} that the longest sequence is quadratic in $n$ for $k = \{1,2\}$.


%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lem:longest-sequence-M-0-1}
Let $\mathcal{W} = \{-M,0,1\}$.
$L_{\mathcal{W}}(1,n) = L_{\mathcal{W}}(2,n)= \Theta(n^{2})$.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let any $p \geq 1$.
Let $G=(V,E)$ be the graph constructed as follows.
Without loss of generality assume $n=3p$.
Let $V=V^{1} \cup V^{2} \cup V^{3}$ with $|V^{1}|=|V^{2}|=|V^{3}|=p$.
For any $u, v \in V^{2} \cup V^{3}$, $w(u,v) = 1$.
For any $u, v \in V^{1}$, $w(u,v) = 0$.
For any $u \in V^{1}$, for any $v \in V^{2}$, $w(u,v) = 1$.

We set $V^{1}=\{u_{1}, u_{2}, \ldots, u_{p}\}$ and $V^{2}=\{v_{1}, v_{2}, \ldots, v_{p}\}$.

Consider the partition $C$ such that any node of $V^{1} \cup V^{2}$ forms a singleton group and there is group formed by all the nodes of $V^{3}$.

Sequentially, each node of $V^{1}$ reaches the group of $v_{1}$.
The utility of $v_{1}$ is now $p$.
Then $v_{1}$ reaches the group composed of all nodes of $V^{3}$.
The utility of $v_{1}$ is now $p+1$, and the utility of each $u_{i}$ is $0$.
The number of $1$-deviations is $p+1$.
We repeat the same process for $v_{2}$ using $p+1$ deviations.
And so on for each $v_{i}$, $3 \leq i \leq p$.

Finally, the number of $1$-deviations is $(p+1)p$.
Thus $L_{\{-M,0,1\}}(1,n) = \theta(n^{2})$ because the global utility, upper-bounded by $n(n-1)$, strictly increases after each $1$-deviation.

Obviously, we get $L_{\{-M,0,1\}}(2,n) = \theta(n^{2})$
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%



\iffalse
Moreover, the result still holds if we add to the set 
$\mathcal{W}=\{-M,0,1\}$ 
some negative integer weights $w(u,v)$, with $-M < w(u,v) < 0$.
Thus, we get a more sufficient condition on $\mathcal{W}$ so that $k(\mathcal{W}) \geq 2$.
\fi

\iffalse
It can be generalized to the multi-channel model as well.
But we then need an extra-property for the function $h$. 
We have to constrain ourselves to a model that takes account of the enmity between two nodes only once.
In other words: for any number of groups $g$, and for any negative weight $w$, $h(g+1,w) = h(g+2,w)$.
However, sharing information with a friend in several groups may be beneficial.\\
\fi





%, \ie there exists a graph with such weights that does not admit 3-stable configuration.

%We first need to define the useful notion of twins.
%We can now prove the following graph is a counter-example:







%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lem:counter-example}
Let $\mathcal{W}=\{-M,0,1\}$.
There exists a graph $G$ such that any configuration for $G$ is not $3$-stable.
\end{lemma}
\fi
%%%%% DEBUT DE LEMME COMMENTE %%%%%


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
We define the graph $D=(V,A,w)$ as follows.
The set of vertices $V$ is partitioned into five subsets: $A_0, A_1, A_2, A_3$ and $\{b_0, b_1, b_2, b_3, c_0, c_1 \}$.
Let $i,i',j,j'$ be four integers (not necessarily distinct), such that $0 \leq i,i',j,j' \leq 3$.
\begin{itemize}
\item First we have that $|A_i| = 4$, and we denote the vertices in $A_i$ by $a_{i,0}, a_{i,1}, a_{i,2} \text{ and } a_{i,3}$.
\item Furthermore, we set $w(a_{i,j},a_{i',j'}) = 1$ if $i=i'$, and $w(a_{i,j},a_{i',j'}) = -M$ otherwise.
\item We also set $w(b_i,a_{i',j}) = 1$ if $i=i'$, or $i' \equiv i + 1$ (mod $4$) and $j \neq i$; $w(b_i,a_{i',j}) = 0$ if $i' \equiv i + 1$ (mod $4$) and $j = i$;  $w(b_i,a_{i',j}) = -M$ otherwise.
\item Moreover, $w(b_i,b_i') = 1$ if $i' \equiv i \pm 1$ (mod $4$); $w(b_i,b_i') = -M$ if $i' \equiv i + 2$ (mod $4$).
\item Finally, for every $0 \leq p \leq 1$, $w(b_i,c_p) = 1$, $w(c_p,a_{i,j}) = 1$ if $i \equiv p$ (mod $2$), and $w(c_p,a_{i,j}) = -M$ otherwise.
\item We also set $w(c_0,c_1) = -M$.
\end{itemize}
Observe that there are only four edges in $D$ whose weight equals $0$.
Figure~\ref{fig:counter-examples} (right) represents the graph $D$.\\

\noindent
We now assume there exists a $3$-stable configuration with single channel $C_3$ for $D$.

We first claim that every subset $A_i$ is a subgroup in $C_3$, that is all the vertices in $A_i$ are in the same group in $C_3$.
Indeed, $A_i \setminus \{a_{i,i}\}$ is a subgroup in $C_3$ by Lemma~\ref{lemma:group}.
Then, by contradiction, suppose $a_{i,i}$ is not in the same group as $A_i \setminus \{a_{i,i}\}$.
Observe that all the vertices in $A_i$ share the same enemies.
Moreover, the only friends of $a_{i,i}$ that are not in $A_i$ are $b_i$ and $c_{i \text{ (mod }2)}$.
Thus $f_{a_{i,i}}(C_3) \leq 2$, so, $\{a_{i,i}\}$ breaks $C_3$, and the claim is proved.
At the end, there are, at least, four groups in $C_3$ (one different group for each subset $A_{i}$).\\

\noindent
We now claim that either $b_i$ is in the same group as $A_i$ in $C_3$, or $b_i$ is in the same group as $A_{i'}$ in $C_3$, with $i' \equiv i+1$ (mod $4$).
By contradiction.
One can check that, if $b_i$ is neither in the same group as $A_i$ nor in the same group as $A_{i'}$, we have $f_{b_i}(C_3) \leq 2$, due to the conflict graph in $D$.
On the opposite, if either $b_i$ is in the same group as $A_i$ in $C_3$, or $b_i$ is in the same group as $A_{i'}$ in $C_3$, we get $f_{b_i}(C_3) \geq 3$, and there is no enemy of $b_i$ that is not enemy with the vertices in $A_i$ or that is not enemy with the vertices in $A_{i'}$.
Again, there is a contradiction, as in this case, $C_3$ would not be $1$-stable.

Especially, we claim that there is an $i$, $0 \leq i \leq 3$, such that $b_i$ and $b_{i''}$ are in the same group as $A_i$ in $C_3$, with $i \equiv i'' + 1$ (mod $4$).
To prove this claim, we first recall that $w(b_i,b_{i''}) = 1$.
Then, again, we prove this claim by contradiction.
Suppose that, for every $0 \leq i \leq 3$, there is only one vertex $b_j$ such that $b_j$ and $A_i$ are in the same group.
By the hypothesis, either $j = i$, or $j=i''$.
Furthermore, either $j = i$ for all $i$, or $j = i''$ for all $i$.
We also have that either $c_0$ is in the same group as $A_0$, or $c_0$ is in the same group as $A_2$.
In the same way, we have that either $c_1$ is in the same group as $A_1$, or $c_1$ is in the same group as $A_3$.
Moreover, for every $0 \leq i \leq 3$, $w(c_0,b_i) = w(c_1,b_i) = 1$.
Thus, if $j=i''$ for all $i$, then any subset $\{b_{i''},c_{i'' \text{ (mod }2\text{)}}\}$ breaks the configuration with single channel $C_3$, by joining the same group as $A_{i''}$, and so, $j = i$ for all $i$, because $C_3$ is $3$-stable.
We have $f_{b_i}(C_3) = 4$ if $c_{i \text{ (mod }2\text{)}}$ is not in the same group as $b_i$ and $A_{i}$, and  $f_{b_{i}}(C_3) = 5$ otherwise. 
However, remark that there are always two vertices $b_i$ such that  $f_{b_i}(C_3) = 4$, because there are only two vertices $c_{0}, c_{1}$.
Furthermore, if $f_{b_{i}}(C_3) = 4$, then the subset $\{b_{i},c_{i' \text{ (mod }2\text{)}}\}$ breaks the configuration with single channel $C_3$, by joining the same group as $A_{i'}$, with $i' \equiv i+1$ (mod $4$).
Hence $C_3$ cannot be $2$-stable, which is a contradiction, and our third claim is proved.

As an immediate consequence, we get that there exists an $i$, $0 \leq i \leq 3$, such that $b_{i}$, $b_{i''}$ and $c_{i \text{ (mod }2\text{)}}$ are in the same group as $A_{i}$ in $C$, with $i \equiv i'' + 1$ (mod $4$).
Such a group is unique in $C_3$, due to the conflict graph in $D$.
By symmetry, suppose that $i = 0$.\\
There are four cases.
\begin{enumerate}
\item If $b_{1}$ and $b_{2}$ are in the same group as $A_{2}$ in $C_3$, then $\{b_{1},c_{1}\}$ breaks the configuration with single channel $C_3$, by joining the same group as $A_{1}$.
\item If $b_{2}$ is in the same group as $A_{3}$, and $b_{1}$ and $c_{1}$ are in the same group as $A_{1}$, then $\{b_{2}\}$ breaks the configuration with single channel $C_3$, by joining the same group as $A_{2}$.
\item If $b_{2}$ and $c_{1}$ are in the same group as $A_{3}$, then $\{b_{3}\}$ breaks the configuration with single channel $C_3$, by joining the same group as $A_{3}$.
\item If $b_{2}$ is in the same group as $A_{2}$, and $b_{1}$ and $c_{1}$ are in the same group as $A_{1}$, then $\{b_{2},b_{3},c_{1}\}$ breaks the configuration with single channel $C_3$, by joining the same group as $A_3$. 
\end{enumerate}
Finally, there does not exist a $3$-stable configuration with single channel $C_3$ for $D$.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%

















\subsection{Game with general weights}

%The combination of all the lemmas in this part show that, if $\{-M,b\} \subset \mathcal{W}$ for some integer $b > 0$, then we have $k(\mathcal{W}) \leq 2$.

%We consider here sets of weights $-M \in \mathcal{W}$

While the two results we obtained ($k\geq 1$ in general, $k=2$ when the set of weights contains $-\infty$,$0$ and $1$) seem constrained, we now prove that these are the best results that one can hope for. 

In particular, we show in this section the negative influence of some pattern for stability.
This pattern is presented in Figure~\ref{fig:fig-triangle}.
We claim there does not exist any $2$-stable partition for the graph it represents.
Indeed, we have in this case that no partition $P$ is $2$ stable unless it contains either $\{u_1,v_2,v_3\}$, $\{v_1,u_2,v_3\}$, or $\{v_1,v_2,u_3\}$. 
Without loss of generality, suppose $\{u_1,v_2,v_3\} \in P$. 
Among remaining nodes, $u_2$ and $u_3$ are enemies and hence in different groups; $v_1$ will then join $u_2$. 
Consequently, there is a $2$-deviation for $P$, namely: nodes $v_1$ and $v_2$ leave their respective groups, and join the group already containing $u_3$ to form a positive triangle.

We will show with the following lemmas many variations exist for this pattern.
First, observe the weights $2,3,4$ in the counter-example of Figure \ref{fig:fig-triangle}. can be replaced by any weights $w_1,w_2,w_3$ such that $w_1 < w_2 < w_3$, and $w_1+w_2 > w_3$. 
Especially, they can be replaced by $b,b+1,b+2$, for any $b \geq 2$.  

We now show through a counter-example, no $2$-stable partition exists in general when $\mathcal{W}$ contains two positive elements, even when the zero is not present.

\begin{figure}[t]
\centerline{\includegraphics[width=0.5\textwidth]{Figures/CtrEx2PosWeight}}
\vspace{-0.2cm}
\caption{A counter-example for $2$-stability with two positive weights and conflict edges.}
\vspace{-0.45cm}
\label{fig:fig-trianglepos}
\end{figure}

\begin{lemma}
\label{lemma:extent}
Let $a,b$ be two positive integers such that $a < b$.
There is a graph $G=(V,w)$ with $\mathcal{W} = \{-\infty,a,b\}$ such that there is no $2$-stable partition for $G$.
\end{lemma}

\iffalse
\begin{proof}
Users are partitioned into four sets $V_1 = \{x_1,x_2,x_3\}$, $V_2 = \{y_1,y_2,y_3\}$, $V_3=\{z_1,z_2,z_3\}$ and $\{u_1,u_2,u_3\}$.
Each of these sets is a clique with weight $b$.
Moreover, all the edges that lie between $V_1$ and $V_2$, $V_2$ and $V_3$, and $V_3$ and $V_1$ have weight $-\infty$.
We also set that for all vertices $x_i \in V_1$, for all vertices $y_j \in V_2$, and for all vertices $z_l \in V_3$, $w_{x_i,u_1} = w_{y_j,u_2} = w_{z_l,u_3} = b$, whereas $w_{x_i,u_3} = w_{y_j,u_1} = w_{z_l,u_2} = -\infty$.
Finally:
\begin{itemize}
\item $w_{u_1,z_1} = w_{u_1,z_2} = b$; $w_{u_1,z_3} = a$;
\item $w_{u_2,x_1} = w_{u_2,x_2} = b$; $w_{u_2,x_3} = a$;
\item $w_{u_3,y_1} = w_{u_3,y_2} = b$; $w_{u_3,y_3} = a$.
\end{itemize}
 
We now assume there exists a $2$-stable partition $P$ for $G$.

\begin{claim}
$V_1, V_2$ and $V_3$ are subgroups in $P$.
\end{claim}

\begin{proofclaim}
By symmetry, it suffices to show the claim for $V_1$.
First, we have that $\{x_1,x_2\}$ is a subgroup in $P$ by Lemma~\ref{lemma:group}.
Remark that all the vertices in $V_1$ have the same enemies in the graph.
Moreover, the sum of the positive weights that lie between $x_3$ and $V \setminus V_1$ equals $b+a$, which is lower than $2b$.
Hence $V_1$ is a subgroup of $P$ because we suppose $P$ to be $1$-stable.
\end{proofclaim}

\iffalse
\begin{claim}
For every $0 \leq i \leq 2$, either $V_i \subset X(u_i)$ or $V_{i-1} \subset X(u_i)$.
\end{claim}
Again by symmetry, we only need to show it for $u_0$.
Note the enemies of $u_0$ are contained within the enemies of $V_0$ (resp. of $V_2$).
Then, the claim says that either $V_0 \subset X(u_0)$, hence $f_{u_0}(P) \geq 3b$, or $V_1 \subset X(u_0)$, hence $f_{u_0}(P) \geq 2b + a$.
Since $w_{u_0,u_1} + w_{u_0,u_2} = 2b < 2b + a$, we can conclude it is true because $P$ is $1$-stable.
\begin{claim}
There exists $i$ such that $V_i \cup \{u_i,u_{i+1}\}$ is a group in $P$.
\end{claim}
By symmetry, we can suppose  $A \cup \{u_1,u_2\}$ is a group in $C_2$.
Then, we have $\{u_2,u_3\}$ that breaks $C_2$, and so $C_2$ cannot be $2$-stable.
A contradiction.
\fi

Then, we can replace subsets $V_1,V_2,V_3$ with three nodes $v_1,v_2,v_3$ in the obvious way.
In so doing, we get the variation of Figure \ref{fig:fig-triangle} with weights $w_1 = b$, $w_2 = 2b+a$ and $w_3 = 3b$.
Moreover, it is important in the counter-example of Figure \ref{fig:fig-triangle} one can always find a $2$-deviation using nodes $u_1,u_2$ and $u_3$ only.
As a consequence, such a $2$-deviation is valid for $G$ and so, there does not exist any $2$-stable partition for $G$. 
\end{proof}
\fi

% Although the stability properties of $\{-M,0,1\}$ are constrained, we now show this is the best result one can hope in the general case.
% This is straightforward when we only add to the set $\mathcal{W}=\{-M,0,1\}$ some negative integer weights $w$ with $-M < w < 0$.
% Indeed, in that case, Theorem~\ref{thm:stability:ktree} still holds and so, $k(\mathcal{W}) = 2$ for such sets.
% 
% Other counter-examples exist for $k=2$, whenever there is at least two positive integers.
% It is interesting to denote those counter-examples use the same pattern as the two graphs in Figure~\ref{fig:counter-examples}.
% Using informal transformations and arithmetic, we can then extend those pathological cases to the case where there is only one negative integer $-a$ and a positive integer $b$, without any $0$.
% It follows that $k(\mathcal{W})$ is upper-bounded by a function of $a$ and $b$, for all these remaining cases.
%Consequently:

% \vspace{-0.2cm}
% \begin{lemma}
% For any $\mathcal{W} \supset \{-M,b\}$ for some integer $b > 0$, then $k(\mathcal{W}) < \infty$.
% \end{lemma}
% \vspace{-0.2cm}
% 

The construction is illustrated with Figure~\ref{fig:fig-trianglepos}.
Conflict edges are not drawn.
The thinnest edges represent edges with weights $a$.
The other ones represent edges with weight $b$.

Other results can be expressed in a convenient way using the subset of non-negative weights $\mathcal{W}^+$ and the subset of non-positive weights $\mathcal{W}^-$.
These two subsets entirely cover the set of weights $\mathcal{W}$, but they may not be disjoint whenever $0 \in \mathcal{W}$.

\begin{corollary}
\label{cor:mn}
Suppose $\{-\infty,N\}$ is a strict subset of $\mathcal{W}$.
Then, $k(\mathcal{W}) = 1$ if $\mathcal{W}^+ \setminus \{N\} \neq \emptyset$, and $k(\mathcal{W}) \leq 2$ otherwise.
%Let $\mathcal{W}$ be a set of weights, such that \\$\{-M,N\} \subset \mathcal{W}$.\footnote{A weight $N$ denotes a best friend if it is far larger (in absolute value) than any weight in $\mathcal{W} \setminus \{-M\}$.}
%There exists a graph $G=(V,E,w)$ such that any configuration for $G$ is not $3$-stable. 
\end{corollary}



\begin{lemma}
\label{lem:counter-example-3}
Let $a,b$ be two positive integers.
There exists a graph $G=(V,w)$ with $\mathcal{W} = \{-a,b\}$ such that any partition for $G$ is not $2(b+a+1)$-stable.
\end{lemma}

\iffalse
\begin{proof}
Our aim in this case is to emulate the variation of Figure~\ref{fig:fig-triangle} with the three weights $w_1 = b+a+1$, $w_2 = 2(b+a) + 3$, and $w_3 = 3(b+a+1)$.
As $b+a+1 < 2(b+a) + 3 < 3(b+a+1)$, and $b+a+1 + 2(b+a) + 3 = 3(b+a+1) +1 >  3(b+a+1)$, this change of weights does not make $2$-stable partitions exist for the graph.

To do that, let $t_1, t_2, t_3$ be any three positive integers that satisfy the following properties:
\begin{itemize}
\item $t_3 \geq t_2 \geq t_1$;
\item $t_1 \geq 5(b+a+1)/\max (b-a, 1)$;
\item $\max ( t_1b, (t_1+1)a + 2(b+a) + 3 ).a \geq (3(b+a)+2)b + 1$;
\item $\max ( t_2b, (t_2+1)a + 2(b+a) + 3 ).a \geq [(t_1+5)(b+a) + 4]b + 1$;
\item $\max ( t_3b, (t_3+1)a + 2(b+a) + 3 ).a \geq [(t_2+5)(b+a) + 4]b + 1$.   
\end{itemize}
We can note the possible values of those three integers are infinite.
Indeed, the value of $t_1$ can be any value that is greater than every of its (finite) lower bounds.
Furthermore, if the value of $t_1$ is arbitrarily fixed, then we can also choose for $t_2$ any value that is sufficiently large and, finally, the value of $t_3$ can be chosen in the same way, depending on the values of $t_1$ and $t_2$.

For every $1 \leq i \leq 3$, we also define the size $s_i = t_i(b+a) + 3(b+a+1) = (t_i+1)(b+a) + 2(b+a) + 3$.\\

\noindent
We now define the graph $G=(V,w)$. 
The vertices consist in three subsets $V_1,V_2$ and $V_3$, plus three other subsets $U_1,U_2$ and $U_3$.
All of them are cliques with weight $b$.
Furthermore, $U_i$ has size $b+a+1$ and $V_i$ has size $s_i$, for every $1 \leq i \leq 3$. 
There are also two distinct subcliques $V_{i,m} \subset V_{i,p} \subset V_i$, with $|V_{i,m}| = t_ib$, $|V_{i,p}| = (t_i+1)b$.

We set $w_{u,u'} = b$ for any $u,u' \in U_1 \cup U_2 \cup U_3$, and in addition, for every $1 \leq i \leq 3$:
\begin{itemize}
\item $w_{u_i,v_i} = b$ for every $u_i \in U_i$, $v_i \in V_i \setminus V_{i,m}$;
\item $w_{u_i,v_{i+1}} = b$, for every $u_i \in U_i$, $v_{i+1} \in V_{i+1} \setminus V_{i+1,p}$ (with the convention $V_{i+1} = V_1$ when $i=3$).
\end{itemize}
Every other weight equals $-a$.\\

\noindent
By contradiction.
Now assume there is a $2(b+a+1)$-stable partition of the nodes $P$.
By Lemma~\ref{lemma:group}, it comes that subsets $U_1,U_2,U_3, V_{1,m}, V_{2,m}, V_{3,m}, V_{1} \setminus V_{1,p},  V_{2} \setminus V_{2,p},  V_{3} \setminus V_{3,p}$ are subgroups in $P$.

\begin{claim}
For every $1 \leq i \leq 3$:
\begin{itemize} 
\item if $a \geq b$ then $|V_{i,p}| + 2(b+a+1) \leq | V_{i} \setminus V_{i,p}|$, 
\item if $b > a$ then $| V_{i} \setminus V_{i,m}| + 2(b+a+1) \leq |V_{i,m}|$.
\end{itemize} 
\end{claim}

\begin{proofclaim}
By the hypothesis, we have $|V_{i,p}| = (t_i+1)b$, hence $| V_{i} \setminus V_{i,p}| = s_i -  (t_i+1)b = (t_i+1)(b+a) + 2(b+a) + 3 - (t_i+1)b  =  (t_i+1)a + 2(b+a) + 3$; furthermore, $|V_{i,m}| = t_ib$, and so, $| V_{i} \setminus V_{i,m}| = s_i - t_ib =   t_i(b+a) + 3(b+a+1) - t_ib =  t_ia + 3(b+a+1)$. 

First if $a \geq b$, then $|V_{i,p}| + 2(b+a+1) =  (t_i+1)b + 2(b+a+1) < (ti+1)a + 2(b+a) + 3 = | V_{i} \setminus V_{i,p}|$, and the claim is proved. Otherwise, the equation $| V_{i} \setminus V_{i,m}| + 2(b+a+1) \leq |V_{i,m}|$ is equivalent to the following lines:
\[  t_ia + 3(b+a+1) +  2(b+a+1) \leq  t_ib\]
\[ 5(b+a+1) \leq t_i(b-a) \]
\[ 5(b+a+1)/(b-a) \leq t_i\]
and the claim is also proved, as $t_i \geq t_1 \geq  5(b+a+1)/\max (b-a, 1)$. 
\end{proofclaim}

In the sequel, we will denote $V_i' =  V_{i} \setminus V_{i,p}$ if $a \geq b$, and $V_i' = V_{i,m}$ if $b > a$.
We recall that $V_i'$ is a subgroup in $P$ by the previous claim.

\begin{claim}
For any $j < i$, none of the vertices in $V_j$ is in the same group in $P$ as vertices of $V_i'$.
\end{claim}

\begin{proofclaim}
Indeed, any vertex in $V_j$ has at most $s_j - 1 + 2(b+a+1) =  (t_j+1)(b+a) + 2(b+a) + 3 +  2(b+a+1) - 1 = (tj+5)(b+a) +4$ friends in its group.
Moreover, $[(tj+5)(b+a) +4]b < \max ( t_ib, (t_i+1)a + 2(b+a) + 3 ).a = |V_i'|a$ by the hypothesis.
\end{proofclaim}

\begin{claim}
Subsets $U_1$ and $V_3'$ are not in the same group in $P$.
\end{claim}

\begin{proofclaim}
By contradiction.
Suppose $U_1 \cup V_3'$ is a subgroup in $P$.
By the previous claim, there can be no vertex of $V_1 \cup V_2$ in this group.
Thus, any vertex of $U_1$ has at most $2(b+a+1) + b+a = 3(b+a) + 2$ friends in its group.
Furthermore, as $|V_3'|a = \max ( t_3b, (t_3+1)a + 2(b+a) + 3 ).a \geq (3(b+a)+2)b + 1$, we have that any vertex of $U_1$ has a negative utility, which is a contradiction because $P$ is $1$-stable.
\end{proofclaim}

In the same way, one can check that $U_2$ and $V_1'$ are not in the same group in $P$,  $U_3$ and $V_2'$ are not in the same group in $P$.

\begin{claim}
For any $1 \leq i \leq 3$, $V_i$ is a subgroup in $P$.
\end{claim}

\begin{proofclaim}
By our first claim, $|V_3 \setminus V_3'| + 2(b+a+1) \leq |V_3|'$, and by our third claim, there can be no vertex $u$ in the same group as $V_3'$ in $P$ such that $w_{u,v_3} = -a$ for any vertex $v_3 \in V_3$. 
Consequently, $V_3$ is a subgroup in $P$, as any vertex of $V_3 \setminus V_3'$ that would not be in the same group as $V_3'$ would break the partition. 
\end{proofclaim}

It directly follows that $V_2$ is a subgroup in $P$, hence $V_1$ is a subgroup in $P$.

Consequently, subsets $V_1,V_2,V_3,U_1,U_2$ and $U_3$ can be replaced with vertices $v_1,v_2,v_3,u_1,u_2$ and $u_3$ in the obvious way.
We get the variation of Figure~\ref{fig:fig-triangle} that we announced at the beginning of the proof.
Observe we can mimic any $2$-deviation involving nodes $u_1,u_2$ or $u_3$ in this reduced graph by a $2(b+a+1)$-deviation involving subsets $U_1,U_2$ or $U_3$ in $G$. 
So, there does not exist any $2(b+a+1)$-stable partition for $G$.
\iffalse
\begin{claim}
Given an $i$, $1 \leq i \leq 3$, if $A_i$ and $V_i$ are in the same group in $C$, then for any vertex $u_i \in A_i$, we get $f_C(u_i) \geq 3(b+a+1)b + (b+a)b$.
\end{claim}

It follows from $(|A_i|-1)b + |V_i \setminus V_{i,m}|b - |V_{i,m}|a = (b+a)b + (t_ia + 3(b+a+1))b - t_iba = 3(b+a+1)b +(b+a)b$.

In the same way, if $A_1$ and $V_2$ are in the same group, then for any vertex $u_1 \in A_1$, $f_C(u_1) \geq (|A_1|-1)b + |V_2 \setminus V_{2,p}|b - |V_{2,p}|a =  (b+a)b + ((t_2+1)a + 2(b+a) + 3)b - (t_2+1)b = (2(b+a)+3)b + (b+a)b$; if $A_2$ and $V_3$ are in the same group, then for any vertex $u_2 \in A_2$, $f_C(u_2) \geq  (2(b+a)+3)b + (b+a)b$; if $A_3$ and $V_1$ are in the same group, then for any vertex $u_3 \in A_3$, $f_C(u_3) \geq  (2(b+a)+3)b + (b+a)b$.

Finally, for every stable configuration $C$ for $G$, there is a corresponding configuration $C'$ for the counter-example of Lemma~\ref{lemma:extent}; moreover, we can mimic any $2$-deviation that breaks $C'$ by a $2(b+a+1)$-deviation that breaks $C$, and so, there does not exist any $2(b+a+1)$-stable configuration for $G$.
\fi
\end{proof}
\fi

Simpler constructions exist for the set $\{-a,0,b\}$.
They show that in this case, $k(\{-a,0,b\}) \leq 3$.
We will omit the proof in this paper.

Table~\ref{tab:tab-1} summarizes the most important tight values for $k(\mathcal{W})$. 
Note in particular that we prove $k(\mathcal{W})=\infty$ if and only if we have one of the following cases: $\mathcal{W}=\{-\infty,b\}$, which is equivalent to the uniform case; $\mathcal{W}$ has no negative (or no positive) elements, in which case the game is trivial; and $\mathcal{W} \subseteq -\mathbb{N} \cup \{N\}$, in which case the stable partition derives from connected components with edges of weight $N$.

More formally: 

\begin{table}[t]
\begin{center}
\noindent
\begin{tabular}{c|c}
%\hline
%\hline
$k(\mathcal{W})$ & $\mathcal{W}$ \\
\hline
%\hline
$1$ & $\{-M,a,b\}$, $0 < a < b$\\
\hline
$2$ &  $\{-M,-\mathbb{N},0,1\}$\\
\hline
$\infty$ & $\{-M,b\}$, $b > 0$; 
$\mathcal{W}\subseteq \NatInt$;
$\mathcal{W}\subseteq -\NatInt$;
$\mathcal{W} = -\NatInt\cup\{N\}$;
\\
\end{tabular}
\end{center}
\vspace{-0.4cm}
\caption{Values of $k(\mathcal{W})$ for different $\mathcal{W}$.}
\label{tab:tab-1}
\vspace{-0.2cm}
\end{table}


\begin{theorem}
\label{lem:car}
$k(\mathcal{W})=\infty$ if, and only if, $\mathcal{W} = \mathcal{W}^{+}$, or $\mathcal{W} = \mathcal{W}^{-}$, or $\mathcal{W} = \{-\infty, b\}$, or $\mathcal{W} = \mathcal{W}^{-} \cup \{N\}$ and $-\infty \notin \mathcal{W}$.
\end{theorem}

\iffalse
\begin{proof}
First, suppose that $\mathcal{W}$ is not of one of these forms.
Let $a,b$ be two positive integers.
If $-a,b \in \mathcal{W}$ then $k(\mathcal{W}) \leq 2(a+b) + 1$ by Lemma~\ref{lem:counter-example-3}.
So, we will assume either $-\infty$ is the only negative weight in $\mathcal{W}$, or $-\infty \in \mathcal{W}$ and $N$ is the only positive weight in $\mathcal{W}$.
In the first case, let $w_p$ denote the largest positive weight in $\mathcal{W}$; then, either there exists a positive integer $a < w_p$ such that $a \in \mathcal{W}$, hence $k(\mathcal{W}) = 1$ by Lemma~\ref{lemma:extent}, or $\mathcal{W} = \{-\infty,0,w_p\}$ and so, $k(\mathcal{W}) = 2$ by Corollary~\ref{lem:counter-example-2}.
In the second case, $k(\mathcal{W}) \leq 2$ by Corollary~\ref{cor:mn}.  
We deduce that $k(\mathcal{W})$ is upper-bounded in all the other cases, by the lemmas that are above in this section.\\

Now, for the 'if part', we start the proof with a preliminary remark.
Let $G = (V,w)$ be any graph, and let $P$ be any $1$-stable partition for $G$.
For any node $u \in V$, $f_{u}(P) \geq \sum_{v \in V}{\min(w_{u,v},0)}$ and $f_{u}(P) \leq \sum_{v \in V}{\max(w_{u,v},0)}$.\\

\noindent
Let $\mathcal{W} = \mathcal{W}^{+}$.
By the first remark, $f_{u}(P) \leq \\\sum_{v \in V}{\max(w_{u,v},0)}$ for any node $u \in V$ and for any stable partition $P$ for $G$.
In our case, $\sum_{v \in V}{\max(w_{u,v},0)} = \sum_{v \in V}{w_{u,v}}$ because $w_{u,v} \geq 0$ for any $uv \in E$.
Let $P = \{V\}$ be the partition for $G$ composed of $1$ group of size $n$.
By construction, for any node $u \in V$, $f_{u}(P) = \sum_{v \in V}{w_{u,v}}$.
Thus $P$ is a $k$-stable partition for $G$.
\iffalse
Consider $q \geq 2$.
Let $V = (u_{1}, \ldots, u_{n})$.
For any $u_{i} \in V$, $1 \leq i \leq n$, let $V^{i}_{1}, \ldots, V^{i}_{q-1}$ be $q-1$ singleton groups, each composed of node $u_{i}$.
Let $C=(V,V^{1}_{1}, \ldots, V^{1}_{q-1},V^{2}_{1}, \ldots, V^{2}_{q-1}, \ldots, V^{n}_{1}, \ldots, V^{n}_{q-1})$ be the configuration with $q$ channels for $G$.
Clearly, $C$ is $k$-stable because $w(u_{i},u_{}j) \geq 0$ and so $f_{u_{i}}(C) = \sum_{v \in V}{w(u,v)}$ for any $u_{i},u_{j} \in V$.
\fi\\

\noindent
Let $\mathcal{W} = \mathcal{W}^{-}$.
By the very first remark, $f_{u}(P) \leq \\\sum_{v \in V}{\max(w_{u,v},0)}$ for any node $u \in V$ and for any stable partition $P$ for $G$.
In our case, $\sum_{v \in V}{\max(w_{u,v},0)} = \sum_{v \in V}{0} = 0$ because $w_{u,v} \leq 0$ for any $uv \in E$.
Let us denote $V=\{u_{1}, \ldots, u_{n}\}$.
Let $P=\{\{u_{1}\}, \ldots,\{u_{n}\}\}$ be the partition for $G$ composed of $n$ groups of size $1$.
$P$ is a $k$-stable partition for $G$ because $f_{u}(P) = 0$ for any $u \in V$.\\

\noindent
The case $\mathcal{W} = \{-\infty, b\}$ is proved in~\cite{Kleinberg:2010ul}.\\

\noindent
Let $\mathcal{W} = \mathcal{W}^{-} \cup \{N\}$ such that $-\infty \notin \mathcal{W}$.
Let $G'=(V,E')$ be the graph induced by the set of arcs $E' = \{uv, w_{u,v}=N \}$.
Let $G_{1}, \ldots, G_{t}$ be the different connected components of $G'$.
Given a node $u \in V$, let $\Gamma_{G'}(u)$ be the set of neighbors of $u$ in graph $G'$.
Formally $\Gamma_{G'}(u) = \{v, uv \in E'\}$.
By the preliminary remark, we get that, for any stable partition $P$ for $G$ and for any node $u \in V$, $f_{u}(P) \leq N|\Gamma_{G'}(u)|$.

\noindent
Let $P= \{V(G_{1}), \ldots, V(G_{t})\}$ be the partition for $G$ composed of the nodes of the different maximal connected components of $G$.
By Definition of $N$, $f_{u}(P) \geq (N-1)|\Gamma_{G}(u)|$.

\noindent
We now prove that $P$ is $k$-stable.
By contradiction.
Suppose that there exists a $k$-deviation.
Let $P'$ be the partition for $G$ obtained after the $k$-deviation.
There are two cases.
\begin{itemize}
\item A subset $S \subset V(G_{i})$, for some $i$, $1 \leq i \leq t$, $|S| \leq k$, forms a new group.
In that case, we prove that at least one node $u \in S$ is such that $f_{u}(P') < f_{u}(P)$.
Indeed, consider a node $u \in S$ such that $\Gamma_{G'}(u) \cap S \neq \Gamma_{G'}(u)$.
Note that there always exists such a node because $|S| < |V(G_{i})|$ and $V(G_{i})$ is a maximal connected component of $G$.
Thus, we get $f_{u}(P') \leq (N-1)|\Gamma_{G'}(u)|$ while $f_{u}(P) \geq \max((N-1),0)|\Gamma_{G'}(u)|$.
So $f_{u}(P') \leq f_{u}(P)$.
A contradiction.
\item A subset $S \subset V$, $|S| \leq k$, reaches a group $V(G_{j})$, for some $i$, $1 \leq i \leq t$.
If $V(G_{i}) \cap S \neq \emptyset$, then we claim $V(G_{i}) \subset S$.
Otherwise, we would have $f_{P'}(u) \leq f_{u}(P)$ for some $u \in V(G_{i})$.
Indeed, consider a node $u \in S$ such that $\Gamma_{G'}(u) \cap S \neq \Gamma_{G'}(u)$.
So $f_{u}(P') \leq (N-1)|\Gamma_{G'}(u)|$ while $f_{u}(P) \geq (N-1)|\Gamma_{G'}(u)|$.
Thus, if $V(G_{i}) \cap S \neq \emptyset$, then $V(G_{i}) \subset S$.
Consider a set $V(G_{i})$, for some $i$, such that $V(G_{i}) \subset S$.
In that case, $f_{u}(P) \leq f_{u}(P')$ for any $u \in V(G_{i})$ because $w_{u,v} \leq 0$ for any $v \in V \setminus V(G_{i})$.
A contradiction.
\end{itemize}
There does not exist a $k$-deviation for $P$ and so $P$ is $k$-stable.
\end{proof}
\fi



% Also, note that the analysis above can be extended to the case without any conflict edges as well.
% Let us denote $W^{-}$ ($W^{+}$, respectively) any set of negative integers (positive integers, respectively).

% \vspace{-0.2cm}
% \begin{lemma}
% \label{lem:car}
% $k(\mathcal{W})=\infty$ $\Leftrightarrow$ $\mathcal{W} = W^{+}$, or $\mathcal{W} = W^{-}$, or $\mathcal{W} = \{-M, b\}$, or $\mathcal{W} = W^{-} \cup \{N\}$ and $-M \notin \mathcal{W}$.
% \end{lemma}
% \vspace{-0.2cm}


%%%%% TRANSFORMATION
%for which they do not exist any $k$-stable configuration.
%It is remarkable the construction of all these graphs uses the same pattern.
%In a way, the transformations that we introduce in this part show that changing the set of weights has few impact, at least in most cases.
%We also completely determine upper- and lower-bounds for $k(\mathcal{W})$.









%We can now present a counter-example that can be deduced from Lemma~\ref{lem:counter-example}.


%%%%% DEBUT DE COROLLAIRE COMMENTE %%%%%
\iffalse
\begin{corollary}
\label{cor:mn}
Let $\mathcal{W}$ be a set of weights, such that $\{-M,N\} \subset \mathcal{W}$.\footnote{Using a single channel, a weight $N$ denotes a best friend if $N > |V| \cdot \max\lset |w(u,v)| :  u,v\in V \rset$.}
There exists a graph $G=(V,E,w)$ such that any configuration for $G$ is not $3$-stable. 
\end{corollary}
\fi
%%%%% FIN DE COROLLAIRE COMMENTE %%%%%


%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
By Lemma~\ref{lem:counter-example}, there exists a graph $D_0 = (V_0,A_0,w_0)$ with $\{-M,0,1\}$ such that there does not exist any $3$-stable configuration for $D_0$.
Now, let $a \in \mathcal{W} \setminus \{-M,N\}$.
Note that $a$ may be positive or non positive.
We define $D_1 = (V_0,A_0,w_1)$ such that, for all vertices $u,v \in V_0$, $w_1(u,v) = -M$ if $w_0(u,v) = -M$,  $w_1(u,v) = N$ if $w_0(u,v) = 1$,  $w_1(u,v) = a$ if $w_0(u,v) = 0$.
As there does not exist any $3$-stable configuration with single channel for $D_0$, there does not exist any $3$-stable configuration for $D_1$ either.
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%




\iffalse
\begin{corollary}
Given two positive integers $a,b$ such that $a < b$, let $\mathcal{W} = \{-M,a,b\}$.
There exists a graph $D=(V,A,w)$ such that any configuration with single channel for $D$ is not $3$-stable. 
\end{corollary}

\begin{proof}
By Lemma~\ref{lem:counter-example}, there exists a graph $D_0 = (V_0,A_0,w_0)$ with $\{-M,0,1\}$ such that there does not exist any $3$-stable configuration for $D_0$.
Moreover, we get by the proof of Lemma~\ref{lem:counter-example} we can assume that, for any vertex $u \in V_0$, there exists at most one vertex $v \in V_0 \setminus \{u\}$ such that $w(u,v) = 0$.
We define $D_1 = (V_0,A_0,w_1)$ such that, for all vertices $u,v \in V_0$, $w_1(u,v) = -M$ if $w_0(u,v) = -M$,  $w_1(u,v) = b$ if $w_0(u,v) = 1$,  $w_1(u,v) = a$ if $w_0(u,v) = 0$.
Note that there is a trivial isomorphism between the configurations for $D_0$ and the configurations for $D_1$, as it is the same graph with a different set of weights.
Let $C_0$ be any configuration with single channel for $D_0$, and $C_1$ be its corresponding configuration with single channel for $D_1$. As $C_0$ is not $3$-stable for $D_0$, there exists a subset $S \subseteq V_0$, with $|S| \leq 3$, such that $S$ breaks $C_0$.
Let $C_0'$ be the new configuration for $D_0$ we get after the $3$-deviation, and $C_1'$ be its corresponding configuration for $D_1$.
By the hypothesis, we have that, for any $u \in S$, $f_u(C_0') \geq f_u(C_0) + 1$, hence $f_u(C_1') \geq b.f_u(C_0') \geq b.f_u(C_0) + b$, whereas $f_u(C_1) \leq b.f_u(C_0) + a <  b.f_u(C_0) + b$.
As a consequence, $S$ also breaks $C_1$, and there does not exist any $3$-stable configuration with single channel for $D_1$.
\end{proof}
\fi



%%%%% DEBUT DE CONSTRUCTION COMMENTEE %%%%%
\iffalse
Other counter-examples can be found using a more general transformation, that we describe below.

Let $G=(V,E,w)$ be a graph with any set $\mathcal{W}$, such that there is not other negative weight in $\mathcal{W}$ than $-M$.
The transformation of $G$ into the graph $G'$ with the set of weights $\{-M,0,1\}$ consists in replacing all the vertices $v \in V$ by a pair of friends $P_v = \{v,v'\}$, and all the edges $(u,v) \in E$ with a positive weight $w(u,v) > 0$ by a new set of vertices $UV$, with $|UV| = w(u,v)$.
We also add a clique of friends $K_{UV}$, whose members are enemies with all the vertices but those in $UV$.
%By construction, all the vertices in the same pair of friends $P_v$ will end in the same group, in any stable configuration with single channel $C'$ for $D'$.
The role of $K_{UV}$ is to prevent vertices in $UV$ to end in a group that does not contain both $P_u$ and $P_v$.

We then double the process, by adding the set $UV'$, and a clique of friends $K_{UV}'$.
That second copy must be enemy with the first one, so that vertices in $UV$ and in $UV'$ cannot be in the same group as $P_u$ and $P_v$ at the same time.
Figure~\ref{fig:transformation-0} describes the transformation for an arc $(u,v) \in V$ such that $w(u,v) > 0$.

\begin{figure}[h]
\centerline{\includegraphics[width=0.6\linewidth]{Figures/Transformation-0.pdf}}
\vspace{-0.4cm}
\caption{Transformation for (u,v) if w(u,v) $>$~0.}
\label{fig:transformation-0}
\vspace{-0.25cm}
\end{figure}

In so doing, we have there always is one of the subsets $UV$ or $UV'$ that agrees to break the current configuration with both $P_u$ and $P_v$, thus allowing us to mimic any possible $k$-deviation for $G$.
Finally, if there does not exist a $k$-stable configuration $C$   for $G$, then there does not exist a $k'$-stable configuration $C'$ for $G'$, where $k' \geq k$ is an integer that only depends on $k$ and on the original set $\mathcal{W}$.

In general, the value of $k'$ is far larger than $k$.
However there are many variants, that even though there are specific to some sets of weights $\mathcal{W}$, they allow to get counter-examples for smaller values of $k'$.
One of them is the following:
%%%%% FIN DE CONSTRUCTION COMMENTEE %%%%%
\fi


%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lemma:extent}
Given two positive integers $a,b$ such that $a < b$, there is a graph $D=(V,A,w)$ with $\mathcal{W} = \{-M,a,b\}$ such that there is no $2$-stable configuration for $D$.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%

%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
We build a graph $D=(V,A,w)$ as follows.
The set $V$ can be partitioned into four sets $A = \{a_1,a_2,a_3\}$, $B = \{b_1,v_2,v_3\}$, $C=\{c_1,c_2,c_3\}$ and $\{u_1,u_2,u_3\}$, such that all the edges between two vertices of the same subset have weight $b$.
Moreover, all the edges that lie between $A$ and $B$, $B$ and $C$, and $C$ and $A$ have weight $-M$.
We also set that for all vertices $a_i \in A$, for all vertices $b_j \in B$, and for all vertices $c_l \in C$, $w(a_i,u_1) = w(b_j,u_2) = w(c_l,u_3) = b$, whereas $w(a_i,u_3) = w(b_j,u_1) = w(c_l,u_2) = -M$.
Finally:
\begin{itemize}
\item $w(u_1,c_1) = w(u_1,c_2) = b$; $w(u_1,c_3) = a$;
\item $w(u_2,a_1) = w(u_2,a_2) = b$; $w(u_2,a_3) = a$;
\item $w(u_3,b_1) = w(u_3,b_2) = b$; $w(u_3,b_3) = a$.
\end{itemize}

Assume there exists a $2$-stable configuration $C_2$ for $D$.

We claim that $A,B$ and $C$ are subgroups in $C_2$.
Indeed, it is clear by Lemma~\ref{lemma:group} that $\{a_1,a_2\}, \{b_1,b_2\}, \{c_1,c_2\}$ are subgroups in $C$.
By symmetry, let us only consider the case of $a_3$.
Remark that all the vertices in $A$ share the same enemies in the graph.
Moreover, the sum of the positive weights that lie between $u_3$ and $V \setminus A$ equals $b+a$, which is lower than $2b$.
Hence $A$ is a subgroup of $C_2$ because $C_2$ is $1$-stable.

We now claim that, for any $u_i \in \{u_1,u_2,u_3\}$, there exists a subgroup $K \in \{A,B,C\}$ such that $K \subset C_2(u_i)$.
By symmetry, we only need to show it for $u_1$.
This is clear as $w(u_1,u_2) + w(u_1,u_3) = 2b < 2b + a$, and the enemies of $u_1$ are contained within the enemies of $A$ and $C$.

At last, we have either $A \cup \{u_1,u_2\}$ or $B \cup \{u_2,u_3\}$ or $C \cup \{u_3,u_1\}$ which is a group in $C_2$.
By symmetry, we can suppose  $A \cup \{u_1,u_2\}$ is a group in $C_2$.
Then, we have $\{u_2,u_3\}$ that breaks $C_2$, and so $C_2$ cannot be $2$-stable.
A contradiction.

As a consequence, there does not exist any $2$-stable configuration for $D$. 
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%





















\subsection{Intractability with conflict graphs}


%%%%% DEBUT DE DEFINITION COMMENTEE %%%%%
\iffalse
\begin{definition}
Let $D=(V,A,w)$ be a graph, and $u,v \in V$ be two vertices.
We say that $u$ and $v$ are \emph{twins} if and only if $w(u,v) > 0$ and for all vertex $s \in V$ $w(u,s) = w(v,s)$. 
\end{definition}
\fi
%%%%% FIN DE DEFINITION COMMENTEE %%%%%


%Informally, twins represent users that share the same interests.
%That notion is very general, and it will be reused later.
%The following lemma follows:


%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lemma:group}
Given a graph $D=(V,A,w)$, and a $1$-stable configuration  $C$ for $D$,
for all vertices $u,v$ such that $u$ and $v$ are twins, we have that $C(u) = C(v)$.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%


% Since we proved there are counter - examples for stability that quickly arise, most of them with only bilateral deviations, one may wonder whether it is tractable to decide whether there exists a $k$-stable configuration for a given graph. 
% We prove in Theorem~\ref{thm:complexity-decision} that any counter-example makes the following decision problem intractable:
Under general weights, we proved that it may not be easy to ensure that all games have a $k$-stable partition. We now prove a much stronger result: not only is the stability not guaranteed for a given game when $k>k(\mathcal{W})$, but it is computationally prohibitive to decide it. We first define:

\vspace{-0.2cm}
\begin{definition}[\SD]
Let $k \geq 1$ and let $\mathcal{W}$ be the (constant) set of weights.
Given a graph $G=(V,w)$, does there exist a $k$-stable partition for the nodes? 
\end{definition}
%\vspace{-0.2cm}

The following Theorem shows that $k(\mathcal{W})$ determines the complexity of the \SD.

\begin{theorem}
\label{thm:complexity-decision}
For $k \geq 1$ and $\mathcal{W}$ containing $-\infty$, either
\begin{itemize}
\vspace{-0.1cm}
\item a $k$-stable partition always exists (\ie $k\leq k(\mathcal{W})$);
\vspace{-0.1cm}
\item or the \SD is NP-hard.
\end{itemize}
\end{theorem}


A previous result of NP-hardness was proved in~\cite{Kleinberg:2010ul}.
However, their proof requires another kind of deviations in addition to the classical $k$-deviations we consider in our paper (see \emph{gossip deviations} in Section~\ref{sec:extensions}).
Moreover, the large positive weight $N$ is essential in their proof, whereas ours overrules these strong constraints.





\iffalse
\subsection{Complementary results without conflict edges}

Since the \SD is NP-hard whenever $-M \in \mathcal{W}$ and $k > k(\mathcal{W})$, it is natural to wonder whether the complexity gap holds if we omit that conflict weight $-M$.
The question is still open. 
However, Lemma~\ref{lem:counter-example-mix} shows how the previous counter-examples can be adapted when there are other negative weights than $-M$.
The case $\{-a,0,b\}$ is apart from the case $\{-a,b\}$, as the weight $0$ makes our transformation easier, and it allows us to upper-bound $k(\mathcal{W})$ by a constant that does not depend on $\mathcal{W}$.


Table~\ref{tab:tab-1} summarizes values of $k(\mathcal{W})$ for different $\mathcal{W}$.
We finally characterize in Lemma~\ref{lem:car}, the sets of weights such that, for any $k \geq 1$, there exists a $k$-stable configuration for any graph.
\fi







%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lem:counter-example-posnegzero}
Given two positive integers $a,b$, let $\mathcal{W}=\{-a,0,b\}$.
There exists a graph $G=(V,E,w)$ such that any configuration for $G$ is not $4$-stable.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%

%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
Let $s_1,s_2,s_3$ be three positive integers that satisfy the following four properties:
\begin{itemize}
\item $ s_1 \leq s_2 \leq s_3$;
\item $\max{(5b/a+4,11)} < s_1$;
\item $(s_1+3)b < (s_2-4)a$;
\item $(s_2+3)b < (s_3-4)a$.
\end{itemize}
We define the graph $D=(V,A,w)$ such that $V = V_1 \cup V_2 \cup V_3 \cup \{ a_1, a_2, b_1, b_2, c_1, c_2\}$, and for any $1 \leq i \leq 3$ $|V_i| = s_i$, as follows.

For every $1 \leq i \leq 3$, there is a distinct subclique of four vertices in $V_i$, namely: $\{v_{i,1}, v_{i,2}, v_{i,3}, v_{i,4}\}$;
furthermore, for all $v,v' \in V_i$, $w(v,v') = b$.
For any $1 \leq i < j \leq 3$, for any $u \in V_i$ and for any $v \in V_j$, $w(u,v) = -a$.

We also have that $w(u,v) = b$ for any $u,v \in  \{ a_1, a_2, b_1, b_2, c_1, c_2\}$, $u \neq v$.
We set:
\begin{itemize}
\item $w(a_1,v) = w(a_2,v) = b$ for any $v \in \{v_{1,1}, v_{1,2}, v_{1,3}, v_{1,4}\}$; 
\item $w(b_1,v) = w(b_2,v) = b$ for any $v \in \{v_{2,1}, v_{2,2}, v_{2,3}, v_{2,4}\}$;
\item $w(c_1,v) = w(c_2,v) = b$ for any $v \in \{v_{3,1}, v_{3,2}, v_{3,3}, v_{3,4}\}$.
\end{itemize}
Moreover: 
\begin{itemize}
\item $w(a_1,v) = w(a_2,v) = b$ for any $v \in  \{v_{2,1}, v_{2,2}, v_{2,3}\}$;
\item $w(b_1,v) = w(b_2,v) = b$ for any $v \in  \{v_{3,1}, v_{3,2}, v_{3,3}\}$; 
\item $w(c_1,v) = w(c_2,v) = b$ for any $v \in  \{v_{1,1}, v_{1,2}, v_{1,3}\}$.
\end{itemize}
We also set $w(a_1,v) = w(a_2,v) = -a$ for any $v \in V_3$, $w(b_1,v) = w(b_2,v) = -a$ for any $v \in V_1$, $w(c_1,v) = w(c_2,v) = -a$ for any $v \in V_2$.
Finally, any other weight $w(u,v)$ equals $0$.\\

\noindent
Let $C$ be a stable configuration with single channel for $D$.
By Lemma~\ref{lemma:group}, $V_i' = V_i \setminus \{v_{i,1}, v_{i,2}, v_{i,3}, v_{i,4}\}$ is a subgroup in $C$, for any $1 \leq i \leq 3$. We also have by Lemma~\ref{lemma:group} $\{a_1,a_2\}$, $\{b_1,b_2\}$ and $\{c_1,c_2\}$ are subgroups in $C$.
Furthermore, if $i < j$, then we claim any vertex $v$ of $V_i$ is not in the same group as $V_j'$.
Indeed, $v$ has at most $(s_i+3)$ friends in its group by the hypothesis, whereas $|V_j'|a =  (s_j-4)a > (s_i+3)b$.
 
Similarly, we claim $a_1$ and $a_2$ are not in the same group as $V_3'$.
By contradiction.
Suppose $a_1$ and $a_2$ are in the same group as $V_3'$.
There can be no vertex of $V_1 \cup V_2$ in the same group as $V_3'$.
Hence, $a_1$ and $a_2$ have at most $5$ friends in their groups (including each other), whereas $|V_3'|a = (s_3-4)a > 5b$.
A contradiction, because $f_{a_1}(C) = f_{a_2}(C) \geq 0$.
By symmetry, we get $b_1$ and $b_2$ are not in the same group as $V_1'$, $c_1$ and $c_2$ are not in the same group as $V_2'$.

Furthermore, if $v_{3,j}$ were not in the same group as $V_3'$ in $C$, for some $1 \leq j \leq 4$, we would have $f_C(v_{3,j}) \leq 7b$, whereas $|V_3'| = s_3 - 4 \geq 8$, and thus $\{v_{3,j}\}$ would break the configuration, as there can be no vertex $u$ in the same group as $V_3'$ such that $w(u,v) = -a$ for any $v \in V_3$.
As it is a contradiction, we get $V_3$ is a subgroup in $C$, and so, $V_2$ is a subgroup in $C$, hence $V_1$ is a subgroup in $C$.
In other words, we proved that: 
\begin{itemize}
\item $V_1$, $V_2$, $V_3$, $\{a_1,a_2\}$, $\{b_1,b_2\}$ and $\{c_1,c_2\}$ are subgroups in $C$;
\item $V_1, V_2, V_3$ are in three different groups in $C$;
\item $a_1$ and $a_2$ cannot be in the same group as $V_3$;
\item $b_1$ and $b_2$ cannot be in the same group as $V_1$;
\item $c_1$ and $c_2$ cannot be in the same group as $V_2$.
\end{itemize}

Thus, we can associate to $C$ a stable configuration $C'$ for the counter-example of Lemma~\ref{lemma:extent}, and we can mimic any $2$-deviation in $C'$ by a $4$-deviation in $C$. Finally, there does not exist any $4$-stable configuration for $D$, because there is no $2$-stable configuration for  the counter-example of Lemma~\ref{lemma:extent}.
\end{proof}
\fi
%%%%% FIN DE PREUVE COMMENTEE %%%%%




%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lem:counter-example}
Given two positive integers $a,b$, let $\mathcal{W}=\{-a,b\}$.
There exists a graph $G=(V,E,w)$ such that any configuration for $G$ is not $2(b+a+1)$-stable.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%








%%%%% DEBUT DE LEMME COMMENTE %%%%%
\iffalse
\begin{lemma}
\label{lem:car}
$k(\mathcal{W})=\infty$ if, and only if, $\mathcal{W} = W^{+}$, or $\mathcal{W} = W^{-}$, or $\mathcal{W} = \{-M, b\}$, or $\mathcal{W} = W^{-} \cup \{N\}$ and $-M \notin \mathcal{W}$.
\end{lemma}
\fi
%%%%% FIN DE LEMME COMMENTE %%%%%

%%%%% DEBUT DE PREUVE COMMENTEE %%%%%
\iffalse
\begin{proof}
First note that any other $\mathcal{W}$ is such that $k(\mathcal{W})$ is upper-bounded, by the lemmas that are above in this section.
We start the proof with a preliminary remark.
Let $D = (V,A,w)$ be any graph, and let $C$ be any configuration for $D$.
For any node $u \in V$, $f_{u}(C) \geq \sum_{v \in V}{\min(w(u,v),0)}$ and $f_{u}(C) \leq \sum_{v \in V}{\max(w(u,v),0)}$.\\

\noindent
Let $\mathcal{W} = W^{+}$.
By the first remark, $f_{u}(C) \leq \\\sum_{v \in V}{\max(w(u,v),0)}$ for any node $u \in V$ and for any configuration $C$ for $D$.
In our case, $\sum_{v \in V}{\max(w(u,v),0)} = \sum_{v \in V}{w(u,v)}$ because $w(u,v) \geq 0$ for any $(u,v) \in A$.
Let $C = (V)$ be the configuration for $D$ composed of $1$ group of size $|V|$.
For any node $u \in V$, $f_{u}(C) = \sum_{v \in V}{w(u,v)}$.
Thus $C$ is a $k$-stable configuration for $D$.
\iffalse
Consider $q \geq 2$.
Let $V = (u_{1}, \ldots, u_{n})$.
For any $u_{i} \in V$, $1 \leq i \leq n$, let $V^{i}_{1}, \ldots, V^{i}_{q-1}$ be $q-1$ singleton groups, each composed of node $u_{i}$.
Let $C=(V,V^{1}_{1}, \ldots, V^{1}_{q-1},V^{2}_{1}, \ldots, V^{2}_{q-1}, \ldots, V^{n}_{1}, \ldots, V^{n}_{q-1})$ be the configuration with $q$ channels for $D$.
Clearly, $C$ is $k$-stable because $w(u_{i},u_{}j) \geq 0$ and so $f_{u_{i}}(C) = \sum_{v \in V}{w(u,v)}$ for any $u_{i},u_{j} \in V$.
\fi\\

\noindent
Let $\mathcal{W} = W^{-}$.
By the very first remark, $f_{u}(C) \leq \\\sum_{v \in V}{\max(w(u,v),0)}$ for any node $u \in V$ and for any configuration $C$ for $D$.
In our case, $\sum_{v \in V}{\max(w(u,v),0)} = \sum_{v \in V}{0} = 0$ because $w(u,v) \leq 0$ for any $(u,v) \in A$.
Let $V=\{u_{1}, \ldots, u_{n}\}$.
By assumption, for any node $u \in V$ and for any configuration $C$ for $D$, $f_{u}(C) \leq 0$ because $w(u,v) \leq 0$ for any $v \in V$.
Let $C=(\{u_{1}\}, \ldots,\{u_{n}\})$ be the configuration for $D$ composed of $|V|$ groups of size $1$.
$C$ is a $k$-stable configuration for $D$ because $f_{u}(C) = 0$ for any $u \in V$.\\

\noindent
The case $\mathcal{W} = \{-M, b\}$ is proved in~\cite{Kleinberg:2010ul}.\\

\noindent
Let $\mathcal{W} = W^{-} \cup \{N\}$ such that $-M \notin \mathcal{W}$.
Let $G=(V,E)$ be the graph induced by the set of arcs $E = \{(u,v), w(u,v)=N, (u,v) \in A\}$.
Let $G_{1}, \ldots, G_{t}$ be the different connected components of $G$.
Given a node $u \in V$, let $\Gamma_{G}(u)$ be the set of neighbors of $u$ in graph $G$.
Formally $\Gamma_{G}(u) = \{v, (u,v) \in E\}$.
By the preliminary remark, we get that, for any configuration $C$ for $D$ and for any node $u \in V$, $f_{u}(C) \leq N|\Gamma_{G}(u)|$.

\noindent
Let $C= (V(G_{1}), \ldots, V(G_{t}))$ be the configuration for $D$ composed of the nodes of the different maximal connected components of $G$.
By Definition of $N$, $f_{u}(C) \geq \max((N-1),0)|\Gamma_{G}(u)|$.

\noindent
We now prove that $C$ is $k$-stable.
By contradiction.
Suppose that there exists a $k$-deviation.
Let $C'$ be the configuration for $D$ obtained after the $k$-deviation.
There are two cases.
\begin{itemize}
\item A subset $S \subset V(G_{i})$, for some $i$, $1 \leq i \leq t$, $|S| \leq k$, forms a new group.
In that case, we prove that at least one node $u \in S$ is such that $f_{C'}(u) < f_{u}(C)$.
Indeed, consider a node $u \in S$ such that $\Gamma_{G}(u) \cap S \neq \Gamma_{G}(u)$.
Note that there always exists such a node because $|S| < |V(G_{i})|$ and $V(G_{i})$ is a maximal connected component of $G$.
Thus, we get $f_{C'}(u) \leq \max((N-1),0)|\Gamma_{G}(u)|$ while $f_{u}(C) \geq \max((N-1),0)|\Gamma_{G}(u)|$.
So $f_{C'}(u) \leq f_{u}(C)$.
A contradiction.
\item A subset $S \subset V$, $|S| \leq k$, reaches a group $V(G_{j})$, for some $i$, $1 \leq i \leq t$.
If $V(G_{i}) \cap S \neq \emptyset$, then $V(G_{i}) \subset S$.
Otherwise, we would have $f_{C'}(u) \leq f_{u}(C)$ for some $u \in V(G_{i})$.
Indeed, consider a node $u \in S$ such that $\Gamma_{G}(u) \cap S \neq \Gamma_{G}(u)$.
So $f_{C'}(u) \leq \max((N-1),0)|\Gamma_{G}(u)|$ while $f_{u}(C) \geq \max((N-1),0)|\Gamma_{G}(u)|$.
Thus, if $V(G_{i}) \cap S \neq \emptyset$, then $V(G_{i}) \subset S$.
Consider a set $V(G_{i})$, for some $i$, such that $V(G_{i}) \subset S$.
In that case, $f_{u}(C) \leq f_{C'}(u)$ for any $u \in V(G_{i})$ because $w(u,v) \leq 0$ for any $v \in V \setminus V(G_{i})$.
A contradiction.
\end{itemize}
There does not exist a $k$-deviation for $C$ and so $C$ is $k$-stable.
\end{proof}
\fi
%%%%% DEBUT DE PREUVE COMMENTEE %%%%%






\iffalse
Finally, we prove the inexistence of a $k$-stable configuration for, at least, one graph $D$ with $\mathcal{W}$ for some integer $k$, makes the problem intractable for set of weights $\mathcal{W} \cup \{-M,0,1\}$ and any $k' \geq k$.
Thus, the counter example described in Figure~\ref{fig:counter-examples} and proved in Lemma~\ref{lem:counter-example}, shows that:

\begin{theorem}
\label{the:counter-ex-implies:np}
Deciding whether there exists a $3$-stable configuration with single channel for a given graph $D=(V,A,w)$ with $\mathcal{W}=\{-M,0,1\}$ is NP-hard. 
\end{theorem}



\begin{proof}
Let $G=(V_{G},E_{G})$ be a graph and $c \leq |V_G|$ be an integer.
By Lemma~\ref{lem:counter-example}, there is a graph $D_0 = (V_0,A_0,w_0)$ with $\mathcal{W}=\{-M,0,1\}$ that does not admit a $3$-stable configuration with single channel.
Furthermore, we can assume that there exists a node $x \in V_{0}$ such that the removal of $x$ makes the existence of a $3$-stable configuration for the gotten subgraph.
Indeed, otherwise, we remove nodes sequentially until obtaining this property.
We now assume the number of friends $v$ of this vertex $x$ in $D_0$ is $n_f \leq |V_0| - 1$.

We build the graph $D = (V,A,w)$, with $V = V_0 \cup V_G \cup V_{x} \cup \{x_1, \ldots, x_{n_f}\}$, such that $|V_x| = c+1$. 
For all vertices $u_0,v_0 \in V_0$, we set $w(u_0,v_0) = w_0(u_0,v_0)$.
Moreover, for any vertex $v_0 \in V_0 \setminus \{x\}$, for any vertex $u \notin V_0$, $w(v_0,u) = -M$.
We also set, for any $1 \leq i < j \leq n_f$, $w(x,x_i) = w(x,x_j) = 1$, $w(x_i,x_j) = 0$, and for any $v_x \in V_x$, $w(x_i,v_x) = w(x_j,v_x) = 1$, $w(x,v_x) = -M$.
The set $V_x$ is a clique of $c+1$ friends;
furthermore, for any $v_x \in V_x$, for any $v$ of $V_G$, and for any $1 \leq i \leq n_f$, we set $w(v_x,v) = -M$, $w(x_i,v) = 1$.
Finally, for all vertices $u,v \in G$, $w(u,x) = w(v,x) = 0$, $w(u,v) = -M$ if $(u,v) \in E_G$, $w(u,v) = 1$ otherwise.
The graph $D$ is described in Figure~\ref{fig:hard}.

We note that all the vertices in $V_x$ end in the same group in $C$, with $C$ being any stable configuration.
We also get that either the club of $x_i$ in $C$ is a subset of $V_x \cup \{x_1,\ldots, x_{n_f}\}$, or it is a subset of $\{x,x_1,\ldots, x_{n_f}\} \cup V_G$.
However, a necessary condition for having $x_i$ not in the same group as vertices in $V_x$ in $C$ is there is, at least, $c$ vertices of $V_G$ in the same group as $x_i$ in $C$. 
Thus, if the size of any independent set in $G$ is at most $c-1$, then $V_x \cup \{x_1,\ldots, x_{n_f}\}$ is a group of $C$.
Hence, vertices in the same group as $x$ are vertices in $V_0$ and so, $C$ is not $3$-stable, because there does not exist a $3$-stable configuration with single channel for $D_0$.

Now assume there is an independent set in $G$ of size larger than $c$.
We identify $G$ to a graph $D_G$ with $\mathcal{W}=\{-M,1\}$ and, by~\cite{Kleinberg:2010ul}, there exists a configuration with single channel $C_G$ for $D_G$, such that $C_G$ is $k$-stable for any $k \geq 1$, and there exists a group $V_{IS}$ in $C_G$ that is a maximum independent set in $G$.
Finally, $C = (C_{G} \setminus V_{IS} \cup (V_{IS} \cup \{x,x_1,\ldots, x_{n_f}\}) \cup (V_x) \cup C_{1})$ is a $3$-stable configuration with single channel for $D$, with $C_{1}$ being a $3$-stable configuration with single channel for $D_{1} = (V_0 \setminus \{x\}, A_0, w_0)$.

We can conclude the NP-hardness, as our transformation is polynomial, and the \MIS is NP-complete~\cite{Kar72}.
\end{proof}

\begin{figure}[t]
\centerline{\includegraphics[width=0.5\linewidth]{Figures/hardness.pdf}}
\vspace{-0.25cm}
\caption{Graph D for the proof of Theorem~\ref{the:counter-ex-implies:np}.}
\label{fig:hard}
\end{figure}

\fi




\iffalse
\subsection{Extension to multi-channel}

It is now natural to wonder what is the behavior of $k(\mathcal{W})$ when the number of channels is higher than $1$.
While it may have none or positive effects for trivial examples of function $h$ that are super-linear, we will show that it is not always the case, even if the function $h$ is as simple as $h(0,w) = 0$, $h(g+1,w) = (1 + \varepsilon g)w$, where $\varepsilon > 0$ is arbitrarily small\footnote{$M$ must be taken as large as $\varepsilon$ is small, for we should have $\varepsilon M > |V|\cdot h(q,\max\lset w(u,v)\dimset u,v\in V \rset )$ if we want to avoid that two vertices $u,v$ such that $w(u,v) = -M$ end in the same group.}.
We prove in this case an increasing number of channels has a negative impact on the upper-bound of $k(\mathcal{W})$.
Indeed, even for $\mathcal{W}=\{-M,1\}$, Lemma~\ref{lem:contre-exemple-q=2} proves $k(\mathcal{W}) \leq 2$ with $2$ channels while $k(\mathcal{W}) = \infty$ with single channel. 
The idea is to emulate a weight $w(u,v) = 0$ by forcing nodes $u$ and $v$ to be in a predetermined group.

\begin{lemma}
\label{lem:contre-exemple-q=2}
There exists a graph $D=(V,A,w)$ with $\mathcal{W}=\{-M,1\}$ such that any configuration with $2$ channels for $D$ is not $3$-stable.
\end{lemma}



\begin{proof}
We use the counter-example $D_{q=1}=\\(V_{q=1},A_{q=1},w_{q=1})$ of Lemma~\ref{lem:counter-example} for the proof.
Note that, for each node $u \in V_{q=1}$, there exists at most one node $v \in V_{q=1}$ such that $w_{q=1}(u,v) = 0$.

Given a clique $K=(V,A)$ or order $p > 2|V_{q=1}|$, we set $w(u,v) = 1$ for any $u,v \in V$.
We now assume that $\varepsilon < 1/p$ for the rest of the proof, and we construct the graph $D_{q=2}=(V_{q=2},A_{q=2},w_{q=2})$ as follows.
For any node $u \in V_{q=1}$ such that $w_{q=1}(u,v) \neq 0$ for any $v \in V_{q=1}$, we add a copy of $K$, denoted $K_{u}=(V_{u},A_{u})$.
We set $w_{q=2}(u,x) = 1$ for any $x \in V_{u}$.
For any edge $(u,v) \in A_{q=1}$ such that $w_{q=1}(u,v) = 0$, we add another copy of $K$, denoted $K_{(u,v)}=(V_{(u,v)},A_{(u,v)})$.
We set $w_{q=2}(u,x) = w_{2}(v,x) = 1$ for any $x \in V_{(u,v)}$.
Furthermore, we set $w_{q=2}(u,v) = 1$.
Finally, for any graph $K_{u}$, with $u \in V_{q=1}$, we set $w_{q=2}(y,x) = -M$ for any $y \in V_{q=1} \setminus \{u\}$ and for any $x \in V_{u}$.
Similarly, for any graph $K_{(u,v)}$, with $(u,v) \in A_{q=1}$, we set $w_{q=2}(y,x) = -M$ for any $y \in V_{q=1} \setminus \{u,v\}$ and for any $x \in V_{(u,v)}$.\\

\noindent
First, we get that for any $u,v \in V_{q=1}$ such that $w(u,v) = 0$, for any $x,y \in V_{(u,v)}$, $|C(x) \cap C(y)| = 2$  in any $3$-stable configuration $C = (V_{1}, \ldots, V_{c})$ with $2$ channels for $D_{q=2}$.

As $\epsilon M > n$, we have that any $x \in V_{(u,v)}$ cannot be in a group containing any node $y \in V_{q=2} \setminus (A_{(u,v)} \cup \{u,v\})$.

We first prove that in any $3$-stable configuration $C=(V_1,\ldots,V_c)$ with $2$ channels for $D_{q=2}$, we have $|C(x) \cap C(y)| \neq 1$, for any $x,y \in V_{(u,v)}$.
By contradiction.
Assume there exist $x,y \in V_{(u,v)}$ such that $|C(x) \cap C(y)| = 1$.
Without loss of generality, assume that $f_x(C) \geq f_y(C)$.
Then, there exists a $1$-deviation: $y$ reaches the group $V_i$ such that $x \in V_i$ and $y \notin V_i$.
In that case, $f_y(C') > f_y(C)$, where $C'$ is the configuration for $D$ after the previous $1$-deviation.
Indeed, $f_y(C') = f_x(C) + \epsilon$.

Thus, we assume that, in any $3$-stable configuration $C=(V_1,\ldots,V_c)$ with $2$ channels for $D_{q=2}$, we have $|C(x) \cap C(y)| \neq 1$, for any $x,y \in V_{(u,v)}$.
Furthermore, if there exist $x,y \in V_{(u,v)}$ such that $|C(x) \cap C(y)| = 0$, then there exist two groups $V_{x_1}$ and $V_{x_2}$ such that $x \in V_{x_1}$, $x \in V_{x_2}$, and $V_{x_1} = V_{x_2}$, and there exist two groups $V_{y_1}$ and $V_{y_2}$ such that $y \in V_{y_1}$, $y \in V_{y_2}$, and $V_{y_1} = V_{y_2}$.
Thus, $f_x(C) = (1+\epsilon)(|V_{x_1}|-1)$, and $f_y(C) = (1+\epsilon)(|V_{y_1}|-1)$.
Without loss of generality, suppose $f_x(C) \geq f_y(C)$.
Then, there exists a $1$-deviation: $y$ leaves $V_{y_1}$ and reaches $V_{x_1}$.
We get $f_y(C') = |V_{x_1}| + |V_{y_2}| - 1 > f_y(C)$ because $\epsilon < \frac{1}{p}$.
Thus, in any $3$-stable configuration $C=(V_1,\ldots,V_c)$ with $2$ channels for $D_{q=2}$, we have for any $x,y \in V_{(u,v)}$, $|C(x) \cap C(y)| = 2$, and so, the claim is proved.\\

\noindent
Then, by the choice of $0 < \varepsilon < 1/p$ with $p > 2|V_{1}|$, there exist two groups $V_{i}$ and $V_{j}$, $1 \leq i < j \leq c$, such that $V_{i} = V_{(u,v)}$ and $V_{j} = V_{(u,v)} \cup \{u,v\}$.
Indeed, otherwise there exists a $1$-deviation for $C$, because by construction $|V_{(u,v)}| > f_{u}(C')$, with $C'$ being any configuration with $2$ channels for $D_{q=1}$.
We obtain the same result for copies $K_{u}$.
To summarize, after setting the groups from the previously necessary conditions for having a $3$-stable configuration with $2$ channels for $D_{q=1}$, each node $u \in V \setminus V_{q=1}$ belongs to exactly $2$ groups, and each node $u \in V_{q=1}$ belongs to exactly $1$ group.

Thus, there exists a $3$-stable configuration for $D_{q=2}$ with $2$ channels if, and only if, there exists a $3$-stable configuration for $D_{q=1}$ with single channel.
Indeed, any two nodes $u,v \in V_{q=1}$ such that $w_{q=1}(u,v) = 0$, are already in a same group.
Thus, by the choice of the function $h$, this mimics a weight $\varepsilon$ between these two nodes for determining the other groups, that is quite the same as a weight $0$, because $\varepsilon$ is arbitrarily small (see Corollary \ref{cor:mn}).
Finally, there does not exists a $3$-stable configuration for $D_{q=2}$ with $2$ channels because there does not exist a $3$-stable configuration for $D_{q=1}$ with single channel by Lemma~\ref{lem:counter-example}.
\end{proof}


We prove that any chaotic behavior may be observed between any two consecutive numbers of channels.

\begin{lemma}
\label{lemma:counter-symmetric-1}
Let $W=\{-M,-4,2,6,7\}$.
There exists a graph $D=(V,A,w)$ such that any configuration $C$ with single channel for $D$ is not $2$-stable.
\end{lemma}

\begin{proof}
Let $D=(V,A,w)$ be the graph built as follows.
Let $V=\{u_{1},u_{2},u_{3},u_{4}\}$.
We set $w(u_{1},u_{2}) = w(u_{1},u_{3}) = -M$, $w(u_{1},u_{4})=7$, $w(u_{2},u_{4})=6$, $w(u_{3},u_{4})=2$, and $w(u_{2},u_{3})=-4$.

For any $k \geq 1$, any $k$-stable configuration $C$ with single channel for $D_1$ is such that $f_{C}(u) \geq 0$ for any $u \in V$.
Thus, for any $k \geq 1$, the following configurations for $D$ are not $k$-stable:
\begin{itemize}
\item $C=(\{u_{1}\},\{u_{2},u_{3},u_{4}\})$ as $f_{u_3}(C) = -2 < 0$;
\item $C=(\{u_{1}\},\{u_{2},u_{3}\},\{u_{4}\})$ as $f_{u_3}(C) = -4 < 0$;
\item $C=(\{u_{1},u_{4}\},\{u_{2},u_{3}\})$ as $f_{u_3}(C) = -4 < 0$;
\item any configuration $C=(V_{1},V_{2},V_{3},V_{4})$ ($V_{i}$ may be empty for some $i$, $1 \leq i \leq 4$) such that $u_{1},u_{2} \in V_{i}$ and/or $u_{1},u_{3} \in V_{i}$ for some $i$, $1 \leq i \leq 4$.
\end{itemize}

Thus, it remains to prove the result for the other configurations for $D$.
\begin{itemize}
\item Consider the configuration $C=(\{u_{1}\},\{u_{2}\},\{u_{3}\},\{u_{4}\})$ for $D$.
$C$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(C') = f_{u_4}(C) + 7 = 7$ where $C'=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ is the resulting configuration with single channel for $D$ after this $1$-deviation.

\item Consider the configuration $C=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ for $D$.
$C$ is not $2$-stable because $u_{2}$ and $u_{4}$ can reach group $\{u_{3}\}$.
Indeed, $f_{u_2}(C') = f_{u_2}(C) + 6 - 4 = f_{u_2}(C) + 2 = 2$ and $f_{u_4}(C') = f_{u_4}(C) -7 + 6 + 2 = f_{u_4}(C) + 1 = 8$ where $C'=(\{u_{1}\},\{u_{2},u_{3},u_{4}\})$ is the resulting configuration for $D$ after this $2$-deviation.

\item Consider the configuration $C=(\{u_{1}\},\{u_{2},u_{4}\},\{u_{3}\})$ for $D$.
$C$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(C') = f_{u_4}(C) -6 + 7 = f_{u_4}(C) + 1 = 7$ where $C'=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ is the resulting configuration for $D$ after this $1$-deviation.

\item Consider the configuration $C=(\{u_{1}\},\{u_{2}\},\{u_{3},u_{4}\})$ for $D$.
$C$ is not $1$-stable because $u_{4}$ can reach group $\{u_{1}\}$.
Indeed, $f_{u_4}(C') = f_{u_4}(C) -2 + 7 = f_{u_4}(C) + 5 = 7$ where $C'=(\{u_{1},u_{4}\},\{u_{2}\},\{u_{3}\})$ is the resulting configuration for $D$ after this $1$-deviation.
\end{itemize}

Finally, any configuration $C$ with single channel for $D$ is not a $2$-stable configuration for $D$.
\end{proof}

\begin{corollary}
\label{cor:base}
Let $W=\{-M,-4,2,6,7\}$.
Given an integer $q \geq 1$, there exists a graph $D_q=(V_q,A_q,w_q)$ such that any configuration $C$ with $q$ channels for $D$ is not $2$-stable, whereas there always exists a $2$-stable configuration $C'$ with $q' \neq q$ channels for $D$.
\end{corollary}

\begin{proof}
We arbitrarily select $\epsilon < 1/N$.
Let $D_1 = (V_1,A_1,w_1)$ be the graph that is presented in the proof of Lemma~\ref{lemma:counter-symmetric-1} (we re-use the same notations for the vertices in $D_1$).
We build the graph $D_q$ as follows.
First, the set of vertices is $V_q = V_1 \cup \{x_1, \ldots, x_{q-1}\}$.
For any $u,v \in V_1$, $w_q(u,v) = w_1(u,v)$.
Furthermore, for any $1 \leq i < j \leq q-1$, $w(x_i,u_4) = w(x_j,u_4) = N$, $w(x_i,x_j) = w(x_i,v) = w(x_j,v) = -M$ for any $v \in V_1 \setminus \{u_4\}$.

We have that, for any $q' < q$, $C_{q'} = ( \{u_4,x_1\}, \ldots, \{u_4,x_{q'}\}, \\\{u_1\}^1, \ldots, \{u_1\}^{q'}, \{u_2\}^1, \ldots, \{u_2\}^{q'}, \{u_3\}^1, \ldots, \{u_3\}^{q'}, \\ \{x_1\}^1, \ldots, \{x_1\}^{q'-1}, \ldots, \{x_{q'}\}^1, \ldots, \{x_{q'}\}^{q'-1}, \\\{x_{q'+1}\}^1, \ldots, \{x_{q'+1}\}^{q'}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'})$ is a $2$-stable configuration with $q'$ channels for $D_q$.

However, in any stable configuration $C_q$ with $q$ channels for $D_q$, we necessarily have $\{u_4,x_i\}$ as a group in $C_q$ (without repetitions), for any $1 \leq i \leq q-1$. As there does not exist any $2$-stable configuration with single channel for $D_1$, there does not exist any $2$-stable configuration with $q$ channels for $D_q$.

If $q' = q+1$, then $C_{q'} = ( \{u_4,x_1\}, \ldots, \{u_4,x_{q-1}\},\\\{u_4,u_1\}, \{u_4,u_2\}, \{u_1\}^1, \ldots, \{u_1\}^{q'-1}, \{u_2\}^1, \ldots, \{u_2\}^{q'-1}, \\\{u_3\}^1, \ldots, \{u_3\}^{q'}, \{x_1\}^1, \ldots, \{x_1\}^{q'-1}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'-1})$ is a $2$-stable configuration with $q'$ channels for $D_q$.

Finally, if $q' \geq q+2$, then $C_{q'} = ( \{u_4,x_1\}^1, \ldots, \{u_4,x_1\}^{q'-q-1}, \\\{u_4,x_2\}, \ldots, \{u_4,x_{q-1}\},\{u_4,u_1\}, \{u_4,u_2\}, \{u_4,u_3\}, \{u_1\}^1, \ldots, \\\{u_1\}^{q'-1}, \{u_2\}^1, \ldots, \{u_2\}^{q'-1}, \{u_3\}^1, \ldots, \{u_3\}^{q'-1}, \{x_1\}^1, \ldots, \\\{x_1\}^{q+1}, \{x_2\}^1, \ldots, \{x_2\}^{q'-1}, \ldots, \{x_{q-1}\}^1, \ldots, \{x_{q-1}\}^{q'-1})$ is a $2$-stable configuration with $q'$ channels for $D_q$.
\end{proof}

\begin{theorem}
For any sequence of positive integers $q_{1}, q_{2}, \ldots, q_{p}$, and for any sequence $1 \leq i_{1} < i_{2} < \ldots < i_{l} \leq p$, there exists a graph $D=(V,A,w)$ such that there is a $2$-stable configuration with $q_j$ channels for $D$ if, and only if, $j \neq i_{t}$, for every $1 \leq t \leq l$.
\end{theorem}

\begin{proof}
For any $1 \leq t \leq l$, let $D_{q_{i_t}}$ be the graph in the proof of Corollary~\ref{cor:base} such that there exists a $2$-stable configuration with $q'$ channels for $D_{q_{i_t}}$ if, and only if, $q' \neq q_{i_t}$.
By convention, $D_0$ is any graph such that there always is a $2$-stable configuration with $q$ channels for $D_0$; for instance, we may assume that all the weights for $D_0$ are positive.

Then we build a graph $D$ from $D_0, D_{q_{i_1}}, \ldots D_{q_{i_l}}$, such that any vertices $u,v$ that are not in the same graph $D_q$ are enemies (e.g. $w(u,v) = -M$).
In so doing, every graph $D_q$ is independent of the other ones, and so, there is a $2$-stable configuration with $q'$ channels for $D$ if, and only if, there exists a $2$-stable configuration with $q'$ channels for every $D_{q_{i_t}}$, $1 \leq t \leq l$. 
\end{proof}
\fi


==> Long/intro-long.tex <==
\section{Introduction}
\label{sec:intro}

Designing algorithms to decompose nodes of a network into various groups, so that they best satisfy some constraints, is both a fundamental computational task and a critical piece for many applications. In a long standing line of research, problems such as network scheduling, resource allocation, and others have been represented as graph coloring. In its simplest form, the objective is to assign a label, generally referred to as a \emph{color}, to each node so that no two adjacent nodes share the same color. In these examples, the \emph{efficiency} of such group assignment is typically estimated by a \emph{global} measure, such as the total number of colors used. Optimizing several measures under different conditions on the graph and the algorithm is now well understood. In contrast much less is known when groups of nodes are formed in a network not by an assignment algorithm but by nodes' selfish choices as each maximizes an \emph{individual} utility that she locally observes. In this paper we are interested to predict the behavior of such selfish group formation process that we call, by analogy with previous graph decomposition algorithm, a \emph{coloring game}.

\paragraph{Understanding group formation in information sharing network.}
Motivation to study group formation among self-interested nodes was recently renewed by the adoption of multiple massive online platforms for information sharing. In previous \emph{directed} communication tools such as phone or email, the intended recipient is stated explicitly. In contrast, online social networks such as Facebook, Google+, and microblogging services such as Twitter and Weibo encourage users to configure \emph{a priori} a set of communities, groups or circles. These groups inherently specifies -- although in a relatively informal way -- the set of people to which an information is visible. Users have embraced this design, and this trend is consistent with a large and increasing body of evidence that spans several decades. As shown in the 1950's by J. Coleman, E. Katz and H. Menzel, \cite{Coleman:1957vq}, and in the 1970's by M. Granovetter \cite{Granovetter:1974te}, your position in a network of \emph{social} connections can be an advantage to receive information about innovation or job offers. With increasing data, more evidence are found of this principle everyday~\cite{Bakshy:2012vv}: participating to social information sharing presents \emph{mutual benefits}, and hence it leads users to create new connections and participate to various groups. On the other hand, sharing information can also be \emph{harmful}, as illustrated by recent examples~\cite{Wang:2011gb,Acquisti:2004gp}. One can informally define the increasing concerns of users for privacy as a need to be protected from such risks. 
Recent trends, such as allowing a user to partition her social neighborhood in various ``circles''~\cite{Kairam:2012dr} are being experimented. However, we lack a general theory bringing insight on how users can possibly navigate this difficult tradeoff to the best of their interest. 

\begin{quote}%\footnotesize
``Nul plaisir n'a goust pour moi sans communication, \\ 
mais il vaut mieux encore estre seul qu'en compagnie \\
ennuyeuse et inepte.''\footnote{loosely translated as: ``Pleasure, I cannot savor it unless I tell someone, but I'd rather be alone than in dull inept company.''}

\hfill 
--
 Montaigne, in \textit{Essais} III-9
\end{quote}

The problem posed to users when deciding which groups to join is a complex one. However, it seems intuitive that users tend to join groups to exchange information primarily because other members are found beneficial, while groups involving individuals that are best not to keep informed (your employer, your ex-partner, or a suspicious stranger) should be avoided. In accordance with previous works~\cite{Kleinberg:2010ul,Adams:1994ht}, we believe that an idealized but general model that reproduce this mechanism already brings important insights. Indeed, understanding groups formed socially can be posed in a very general case as the analysis of a \emph{coloring game}.

\paragraph{Coloring game: Definition, Example.}

We define a \emph{coloring game} on a general weighted graph as follows: each edge denotes a potential connection or alliance, and its weight represents how advantageous this connection is to both nodes\footnote{Although we keep weights symmetric for simplicity here, we also present results for the asymmetrical case in which an alliance is more profitable to one of the nodes (see Section~\ref{sec:extensions}).}. Edges with positive weights denote desirable connections, while an edge with negative weight, \emph{a fortiori} if the weight is very large, denotes a conflictual relationship. A player can strategically decide which color she uses, knowing that she will then receive a utility which depends on the weights of her neighboring edges towards other players picking the same color\footnote{While we mostly focus on the case where the utility is the sum of all these weights, we also present a more general case using subsets (see Section~\ref{sec:extensions}).}. One possible choice is to pick a color no-one else is currently using, in which case she will be isolated and by convention will receive a null utility, as Montaigne suggests above. In addition, a subset of players can decide to act collectively to form a \emph{$k$-deviation} (where $k$ is the size of this subset), by simultaneously changing their colors, as long as \emph{each player in the subset} {strictly increases} her utility.

Figure~\ref{fig:example} presents an example of coloring game involving 12 nodes. The edges in green have a weight $1$, all pairs of nodes that are not connected by a green edge are supposed to be enemies, \ie they are connected by a conflict edge with weight $-\infty$. This graph connects $4$ groups of mutual friends, as shown on the left. All nodes in a given group are enemies with members of other groups except for one node (that can be called the \emph{connector} or the \emph{hub}) that befriends all other connectors or hubs. The number inside a node represents its current utility according to the colors that are assigned.
\begin{figure}[t]
\centerline{\includegraphics[width=0.6\linewidth]{Figures/4transformationArrows.pdf}}
\vspace{-0.2cm}
\caption{Example of a deviation in a coloring game.}
%\vspace{-0.45cm}
\label{fig:example}
\end{figure}

Relatively little is known to date of the behavior of a coloring game, primarily because this model combines features that are rarely found together:
\begin{itemize}
\item {Networks include \emph{positive} and \emph{negative} edges.} 
We can assume that nodes base their decisions to join groups according to a weighted graph in which an edge represents how advantageous it is for these nodes to be in the same group. But as we indicated, an edge may denote a ``positive'' or a ``negative'' interaction to capture both the benefit of connection and the privacy risk. As an extreme case, one node may wish to avoid another \emph{at all costs}: we say in that case that they have a conflict edge. 

\item {Players preferences are arbitrary and private.} 
The information used by nodes to make their decision is typically not public. The game evolves as a series of selfish decisions based on a partial view. It is hence important to obtain results on convergence that apply to \emph{any} graph and also to consider the \emph{worst} sequences of decisions that could delay convergence.

\item {Players can collide.} It is frequently assumed in game theory that nodes can unilaterally deviate but cannot act \emph{collectively} to increase their utility. However, that assumption does not seem to apply so strictly here. Although it can be rare and difficult to do, multiple players can in theory coordinate to change groups at once and form a $k$-deviation. We should carefully study how this could affect the behavior of the game. 
\end{itemize}

\paragraph{Can groups formed in a selfish manner be self-enforcing?}
Our results answer one fundamental challenge: to determine the conditions under which a selfish group formation mechanism leads to a stable outcome. When these conditions are satisfied, it means that the process can lead to inherent groups representing potential communities of interest present in the network. Otherwise, we know that the game will never converge.

To be more precise, we focus on the following properties:
\begin{itemize}
	\item \textbf{Stability:}
		We say that a partition is \emph{$k$-stable} if no deviation of at most size $k$ exists. The existence of such partitions is necessary for the game to converge when these deviations take place. This condition ensures that groups are self-perpetuating: their members have no incentive to deviate and form new alliances. 

In Figure~\ref{fig:example}, partitioning the network into 4 peripheral cliques is self-perpetuating when only 1-2 and 3-deviations are allowed. On the other hand, this partition is not stable against $4$-deviations. 
\item \textbf{Time to converge:} When $k$-stable partitions exist, we also wish to prove that a small number of steps is needed for the game to converge. Note that nodes are not coordinated and hence we need to bound the \emph{longest sequence} of steps before convergence.

For instance, in Figure~\ref{fig:example}, the longest sequence ending in the 4-stable partition on the right has at least one more step than the longest sequence ending to the left. 
\item \textbf{Efficiency:} All games that converge end in a partition in which players will continuously remain in their group, but how does it compare to some optimal choice? One way to answer this question is to compare the sum of all utilities received by players (also called the social welfare of this coloring) to the partition where this quantity is maximized. 

In Figure~\ref{fig:example}, the socially optimal partition shown on the left is not $4$-stable. The right partition is but it achieves a social welfare that is only a fraction $\frac{5}{6}$ of the optimal.
\end{itemize}

\paragraph{Our contribution: the uniform case}

In cases where all edges that do not denote enemies have the same unit weight, a player receives a utility equal to the number of people in her group minus 1. In other words, she always wishes to join a larger group, as long as it does not include nodes connected to her by a conflict edge. This game is equivalent to the information sharing game introduced in \cite{Kleinberg:2010ul}. The authors showed that for small values of $k$ (up to $k=3$) any arbitrary sequence of deviations converges in polynomial time. However, while the mere existence of a $k$-stable partition has been independently established for any $k\geq 0$, we still have no understanding of the \emph{cost} in the number of deviations that are required to attain it. The potential function method used for $k\leq3$ fails otherwise, primarily because deviations of size $4$ can decrease the overall utility of the game (\eg Figure~\ref{fig:example}). A first hint at the difficulty of this problem is that finding a $k$ stable partition is NP-hard whenever $k$ is part of the input.

We prove that the longest sequence of steps in a uniform game can be analyzed in the Dominance Lattice (previously introduced in theoretical physics and combinatorics). In contrast with potential function methods, that are shown to be loose, this new proof methods provides for the first time an \emph{asymptotically exact} formula for the number of steps required in the worst case. Our second major result is to close the main open problem in~\cite{Kleinberg:2010ul} by proving that as soon as $k=4$ the number of steps needed in this game admits no polynomial bound. This \emph{sudden complexity increase} can be established using a new representation of the game in a space where sequences of steps can be built to satisfy a \emph{cascading} property. This offers an entirely new method to construct lower bounds, which brings other results completing the analysis of convergence in the uniform case.

\paragraph{Our contribution: the general case}
Coloring games when weights are non-uniform are far more difficult to analyze. As an example, we provide a simple graph that does not admit a $2$ stable partition in Figure~\ref{fig:nonstable}.
\begin{figure}[t]
\centerline{\includegraphics[width=0.6\linewidth]{Figures/TriangleWPart.pdf}}
\caption{A coloring game that does not admit $2$-stable partition: Edges in green have the positive weight indicated, Red edges denote enemies. All partitions are unstable. As an example, starting from assignment into groups on the right, nodes $v1$ and $v2$ can decide to simultaneously move into the group containing $u3$, which effectively ``rotates'' the group partition.}
\label{fig:nonstable}
\end{figure}
Prior to our work, no result exists that even guarantees simply the existence of a $k$-stable partition. 
First, on the positive side, we generalize the potential method to prove the convergence in polynomial time for all games when only $1$-deviations are allowed. Our argument extends to $2$-deviations whenever all positive weights are equal to $1$ and all other negative or null weights are allowed. Our analysis again provides tight bounds on the convergence time.

We completely answer the general case as we are able to show that these results are tight in a very strong sense. \emph{First}, we show no more general results ever exist: as soon as $3$-deviations are allowed, even when a single positive weight is used, a counterexample can be derived. All other sets of possible weights that are neither trivial nor trivially equivalent to one of these cases, admit games that are not $2$-stable. \emph{Second}, we prove that whenever the conditions of our above results are not satisfied, deciding if the game will converge is not just uncertain, but it is a NP-hard problem.
In order to establish such results that completely determine conditions for self-enforced groups in the general case, we need to build a series of graph transformations that allow to derive stronger counterexamples while reducing the weights that are allowed. We also build a reduction between convergence from \emph{any} graph and a maximum independent set only using that a single counterexample exists. We found many of these results surprising, especially as in most of those cases they use 2-deviations and those never diminish total utility. 

\paragraph{Our contribution: more general coloring games}
We finally show that our results generalize for more general classes of games. First, we show that assuming asymmetrical weights or allowing the ``gossip'' deviation defined in \cite{Kleinberg:2010ul} creates additional instability. Second, we show that allowing a node to choose multiple colors, or equivalently to build overlapping groups, allows convergence under the same general conditions we previously identified. However, surprisingly in the other cases multiple colors per node are \emph{counter-productive}: we even exhibit a counter-example that is not $3$ stable \emph{in the uniform case}, whereas a partition exists for all $k$ with a single color. Finally, we prove that all our results naturally extend beyond symmetric pairwise relationships to account for multimodal interaction in hypergraphs.

We conclude with two results illustrating the tension between stability and efficiency in coloring games. While we show that the ``price of anarchy'' is generally large, we demonstrate that allowing collusions and using multiple colors have a significant and positive effect on the efficiency. This complements our analysis by showing that the cases in which convergence is the most difficult to guarantee are also those in which the system may form better groups overall. It motivates future research to design games operating close but not beyond the complexity frontier we unveil.

\paragraph{Related work}
The work most relevant to coloring games is an information sharing model where groups are connected components of a graph formed as local edges are opened by peers \cite{Kleinberg:2010ul}. We already discussed those results in the uniform case, for which this game is equivalent to ours. In the general case, the authors provide one counter-example of stability, which is built around the \emph{gossip} deviation. In gossip deviation, two nodes are allowed to merge their connected components or, equivalently, that the two nodes' colors become a single color. We analyze games with and without the gossip deviation, as we show more generally that the deviation always introduces instability. 

Graph coloring, in which an edge represents such a conflict, has been the subject of a long tradition of computational research. Similarly, the structure of social networks with positive and negative edges has been a topic of interest since the 1950s. 
A first aspect that sets our results apart from previous works is that we consider the individual interest of the nodes, instead of attempting to satisfy a global property (\eg minimizing the number of colors). 
Similarly, networks with positive and negative links have been studied traditionally by looking at \emph{global} properties that they satisfy such as \emph{structural balance}~\cite{Cartwright:1956dh}. This theory predicts that positive and negative relationships evolve so as to avoid triangles with an odd number of conflict edges. In fact, structurally balanced graph admits trivially self-enforcing group-assignment as they end up forming one or several cliques of mutual friends that are enemies with other cliques. However, recent results on signed networks in social media~\cite{Leskovec:2010us,Leskovec:2010wu,Yang:ht} showed that graphs are rarely perfectly balanced. Our results extend this work to understand under which conditions even non-structurally balanced graphs, and some with various weights, can still lead to self-enforcing groups.
Our work also highlights for one of the first time the importance of accounting for complexity, and not only existential results, when analyzing networks with positive and negative edges.

This model of group formation is a novel direction. Most models explaining network formation either deal with ensuring connectivity~\cite{Jackson:2003ua}, or matching~\cite{Ming:2011tq} under local cost constraint such as number of edges or queries. \emph{Alternatively}, they may balance a global risk propagation with rewards from local connections \cite{Blume:2011vg}. In contrast, we \emph{jointly} consider both the positive and negative aspects of social interaction \emph{within the same graph}. This mirrors the situation many users face online when balancing privacy with utility. This topic, one of fundamental importance to the design of social networking software (see~\eg \cite{Kairam:2012dr}) was previously unexplored. 
Our work is also one of the first to consider how groups and connections form when users follow non-uniform preferences, and to attempt to go beyond Nash equilibrium, as opposed to most previous game-theoretical approaches~\cite{Galeotti:2010tj}. 

\cite{Chatzigiannakis:2010vo,Epstein:2007gv,Augustine:2011wj,Zick:2012ui,Chalkiadakis:2010ui,Bloch:2011ta,Panagopoulou:2008dr,Escoffier:2012vu}

%We omit most proofs, they can be found in~\cite{RR}.




==> Long/model-long.tex <==
%\begin{figure}[t]
%\centerline{\includegraphics[width=0.5\textwidth]{Figures/triangle-ex}}
%%\vspace{-0.2cm}
%\caption{A network with set of weights $\mathcal{W}=\{-\infty,2,3,4\}$.}
%%\vspace{-0.45cm}
%\label{fig:fig-triangle}
%\end{figure}

\section{Information Sharing Model}
\label{sec:model}

Let us first define coloring games in a formal way.

\paragraph{The Social Network}
We model the social network with an edge-weighted graph $G=(V,E,w)$, where $V$ denotes the set of users.
There are $n = |V|$ users in the network.
Moreover, it is supposed to be a \emph{simple} graph, hence there is no loop and no multiple edges.
The weight $w_{uv}$ is defined for every edge $uv \in E$ as the utility both $u$ and $v$ receive if they share information.
Note that $w_{uv} = w_{vu}$ by symmetry.
In the general case, $w_{uv} \in \mathbb{Z} \cup \{ - \infty , N\}$, where $N$ denotes an arbitrarily large positive weight that is at least $n$ times greater than any other (finite) weight in absolute value.
In other words, for any two vertices $u,v \in V$, if $w_{uv} = -\infty$ then the users are \emph{enemies} and they never share anything, whereas if $w_{uv} = N$ then they are \emph{best friends} and they always share information unless there is an enemy to interfere. 
Given the natural dominance of weight $-\infty$ over all the other ones, we also say that $uv$ is a \emph{conflict edge} when $w_{uv} = -\infty$.

Sometimes, the set of possible weights may be constrained, and we will denote it $\mathcal{W}$.
Also, missing edges in the graph can be added with weight $0$; so, without loss of generality, we assume that $G$ is a complete graph, and we will simply write $G=(V,w)$ in the sequel.
An example of a network with  $\mathcal{W} = \{-\infty,2,3,4\}$ is presented in Figure~\ref{fig:nonstable}.\\

\noindent
We suppose in our model that the users are \textit{partitioned} into $n$ sharing groups, some of them may be empty. 
Such a partition of the nodes is denoted $P = \{X_1, X_2, \ldots, X_n\}$.
Figure~\ref{fig:example} presents two different partitions of the nodes for a graph with $\mathcal{W} = \{-\infty, 1\}$.

For a given $P$, the \emph{utility} for the user $u$ is defined as $f_u(P) = \sum_{v \in X(u) \setminus \{u\}} w_{uv}$, where $X(u)$ denotes the sharing group in $P$ which $u$ belongs to.
The global utility, or social welfare, is $f(P) = \sum_{u \in V} f_u(P)$. 
Note as an example that vertices in Figure~\ref{fig:example} are labeled with their individual utilities.

\paragraph{Dynamic of the game}
Users in the networks want to maximize their individual utility.
Initially, none of them share information, and so, we only have singleton groups.
Then we fix a constant parameter $k \geq 1$, and the coloring game starts.

At each round $i$, we consider the current partition $P_i$ of the nodes.
In particular, there are only singleton groups in $P_0$.
Given a coalition $S$ with at most $k$ players, we say that $S$ is a \emph{$k$-deviation}, or $k$-set, when all the users in $S$ have an incentive to join the same (possibly empty) group in $P_i$, so that they \emph{all} increase their individual utility in the process.
When such a deviation exists, we may allow any \emph{one} of them to happen and, in so doing, we \emph{break} $P_i$, and we get a new partition $P_{i+1}$.

For instance, Figure~\ref{fig:example} shows a possible update of the partition of the nodes after a $4$-deviation.
Finally, the game stops if and only if there is no possible $k$-deviation.
We call a partition $P$ such that there is no $k$-deviation that breaks $P$, if any,  a \emph{$k$-stable} partition.
An algorithmic presentation of the game is given below.

\begin{algorithm}[h]
%\caption{- Cascading failure model}
\textbf{Dynamic of the system}\vspace{1mm}
{\hrule height0.8pt depth0pt \kern0pt}\vspace{-.5mm}
\label{algorithm:dynamic}
\begin{trivlist}
\item\textbf{Input:} A positive integer $k \geq 1$, a set of weights $\mathcal{W}$, and a graph $G=(V,w)$.
\vspace{-0.1cm}
\item\textbf{Output:} A partition $k$-stable for $G$.
\end{trivlist}
\vspace{-0.2cm}
\begin{algorithmic}[1]
\STATE Let $P_{0}$ be the partition composed of $n$ singletons groups.
\STATE Set $i = 0$.
\WHILE{there exists a $k$-deviation for $P_{i}$}
\STATE Set $i = i+1$.
\STATE Compute the partition $P_{i}$ after any $k$-deviation.
\ENDWHILE
\RETURN Partition $P_{i}$.
\end{algorithmic}
\end{algorithm}



We will discuss in the sequel several extensions of the model.
We will show that most of our results still hold for these more general games.   


==> Long/unweighted-long-k=1,2.tex <==
\section{The uniform case: Are longest deviation sequences polynomial?}
\label{sec:unweighted}

A coloring game is said \emph{uniform} if, except for conflict edges, all edges have the same unit weight (\ie $\mathcal{W} = \{-\infty,1\}$). This game is entirely characterized by an unweighted and undirected \emph{conflict graph} $G^-=(V,E)$ that contains all the conflict edges (\ie those with weight $-\infty$).
The complementary graph of $G^{-}$ represents all the pairs of friends (with unit weight).
Note also that, for any user $u$, the individual utility $f_u(P)$ equals $|X(u)|-1$, which is how many nodes are in the group in addition to $u$. As shown in~\cite{Escoffier:2012vu,kleinberg2013information} $k$-stable partitions always exist for any value of $k$.
Let us first mention why this game converges for any $k\geq 1$. For a partition $P$ and any $i$ we define $\lambda_{i}(P)$ to be the number of groups of size $i$, and let $\Lambda(P) = (\lambda_{n}(P), \ldots, \lambda_{1}(P))$ be its \emph{partition vector}. One can see that a deviation \emph{of any size} produces a partition vector that is strictly higher in the lexicographical ordering. (for a more formal argument, see our Lemma~\ref{lem:convergence-k-stable} in the Appendix) 

We can then define $L(k,n)$ as the size of a longest sequence of $k$-deviations among all the graphs with at most $n$ nodes. One can prove (see Lemma~\ref{lem:graphe-vide} in the Appendix) that $L(k,n)$ is always attained in the graph containing no conflict edges, an instrumental observation for our next proofs. 

Prior to this work, no lower bound on $L(k,n)$ was known, and the analysis was limited to potential function that only applies when $k=1,2,$ and $3$~\cite{Escoffier:2012vu,kleinberg2013information}. The analysis of the game becomes much more difficult as soon as $4$-deviations are allowed. Table~\ref{tab:tab-graph-complexity} summarizes our contributions: 

%the exact value of $L(k,n)$ for small values of $k$ and the proof that its combinatorial properties suddenly increases as $k=4$.

% We represent this class of instances by undirected graphs where edges represent enemies.
% Furthermore, the dynamic of the system always converges to a stable partition.
% A useful remark is that such a sequence of $k$-deviations is maximum for graphs without edges.\\

\begin{table}[h]
\begin{center}
\tbl{Previous Bounds and results we obtained on $L(k,n)$.}{%
\begin{tabular}{|c|c|c|c|}
\hline
$k$ & Prior to our work & \multicolumn{2}{c|}{\textbf{Our results}} \\
\hline
1 & $O(n^{2})$ \cite{kleinberg2013information}& exact analysis, which implies $L(k,n) \sim \frac{2}{3}n^{3/2}$ & Theorem~\ref{lem:tight:k=1}  \\
\hline
2 & $O(n^{2})$ \cite{kleinberg2013information}& exact analysis, which implies $L(k,n) \sim \frac{2}{3}n^{3/2}$ & Theorem~\ref{lem:tight:k=2}  \\
\hline
3 & $O(n^{3})$ \cite{kleinberg2013information}& $\Omega(n^{2})$ & Theorem~\ref{thm:lower-bound-3}  \\
 & \cite{Escoffier:2012vu}&  & \\
\hline
$\geq 4$ & $O(2^{n})$ \cite{kleinberg2013information} & $\Omega(n^{\Theta(\ln(n))})$, $O(\exp({\pi\sqrt{{2n}/{3}}})/n)$ & Theorem~\ref{lem:lower-bound-4}  \\
%$\geq 4$ & $O(2^{n})$~\cite{kleinberg2013information} & $\Omega(n^{a \ln(n)})$, $O(\frac{e^{\pi\sqrt{\frac{2n}{3}}}}{n})$ & Theorem~\ref{lem:lower-bound-4}  \\
\hline
\end{tabular}}
\label{tab:tab-graph-complexity}
\end{center}
\end{table}


\subsection{Exact analysis for k $\leq$ 2}
\label{ssec:k=12}

In~\cite{kleinberg2013information}, the authors proved the global utility increases for each $k$-deviation when $k \leq 2$. As that potential function is also upper bounded by $O(n^2)$, the system converges to a $2$-stable partition in at most a quadratic time.
We improve this result as we completely solve this case and give the exact (non-asymptotic) value of $L(k,n)$ when $k\leq 2$. It also proves that this potential function method is not tight. The gist of the proof is to re-interpret sequences of deviations in the Dominance Lattice.
This object has been widely used in theoretical physics and combinatorics to study systems in which the addition of one element (\eg a grain of sand) creates consequences in cascade (\eg the reconfiguration of a sand pile)~\cite{Goles1993321}. 
%This property, frequently called self-organized criticality, shows that coloring games are strongly chaotic. 
Let us define:
\begin{definition}[\cite{Brylawski1973201}]
An integer partition of $n \geq 1$, is a decreasing sequence of integers $Q = q_1 \geq q_2 \geq \ldots \geq q_n \geq 0$ such that $\sum_{i=1}^{n}q_{i} = n$. 
\end{definition}

Given any game with $n$ nodes, there are as many partition vectors as there are integer partitions of $n$.
Thus in the sequel, we will make no difference between a partition vector and the integer partition it represents.
If we denote the number of integer partitions by $p_{n}$, then we know the system reaches a stable partition in at most $p_{n}=\Theta((e^{\pi\sqrt{\frac{2n}{3}}})/n)$ steps\footnote{The upper-bound directly follows from Lemma~\ref{lem:convergence-k-stable} (\ie the lexicographical ordering argument).}.
This is already far less than $2^n$, which was shown to be the best upper bound that one can obtain for $k \geq 4$ when using an additive potential function~\cite{kleinberg2013information}. 
%To go further, one needs to go beyond lexicographical ordering.
For $n\geq 6$ it can be seen that some partitions $P$ of the nodes may never be in the same sequence.
It is hence important to deal with a partial ordering instead of a total one. Brylawski proved in~\cite{Brylawski1973201} that a dominance ordering creates a lattice on integer partitions, where successors and predecessors can be defined by covering relation:
\begin{definition}(dominance ordering)
Given two integer partitions 
of $n \geq 1$,
denoted $Q = q_{1} \geq \ldots \geq q_{n}$ and $Q' = q_{1}' \geq \ldots \geq q_{n}'$, we say that $Q'$ dominates $Q$ if 
$\sum_{j=1}^{i}q_{j}' \geq \sum_{j=1}^{i}q_{j}$,
for all $1 \leq i \leq n$.
\end{definition}
%That dominance relation can be extended to a partial ordering of the integer partitions. In so doing, 
\begin{definition}(covering)
Given two integer partitions $Q,Q'$ of $n \geq 1$, 
$Q'$ \emph{covers} $Q$ if and only if $Q'$ dominates $Q$ and no other integer partition $Q''$ satisfies $Q'$ dominates $Q''$ and $Q''$ dominates $Q$.
\end{definition}

% One can also check that $a$ dominates $b$ if, and only if, we have a sequence $a = q_1, q_2, \ldots, q_p = b$, where $q_i$ covers $q_{i+1}$ for all $1 \leq i \leq p-1$. 

\noindent
The main ingredient of our analysis is to exploit a strong relationship between this structure and $1$-deviations in a game, that holds as long as no conflict edges exist (see details of the proof in appendix).
\begin{lemma}[\cite{Brylawski1973201}]
\label{dominance-characterization}
%Given two partitions $a = (a_1,\ldots,a_n)$ and $b=(b_1,\ldots,b_n)$ of an integer $n \geq 1$, then 
Given $Q,Q'$,
$Q'$ covers $Q$ if and only if there are $j,k$ such that:
%\begin{itemize}
%\item 
$(i)$ 
$q_j' = q_j+1$;
%\item 
$(ii)$ 
$q_k' = q_k - 1$;
%\item 
$(iii)$ 
for all $i \notin\{j,k\}$, we have $q_i' = q_i$;
%\item 
$(iv)$ 
either $k=j+1$ or $q_j = q_k$. 
%\end{itemize}
\end{lemma}
%\vspace{-0.5cm}
\begin{corollary}
\label{corollary:equiv-dominance-dev}
Assuming no conflict edges exist (\ie $G^{-}=(V,E)$ with $E=\emptyset$), let $Q,Q'$ be two integer partitions of $n$.
Then, $Q'$ dominates $Q$ if and only if there exist two partitions $P,P'$ of the nodes such that $\Lambda(P') = Q'$, $\Lambda(P) = Q$, and there is a valid sequence of $1$-deviations from $P$ to $P'$.
\end{corollary}

\begin{figure}[t]
\centerline{%\includegraphics[width=0.5\linewidth]{Figures/Unstablek4noborder.pdf}
\includegraphics[width=0.65\linewidth]{Figures/Sandpile.pdf}}
%\vspace{-0.3cm}
\caption{An example of decomposition for a $1$-deviation from group $X_k$ to group $X_j$.}
%\vspace{-0.25cm}
\label{fig:sandpile}
%\vspace{-0.3cm}
\end{figure}


In other words, any sequence of $1$-deviations, from a partition $P$ to another partition $P'$, can be decomposed into more elementary $1$-deviations, satisfying that if there is such an elementary deviation from the partition $P_i$ to the partition $P_{i+1}$, then the integer partition $\Lambda(P_{i+1})$ covers $\Lambda(P_i)$. Note that, by doing so, we may get another final partition $P'' \neq P'$ but it will have the same partition \emph{vector}, as seen on an example in Figure~\ref{fig:sandpile}.  
%For our purpose, since the new sequence has a size that is larger than the original one, and it is a sequence of $1$-deviations that %is also valid, which proves (see appendix).
% We call a \emph{chain} any  sequence $q_1, q_2, \ldots, q_p$, such that for every $2 \leq i \leq p$ we have $q_{i+1}$ dominates $q_{i}$.
% The size of such a chain is the number $p$ of partitions in the chain.
% We can now prove the main result of this section:
%
% \begin{lemma}[\cite{Greene:1986:LCL:11002.11003}]
% \label{lemma:max-chain}
% Given an integer $n$, it can be written as $n = \frac{m(m+1)}{2} + r$ in a unique way, such that $0 \leq r \leq m$.
% Then the longest chain of integer partitions of $n$ has a size $\frac{m(m+1)}{2} -  \frac{(m-r)(m+1-r)}{2} + \frac{r(r-1)}{2} \sim \frac{2}{3} n\sqrt{n}$.
% \end{lemma}
\begin{theorem}
\label{lem:tight:k=1}
Let $m$ and $r$ be the unique non negative integers such that $n = \frac{m(m+1)}{2} + r$, and $0 \leq r \leq m$.
We have $L(1,n) = 2 \binom{m+1}{3} + mr$.
This implies that $L(1,n) \sim \frac{2}{3} n\sqrt{n}$ as $n$ gets large.
\end{theorem}

Interestingly, we prove that $2$-deviations have a similar action on partition vectors, which implies:
%Following a similar line of argument using partition vectors we can further prove:
\begin{theorem}
\label{lem:tight:k=2}
$L(2,n) = L(1,n)$.
\end{theorem}

